Quantitative Analysis of Community Evolution in Developer Social Networks Around Open Source Software Projects

Understanding the evolution of communities in developer social networks (DSNs) around open source software (OSS) projects can provide valuable insights about the socio-technical process of OSS development. Existing studies show the evolutionary behaviors of social communities can effectively be described using patterns including split, shrink, merge, expand, emerge, and extinct. However, existing pattern-based approaches are limited in supporting quantitative analysis, and are potentially problematic for using the patterns in a mutually exclusive manner when describing community evolution. In this work, we propose that different patterns can occur simultaneously between every pair of communities during the evolution, just in different degrees. Four entropy-based indices are devised to measure the degree of community split, shrink, merge, and expand, respectively, which can provide a comprehensive and quantitative measure of community evolution in DSNs. The indices have properties desirable to quantify community evolution including monotonicity, and bounded maximum and minimum values that correspond to meaningful cases. They can also be combined to describe more patterns such as community emerge and extinct. We conduct experiments with real-world OSS projects to evaluate the validity of the proposed indices. The results suggest the proposed indices can effectively capture community evolution, and are consistent with existing approaches in detecting evolution patterns in DSNs with an accuracy of 94.1\%. The results also show that the indices are useful in predicting OSS team productivity with an accuracy of 0.718. In summary, the proposed approach is among the first to quantify the degree of community evolution with respect to different patterns, which is promising in supporting future research and applications about DSNs and OSS development.

==> 1_introduction.tex <==
\IEEEraisesectionheading{\section{Introduction}
\label{sec1}}
%%%%%%%%%%%%%%%%%%  %%%%%%%%%%%%%%%%%%%%%
\IEEEPARstart{I}{n} the face of a huge number of web users and information explosion, recommender systems are of vital importance which can alleviate information overload and provide users with more efficient and high-quality services. An effective recommender system can benefit both users by acquiring their preferred contents (e.g. movies, music, merchandise) from a large amount of information, and service providers by reducing promotional costs. As a result, recommender systems have attracted widespread interests in recent years. 
%A variety of Internet companies, such as Alibaba, Amazon, Facebook, etc., and many academics are pushing for this technology. 
%Generally speaking, there are two main types of recommender algorithms: content-based algorithms \cite{PazzaniBillsus07} and collaborative filtering algorithms \cite{GoldbergNichols92}. Among these methods, collaborative filtering has been widely used because of its effectiveness and scalability. Matrix factorization \cite{HuKoren08,KorenBell09}, one of the most important collaborative filtering methods, has achieved great success in various scenarios \cite{LiuRogers17,SmithLinden17}. It maps users and items to a shared latent factor space, and interactions between users and items are modeled by the inner product of their latent factors.
Meanwhile, exploiting social relations to improve the performance of recommendation has also become increasingly popular with the growth of social media \cite{MaZhou11,TangHu13a,TangWang16}.  %\cite{MaZhou11,TangHu13a,TangWang16} demonstrated that exploiting because social relations can contribute to improve recommendation performance
In social networks, there is a flow of information among connected friends. A user's preference is similar to or influenced by the people around him/her, which has been proved by social correlation theories \cite{MarsdenFriedkin93,McPhersonSmith01}. 

%In \cite{WengLimwsdm10}, the authors found that users with following relations are more likely to share similar interests in topics than two randomly chosen users. Moreover, users with strong ties are more likely to share similar tastes than those with weak ties, treating all social relations equally is likely to lead to degradation in recommendation performance \cite{TangHu13b}. Therefore, the social relations play a significant role to help the users filter information. Many social-based recommendation algorithms have been presented to improve the recommendation accuracy \cite{MaYang08,JamaliEster10,MaZhou11,YangLei16}. In \cite{MaYang08}, a factorization approach was proposed to solve the rating prediction problem by employing both the users' social network information and rating records. TrustMF \cite{YangLei16} was introduced by using the matrix factorization of the trust network between the users in social interactions for the rating prediction. One can find comprehensive overviews about social recommendations in \cite{TangHu13b}.

Recently, deep learning has shown strong capability to achieve good performance due to its high expressiveness and model fidelity. Graph neural networks (GNNs) utilize the advances of deep learning for graph-structured data and have been applied for various fields such as geo-location \cite{nassar2020geograph, rahimi2018semi} and bio-informatic \cite{fout2017protein,liu2020deep}.
% Despite utilizing deep learning for feature extraction (e.g.,music audio features \cite{VanDieleman13} and image visual content \cite{ZhaoLu16}), attempts have also been made to directly use deep learning to model user-item interactions. 
For the domain of social recommendation, the user-item interactions and user-user friendship can be naturally represented as graphs, in which users and items are the nodes while interactions (friendship) are the edges. Based on such observations, utilizing the recent advance of GNNs for social recommendation has become a promising research direction. 


However, almost GNN-based recommendation methods are learned from the original interaction graph with little attention paid to the statistical information of the graphs, which could result into misunderstanding of the real user preference. For example, from the user perspective, a fastidious user may tend to give a low rating to every movie he has watched, then a rating of 3 out of 5 may actually denote a positive preference of this user. From the item perspective, a rating 4 of 5 could also represent a negative attitude if the average rating for this item can achieve a high score (e.g., 4.5). This is a bias hidden in the data that would mislead the training for users and items representations. The author in \cite{koren2008factorization} has introduced similar considerations. Based on this insight, FunkSVD and SVD++ have been proposed, which model these user and item biases as scalars in rating predictions. However, we argue that these methods are simple but do not capture the true bias hidden in practice.  Firstly, we consider that using scalar is not enough to completely model the real biases of users and items. Secondly, existing methods do not explicitly construct the biases in data, but use original data to learn. It also lead to an inability to learn the bias well.
Besides, the social connection strength should also be differentiable. In  \cite{TangHu13b}, it demonstrates that users with strong connections are more likely to share similar tastes than those with weak connections and thus treating all social relations equally would also lead to sub-optimal solutions.


In this paper, we design a new GNN-based model to address the above problems for social recommendation. More precisely, we treat the biases as vectors and fuse them into user/item representations in the proposed model. This design could help us to learn the representations well. To this end, we design a decentralized interaction graph to consider the statistical bias offsets of users (items). This graph is constructed by extracting bias information explicitly and helps the model learn better representations. Besides, we re-weight the user-user connections according to the preference similarity, which can help the model focus on useful friendship connections while denoise the redundant aggregation.
Our major contributions are summarized as follows:
\begin{itemize}[leftmargin=*]
	\item We treat the rating biases as vectors and fuse them into the process of learning user and item representations. To this end, we introduce a new perspective to process the original graph to a decentralized graph and learn the user and item representations from it. The decentralized graph is acquired through exploiting the statistical information of the original data, thus the bias information is extracted explicitly on the graph.
	\item A simple yet effective explicit strength of the social connection is given, which can be then incorporated into the final prediction rule and helps to improve the recommendation performance.
	%The explicit strength of the social relation can help to improve the prediction accuracy.
	\item We propose a new GNN-based collaborative filtering model (GDSRec) for social recommendation, which are learned on the decentralized graph with explicit differentiable social connection strengths.
	\item We conduct experiments on two real-world datasets to verify the effectiveness of the proposed model. Experimental results show that GDSRec outperforms the compared state-of-the-art baselines.
\end{itemize}

The remainder of this paper is organized as follows. In Section \ref{sec2}, we introduce the background including related works and some notations. The proposed framework is detailed in Section \ref{sec3}. In Section \ref{sec4}, experiments on two real-world datasets are conducted to validate the proposed approach. Finally, we give a conclusion of this paper in Section \ref{sec5}.



==> 2_background.tex <==
\section{Background}
\label{sec2}

\subsection{Related Work}
For the general recommendation task, there are two main types of algorithms: content-based algorithms \cite{PazzaniBillsus07} and collaborative filtering algorithms \cite{GoldbergNichols92, JinSi03}. Among these methods, collaborative filtering has been widely used because of its effectiveness and scalability. Matrix factorization \cite{HuKoren08,KorenBell09,GuZhou10}, one of the most important collaborative filtering methods, has achieved great success in various scenarios \cite{LiuRogers17,SmithLinden17}. It maps users and items to a shared latent factor space, and interactions between users and items are modeled by the inner product of their latent factors. In \cite{koren2008factorization}, SVD++ considers user and item biases that extends matrix factorization model. Besides, explorations of social networks for recommendation have been proved to be effective. In \cite{WengLimwsdm10}, the authors found that users with following relations are more likely to share similar interests in topics than two randomly chosen users. Therefore, the social relations play a significant role to help the users filter information. Based on such observation, many social-based recommendation algorithms have been presented \cite{MaYang08,JamaliEster10,MaZhou11,YangLei16,WangLu16,WangHoi17}. In \cite{MaYang08}, a factorization approach was proposed to solve the rating prediction problem by employing both the users' social network information and rating records. TrustMF \cite{YangLei16} was introduced by using the matrix factorization of the trust network between the users in social interactions for the rating prediction. TrustSVD \cite{guo2015trustsvd} exploits trust information that extends SVD++. The authors in \cite{WangLu16,WangHoi17} utilized Jaccard's coefficient to compute the strength of the social relations, but did not take the ratings into account. Furthermore, some other works utilized side information to improve the recommendation quality, e.g. \cite{YuRen14,ShiHu18}. Recently, SREPS \cite{liu2018social} learns the user's multiple preference in different scenarios. 

Deep learning models have also been exploited to enhance the model expressiveness for recommendation.
Due to the fact that the recommendation data can be naturally organised as graphs, research about exploiting GNNs \cite{ThomasWelling16,DefferrardBresson16,HamiltonYing17,MaWang19} for recommendation have also been conducted. The key insight of GNNs is to learn the representations of the nodes by aggregating feature information from neighborhoods. This conforms the nature of collaborative filtering. 
In \cite{BergKipf17}, the authors proposed a graph auto-encoder framework called graph convolution matrix completion (GCMC) based on differentiable message passing on the user-item interaction graph without using the social relations. Neural graph collaborative filtering (NGCF) \cite{WangHesigir19} was proposed to integrate the user-item interactions into the embedding
process.Knowledge graph attention network for recommendation (KGAT) \cite{WangHesigkdd19} was introduced to explicitly model the high-order connectivities in knowledge graph. DiffNet \cite{WuSun19} was proposed by using a layer-wise influence diffusion part to model how users' latent preferences are recursively influenced by trusted users. A GNN-based social recommendation algorithm, GraphRec, was introduced in \cite{FanMa19}. It provides an approach to jointly capture the interactions and the ratings for learning the representations of the users and the items. Further, the social network information is employed in GraphRec for learning better representations of the users. DANSER \cite{wu2019dual} proposes two dual graph attention networks to learn deep representations for social effects in recommender systems. Diffnet++ \cite{wu2020diffnet++} promotes the user and item representations by injecting both the higher-order user latent interest reflected in the user-item graph and higher-order user influence reflected in the user-user graph. LightGCN \cite{he2020lightgcn} simplifies NGCF with removing nonlinear activation and feature transformation in graph convolution networks and promotes the performance of recommendation. ESRF \cite{yu2020enhance} develops a deep adversarial framework based on graph convolution networks to address the challenges of social recommendation. FBNE \cite{chen2020social} explores the implicit higher-order user-user relations though folding a user-item bipartite graph to improve the performance of social recommendation. HOSR \cite{liu2020modelling} is to generate user embedding by performing embedding propagation along high-order social neighbors. However, most of these methods fail to consider the statistic offsets existing in the graph data while also lack an effective yet simple design for the strength of social relations. 


\subsection{Notations}
Let $\mathcal{O}$ be the set of observed ratings (i.e., $r_{ij} \neq 0$). $R(v_j)$ is the set of users who have interacted with the item $v_j$ and $R(u_i)$ is the set of items which the user $u_i$ has interacted with. Let $N(u_i)$ be the set of users whom the user $u_i$ connects within the social network directly. The vector $\mathbf{p}_{u_i} \in \mathbb{R}^D$ denotes the embedding of user $u_i$, and $\mathbf{q}_{v_j} \in \mathbb{R}^D$ represents the embedding of item $v_j$, where $D$ is the embedding size. $E(u_i)$ and $E(v_j)$ denote the average ratings of the user $u_i$ and the item $v_j$, respectively. $\lceil\cdot\rceil$ and $|\cdot|$ are the integer-valued function and the absolute-valued function, respectively. $\oplus$ denotes the concatenation operation between two vectors. $\langle\cdot\rangle$ is used to obtain the number of entries in a dataset.


==> 3_methodology.tex <==
\section{The Proposed Framework}
\label{sec3}
We first give the problem formulation, then introduce the decentralized graph and the proposed framework. Later, we detail how to get a predicted rating and learn the user/item latent factor offsets from the proposed model. Finally, we explain how to train the model.

\begin{figure}
	\centering
	\setlength{\abovecaptionskip}{0cm}
	\includegraphics[width=0.48\textwidth]{Picture/problem_definition_combination.eps}
	\caption{(a) The user-item rating matrix; (b) the interactions of the user $u_1$. }
	\label{fig1}
	\vspace{-0.2cm}
\end{figure}

\begin{figure}[t]
% \setlength{\abovecaptionskip}{-0.1cm} %缩小caption和图像之间的距离
	\centering
	\includegraphics[width=0.5\textwidth]{Picture/decentralized_graph.eps}
	\caption{The original bipartite graph can be processed as a decentralized graph.}
	\label{fig2a}
\end{figure}


\begin{figure}[t]
\setlength{\abovecaptionskip}{-0.1cm} %缩小caption和图像之间的距离
	\centering
	\includegraphics[width=0.5\textwidth]{Picture/proposed_framework_new_1.pdf}
	\caption{The overview of the proposed framework. It contains four components: user modeling, item modeling, social modeling and preference rating prediction.}
	\label{fig2}
\end{figure}

\subsection{Problem Formulation}
\label{subsecproblem}
Suppose that there are $N$ users $\mathcal{U} = \{u_1, u_2, \cdots, u_N\}$ and $M$ items $\mathcal{V} = \{v_1, v_2, \cdots, v_M\}$. As illustrated in Fig. \ref{fig1}(a), each user rates some items. If the rating can be observed, the rating score is greater than 0, otherwise there are missing values. %The higher the rating is, the more the user likes the item. 
The user-item rating matrix is denoted by $\mathbf{R} \in \mathbb{R}^{N \times M}$. %In this paper, we consider the task of rating prediction which 
The task is to predict the unobserved ratings in $\mathbf{R}$ and then return a ranked list of items for recommendation. To this end, the rating history and social relationships of users are employed to solve this problem. For example, we assume that the items $v_2$ and $v_4$ are rated by the user $u_1$ in Fig. \ref{fig1}(a), and the user $u_1$ has social relationships with the users $u_2$ and $u_4$ directly, as illustrated in Fig. \ref{fig1}(b). The left part of Fig. \ref{fig1}(b) containing the interactions between the users and the items is called user-item graph, and the right part containing the interactions between the users is called social graph. For the 
value in the edge of user-item graph, it represents the user $u_i$'s rating $r_{ij}$ on the item $v_j$. For the value in the social graph, we define it as the relationship coefficient between the users $u_i$ and $u_j$, i.e.,
\begin{equation}
   T_{ij} = 1 + \sum\limits_{v_k \in \{R(u_i)\cap R(u_j)\}} I\left(\left|r_{ik}-r_{jk}\right| \leq \delta \right), 
\end{equation}
where $I(x) = 1$ when $x$ is satisfied and zero otherwise, $\delta$ is the threshold for evaluating two users whether they like the same one item. 
%We do not consider using $I\left(\left|r_{ik}-r_{jk}\right|=0)$ for two reasons. One is that data with equal ratings between users and friends is very sparse, the other is that the ratings may not be the same for the same preference. To this end, the condition is slack. 
The relationship coefficient $T_{ij}$ represents the explicit relationship strength between the users, and denotes how much the user $u_i$ is similar to the socially connected user $u_j$. The higher the relationship coefficient is, there are more common items the two users like or dislike, in other words, the two users are more similar with each other. In order to predict the ratings of the user $u_1$ on the items $v_1$, $v_3$, we use the data described in Fig. \ref{fig1}(b) and the predicted ratings can be obtained by employing the GDSRec.


\subsection{General Framework}
Generally, the original data (e.g. Fig. \ref{fig1}) can be treated as a bipartite graph, as the left side in Fig. \ref{fig2a}, in which users have relations with other users and interactions with items. However, directly learning from such graphs may lead to the misunderstanding of the real user preference. Considering that a low rating from a fastidious user may not denote a negative attitude on this item because the user tends to assign low ratings to all items. Such phenomenon is not uncommon. If we only use the original data to learn the representations of users and items, this bias may lead to sub-optimal solution. To alleviate the above issue due to these user behaviors, we believe the statistical information can be utilized to address the bias offsets of users and items. Motivated by this idea, the original bipartite graph can be processed as a decentralized graph, as shown on the right side of Fig. \ref{fig2a}. For each user-item interaction, we subtract it from the centralized mean average. Then, the decentralized graph is utilized to train our model. We will give more details in the follow. 

In Fig. \ref{fig2}, we show an overview of the proposed model. This model includes four components: user modeling, item modeling, social modeling and preference rating prediction. For the user modeling, its aim is to learn the latent factor offsets of the users. The function of the social modeling is similar to that of the user modeling. The difference between two modelings is that the user modeling only models one user while the social modeling needs to integrate the learning for the social relations of the user simultaneously. The item modeling is used to learn the latent factors of the items.


As mentioned before, we solve the rating prediction problem by exploiting the decentralized graph data consisting of the decentralized user-item graph and the social graph. It is intuitive to obtain the final predicted rating $\hat{r}_{ij}$ between the user $u_i$ and the item $v_j$, including three components: the average rating $E(u_i)$ of the user $u_i$, the average rating $E(v_j)$ of the item $v_j$, and the final preference rating between the user $u_i$ and the item $v_j$, i.e.,
\begin{equation}
\label{301}
\hat{r}_{ij} = \frac{1}{2}[E(u_i) + E(v_j)] + f(u_i, v_j),
\end{equation}
where $E(u_i)$ and $E(v_j)$ set the benchmark for the prediction, $f(u_i, v_j)$ computes the final preference rating between the user $u_i$ and the item $v_j$. The function $f(u_i, v_j)$ can be expressed as
\begin{equation}
\label{302}
f(u_i, v_j) = \frac{1}{2}\left(r_{ij}^p + \sum\limits_{u_k \in N(u_i)} \lambda_{ik}r_{kj}^p\right),
\end{equation}
with
\begin{equation}
\label{303}
\lambda_{ik} = \frac{T_{ik}}{\sum\limits_{u_k \in N(u_i)}T_{ik}},
\end{equation}
where $r_{ij}^p$ is the preference rating between the user $u_i$ and the item $v_j$. The final predicted preference rating can be understood to consist of the user's own opinions and references of his socially connected users' ratings.
Since it is easy to obtain $E(u_i)$ and $E(v_j)$ from the original data, the key problem is how to derive the preference rating $r_{ij}^p$ between the user $u_i$ and the item $v_j$. To this end, we utilize the decentralized user-item graph to learn the representations of the users and the items. These representations are called latent factor offsets, because the proposed model maps the users and the items into a latent factor space by exploiting the decentralized graph data. In order to obtain the latent factor offsets of the users and the items, different data are employed to accomplish different goals. With the example in Fig. \ref{fig1}, the items interacted with the user (i.e., item aggregation of $v_2$ and $v_4$) are utilized for learning the latent factor offset of the user $u_1$. For the latent factor offset of item $v_4$, it is learned from the users whom the item interacts with (i.e., user aggregation of $u_1$ and $u_2$). The social offsets of $u_1$ is learned by performing social 
aggregation between the users that $u_1$ is socially connected with (i.e., $u_2$ and $u_4$). The preference rating prediction component is to learn the model parameters via prediction by integrating the user, item and social modeling components. It should be noted that if there is a new user or item without interaction records, the average rating of this user or item can be replaced by the global average value. The details of these model components are discussed as follows.

\subsection{User Modeling}
In this subsection, we detail how to model the latent factor offset (denoted as $\mathbf{h}_{u_i} \in \mathbb{R}^D$) of the user $u_i$ from item aggregation.


It can be seen that the decentralized user-item graph contains the interactions history between the users and the items, and the users' ratings on these items. In \cite{FanMa19}, the authors provided an approach to capture the interactions and the ratings for learning the latent factor of the user $u_i$. However, this approach does not reflect the statistical difference between $u_i$ and other users. As a result, instead of using the rating directly, we exploit the rating difference $\bar{r}_{ij}$ in the user modeling, i.e.,
\begin{equation}
\label{baruserrij}
\bar{r}_{ij} =  \lceil|r_{ij} - E(v_j)|\rceil.
\end{equation}
We create an embedding lookup table to map each difference $\bar{r}_{ij}$ into the table and one can easily obtain the difference representation $\mathbf{s}_{\bar{r}_{ij}}$ in this table. The reason that we do not use $r_{ij} - E(v_j)$ directly is that it is not convenient to use the embedding method in codes due to decimals. We believe quantitative methods can be utilized to tackle this problem and we leave it for future works.

To get the latent factor offset $\mathbf{h}_{u_i}$ for the user $u_i$ mathematically, we use the following function as
\begin{equation}
\mathbf{h}_{u_i} = \text{Tanh}\left(\mathbf{W} \cdot G_I(\{\mathbf{x}_{il}, \forall v_l \in R(u_i)\}) + \mathbf{b}\right),
\end{equation}
where $\mathbf{x}_{il}$ is the representation vector denoting the rating-difference-aware interaction between the user $u_i$ and the item $v_l$, $G_I$ is the item aggregation function, $\mathbf{W}$ and $\mathbf{b}$ are the weight and bias of a neural network, respectively. The purpose of the rating-difference-aware interaction is to capture the users' preference differences, which can help us to model the users' latent factor offsets. This is different from directly obtaining users' preferences in the past \cite{BergKipf17,FanMa19}. 
For the interaction between the user $u_i$ and the item $v_l$ with the rating difference $\bar{r}_{il}$, we model this interaction representation $\mathbf{x}_{il}$ as
\begin{equation}
\mathbf{x}_{il} = L_U([\mathbf{q}_{v_l} \oplus \mathbf{s}_{\bar{r}_{il}}]),
\end{equation}
where $L_U$ is a Multi-Layer Perceptron (MLP). As mentioned in the introduction, this method treats the bias as a vector and fuses it into the process of learning the user representation. In this way, we could better capture bias hidden in user interaction records.

Consider that each interaction between one user and the interacted items contributes differently to the user's latent factor offset. Inspired by the attention mechanisms \cite{YangYang16,ChenZhang18}, we define the item aggregation function $G_I$ as
\begin{equation}
G_I(\{\mathbf{x}_{il}, \forall v_l \in R(u_i)\}) = \sum\limits_{v_l \in R(u_i)}\eta_{il}\mathbf{x}_{il},
\end{equation}
where $\eta_{il}$ is the attention weight of the interaction between the user $u_i$ and the item $v_l$. In this way, the model can better capture the differences in the users' preferences. The core problem is how to get the attention weight. We take the following attention network to solve it.

\subsubsection*{Attention Network}
The input of this network is the interaction representation $\mathbf{x}_{il}$ and the user $u_i$'s embedding vector $\mathbf{p}_{u_i}$. According to \cite{FanMa19}, we exploit a two-layer neural network,
\begin{equation}
\dot{\eta}_{il} = \mathbf{w}_2^ T \cdot \text{ReLU}\left(\mathbf{W}_1 \cdot [\mathbf{x}_{il} \oplus \mathbf{p}_{u_i}] + \mathbf{b}_1 \right) + b_2,
\end{equation}
where $\text{ReLU}$ is rectified linear unit. The attention weight $\eta_{il}$ is obtained by normalizing above attentive scores with Softmax function, i.e.,
\begin{equation}
\label{atteta}
\eta_{il} = \frac{\exp(\dot{\eta}_{il})}{\sum\limits_{v_l \in R(u_i)} \exp(\dot{\eta}_{il})}.
\end{equation}
Finally, the latent factor offset $\mathbf{h}_{u_i}$ for the user $u_i$ can be written as
\begin{equation}
\mathbf{h}_{u_i} = \text{Tanh}(\mathbf{W} \cdot \left\{\sum\limits_{v_l \in R(u_i)} \eta_{il}\mathbf{x}_{il} \right\}+ \mathbf{b}).
\end{equation}

\subsection{Item Modeling}
This part aims to learn the latent factor offset $\mathbf{h}_{v_j}$ of the item $v_j$ from the user aggregation in the decentralized user-item graph. The user aggregation contains all users who interact with the item $v_j$, as well as users' ratings on $v_j$. Different users may express different attitudes towards the same item. This can help us to characterize the item to some extent. In order to describe the different characteristics of the item on different users, we modify the way of using the rating utilized in the user modeling. A new rating difference $\bar{r}_{ij}$ between the user $u_i$ and the item $v_j$  is defined as
\begin{equation}
\label{tildeitemrij}
\tilde{r}_{ij} = \lceil|r_{ij} - E(u_i)|\rceil.
\end{equation}
Exploiting this type of rating difference, we use the model to learn the latent factor offset of one item from different users.
The following whole process is similar to the user modeling.
For the interaction between the user $u_k$ and the item $v_j$ with the rating difference $\tilde{r}_{kj}$, we present a rating-difference-aware interaction representation $\mathbf{y}_{jk}$ composed by the user embedding $\mathbf{p}_{u_k}$ and the rating difference embedding $\mathbf{s}_{\tilde{r}_{kj}}$, i.e.,
\begin{equation}
\mathbf{y}_{jk} = L_I([\mathbf{p}_{u_k} \oplus \mathbf{s}_{\tilde{r}_{kj}}]),
\end{equation}
where $L_I$ is a MLP same as $L_U$ and the method for getting $\mathbf{s}_{\tilde{r}_{kj}}$ is the same as for $\mathbf{s}_{\bar{r}_{ij}}$ in the user modeling. For learning the latent factor offset $\mathbf{h}_{v_j}$, we introduce the function
\begin{equation}
\mathbf{h}_{v_j} = \text{Tanh}(\mathbf{W} \cdot G_U(\left\{\mathbf{y}_{jk}, \forall u_k \in R(v_j)\right\}) + \mathbf{b}),
\end{equation}
where $G_U$ is the user aggregation function. After introducing the attention mechanism for differentiating the contributions of users' interactions to $\mathbf{y}_{jk}$, we have
\begin{equation}
G_U(\left\{\mathbf{y}_{jk}, \forall u_k \in R(v_j)\right\}) = \sum\limits_{u_k \in R(v_j)} \xi_{jk}\mathbf{y}_{jk},
\end{equation}
where $\xi_{jk}$ is the attention weight obtained by using a two-layer neural attention network taking $\mathbf{y}_{jk}$ and $\mathbf{q}_{v_j}$ as the input. It can be written as
\begin{equation}
\label{attxi}
\xi_{jk} = \frac{\exp(\dot{\xi}_{jk})}{\sum\limits_{u_k \in R(v_j)}\exp(\dot{\xi}_{jk})},
\end{equation}
with
\begin{equation}
\dot{\xi}_{jk} = \mathbf{w}_2^T \cdot \text{ReLU}(\mathbf{W}_1 \cdot [\mathbf{y}_{jk} \oplus \mathbf{q}_{v_j}] + \mathbf{b}_1) + b_2.
\end{equation}
Similar to $\mathbf{h}_{u_i}$, $\mathbf{h}_{v_j}$ can be expressed as
\begin{equation}
\mathbf{h}_{v_j} = \text{Tanh}(\mathbf{W} \cdot \left\{\sum\limits_{u_k \in R(v_j)} \xi_{jk}\mathbf{y}_{jk}\right\} + \mathbf{b}).
\end{equation}


\subsection{Social Modeling}
The function of the social modeling is similar to that of the user modeling. When the user modeling learns the latent factor offset of the user $u_i$, this social modeling aims to learn the latent factor offsets of $u_i$'s socially connected users. For example, in Fig. \ref{fig2}, when the user modeling learns the latent factor offset of the user $u_1$, the social modeling learns the latent factor offsets of $u_2$ and $u_4$ in the way the user modeling does, respectively. 
Hence, we can directly obtain $\{\mathbf{h}_{u_k}, \forall u_k \in N(u_i)\}$. It should be noted that in this module, data is still the decentralized graph data. The main purpose of this module is to help target users calibrate their ratings through their social users. When calculating the rating between a user and an item, the preference of socially connected users of this user is an important reference. It can help the model get more accurate ratings.




\subsection{Rating Prediction}
After acquiring the latent factor offsets $\mathbf{h}_{u_i}$, $\mathbf{h}_{v_j}$ and $\{\mathbf{h}_{u_k}, u_k \in N(u_i)\}$ of the user $u_i$, the item $v_j$ and $u_i$'s social-connected users, respectively, the preference rating can be obtained using a three-layer neural network. For the preference rating $r^p_{ij}$, we use the following process to obtain it,
\begin{align}
\mathbf{z}_1 &= \text{Tanh}(\mathbf{W}_1 \cdot [\mathbf{h}_{u_i} \oplus \mathbf{h}_{v_j}] + \mathbf{b}_2),\\
\mathbf{z}_2 &= \text{Tanh}(\mathbf{W}_2 \cdot \mathbf{z}_1 + \mathbf{b}_2),\\
r^p_{ij} &= \mathbf{w}^T \cdot \mathbf{z}_2.
\end{align}
For $u_i$'s social users, their preference ratings $\{r^p_{kj}, \forall u_k \in N(u_i)\}$ are derived in the same way. Then using the expressions in \eqref{301}--\eqref{303}, we can obtain the final rating prediction between the user $u_i$ and the item $v_j$. It should be noted that in the testing stage, the average ratings of users and items are consistent with that in the training stage.


\subsection{Model Training}
We evaluate our proposed model from two perspectives including rating prediction and ranking prediction.  
%To train our model, two objective functions need to be established for above two tasks respectively. 
For the task of rating prediction, there is a commonly used objective function
\begin{equation}
\mathcal{L}_1 = \frac{1}{2\langle\mathcal{O}\rangle} \sum\limits_{(u_i, v_j) \in \mathcal{O}}(\hat{r}_{ij} - r_{ij})^2,
\end{equation}
where $r_{ij}$ is a ground truth rating rated by user $u_i$ on item $v_j$.

Learning to rank focuses on providing the end-user a ranked list of items \cite{RafailidisCrestanires17} and is widespread in different kinds of recommendation scenarios, e.g., top-k recommendation, sequential recommendation \cite{RendleChristophuai09,ChenXuwsdm18}.
% the performance at the top positions of the list, with the recommended items that end-users will actually see \cite{RafailidisCrestanires17}. Ranking problems are widespread in different kinds of recommendation tasks, e.g., top-k recommendation, sequential recommendation \cite{RendleChristophuai09,ChenXuwsdm18}.
In this task, for each user, the interacted items are labeled as 1 (i.e., positive samples) if the rating is equal to or greater than $F$, or 0 (i.e., negative samples) if not. This is to say, the users would like to click on or browse the items with a rating equal to or greater than $F$. As the two datasets in our experiment contain ratings from 1 to 5, we set up two cases including $F=3$ and $F=4$ in our experiments. The output prediction scores of all models is adjusted using the sigmoid function. For the ranking task, we choose the binary cross-entropy loss as the objective function
\begin{equation}
\mathcal{L}_2 = \sum\limits_{(u_i, v_j) \in \mathcal{O}} y_{ij}\log(\hat{y}_{ij}) + (1-y_{ij})\log(1-\hat{y}_{ij}),
\end{equation}
where $y_{ij}$ is a ground truth label of a sample and $\hat{y}_{ij}$ is a value between $(0,1)$ as predicted by the model. 

In the optimization of the objective functions, we adopt the RMSprop \cite{HintonSrivastava12} as the optimizer. It randomly selects a training instance, and updates each model parameter along the negative gradient direction. All the embedding vectors are initialized randomly and learned during the stage of training. For the rating difference embedding, it depends on the rating scale. In our experiment, each rating is in $\{1,2,3,4,5\}$. Hence one can set the input dimension of the embedding to be 5. 

To reduce the influence of overfitting and improve generalization performance, we apply the dropout strategy \cite{Srivastava14}. In particular, we introduce a node dropout strategy.

\subsubsection*{Node dropout}
In the decentralized user-item graph and the social graph, each user or item has a different number of interactions. For example, one user may have interacted with a dozen items, but another may have only interacted with a few items. In order to prevent the overfitting impact of too many interactions on the representation learning, we need to reduce some interactions in the training stage.
Based on the above ideas, node dropout is presented. In \cite{BergKipf17}, the authors introduced a way of dropping out nodes with a probability. However, this approach was detrimental to the nodes with few interaction records. Hence, in the process of learning the latent factor offsets for the users and the items, we reserve up to $K$ interaction nodes for each node randomly, such that we can protect the node where the learning resources are few.

In the next section, we validate the performance of the proposed model on two real-world datasets.

\vspace{-0.2cm}
\subsection{Time Complexity}
As described in the section \ref{subsecproblem}, there are $N$ users, $M$ items and $\langle\mathcal{O}\rangle$ training samples. We use node dropout and reserve up to $K$ interaction nodes for each node. At each module, we need to calculate two MLPs with small layers (e.g., two-layers). Thus the time cost for three modeling modules is about $O((N+M)KD)$. For the rating prediction module, the time cost is about $O(\langle\mathcal{O}\rangle D)$. Therefore, the total time cost is about $O(((N+M)K+\langle\mathcal{O}\rangle)D)$. In practice, as $K \ll \{N, M\}$, thus the total time complexity is acceptable.




==> 4_experiments.tex <==
\vspace{-0.2cm}
\section{Experiment}
\label{sec4}
In this section, we conduct experiments to verify the effectiveness of the proposed GDSRec. We aim to answer the following research questions:

\textbf{RQ1:} How does GDSRec perform compared with existing methods, regarding both rating prediction and item ranking?
	
%\textbf{RQ2:} How does the negative sampling strategy affect the performance?

\textbf{RQ2:} How does the specific design of GDSRec affect the model performance? (i.e., ablation study)


\textbf{RQ3:} How does the node dropout strategy affect the model performance?

\textbf{RQ4:} How do the threshold $\delta$ affects the model performance?

% \vspace{-0.2cm}
\subsection{Dataset}
We evaluate our model on two benckmark datasets Ciao and Epinions\footnote{https://www.cse.msu.edu/\%7etangjili/trust.html}. They are taken from popular social networking websites. These two datasets contain users, items, ratings and social relations. The ratings are from 1 to 5. The statistics of Ciao and Epinions are shown in Table \ref{tabsta}.


\begin{center}
    \linespread{1.5}
    \begin{table}[]
    % \setlength{\abovecaptionskip} %缩小caption和图像之间的距离
    	\centering
    	\setlength{\belowcaptionskip}{0.2cm}
    	\caption{Statistics of the two datasets}\label{tabsta}
    	\rule{0pt}{15pt}
    	\begin{tabular}{c|c|c}
    		\hline  
    		Feature & Ciao & Epinions\\
    		\hline 
    		Users   & 7,317& 18,088\\
    		Items   & 10,4975& 261,649\\
    		Ratings & 283,319& 764,352\\
    % 		Density & 0.0368\%& 0.0161\%\\
    		\hline
    		Social Relations & 111,781 & 355,813\\
    % 		Density & 0.2087\% & 0.1087\%\\
    		\hline
    	\end{tabular}
    \end{table}
    % \vspace{-0.2cm}
\end{center}


\linespread{2}
\setlength{\tabcolsep}{1.1mm}{
% \usepackage{multirow}
% \usepackage[normalem]{ulem}
% \useunder{\uline}{\ul}{}
\begin{table*}[]
\setlength{\belowcaptionskip}{0.2cm}
\renewcommand{\arraystretch}{1}
\caption{Performance comparison of different recommender models}\label{tabres}
\begin{tabular}{|c|c|c|c|c|c|c|c|c|c|c|c|c|}
\hline
Training                        & Metrics & PMF    & FunkSVD & TrustMF & NeuMF  & DeepSoR & GCMC   & GCMC+SN & LightGCN & GraphRec     & Diffnet++    & GDSRec          \\ \hline
\multirow{2}{*}{Ciao(60\%)}     & MAE     & 0.9520 & 0.8462  & 0.7681  & 0.8251 & 0.7813  & 0.8157 & 0.7697  & 0.7715   & 0.7540       & \underline{0.7459} & \textbf{0.7328} \\ \cline{2-13} 
                                & RMSE    & 1.1967 & 1.0513  & 1.0543  & 1.0824 & 1.0437  & 1.0527 & 1.0225  & 1.0203   & 1.0093       & \underline{0.9987} & \textbf{0.9846} \\ \hline
\multirow{2}{*}{Ciao(80\%)}     & MAE     & 0.9021 & 0.8301  & 0.7690  & 0.8062 & 0.7739  & 0.8001 & 0.7526  & 0.7562   & \underline{0.7387} & 0.7398       & \textbf{0.7323} \\ \cline{2-13} 
                                & RMSE    & 1.1238 & 1.0515  & 1.0479  & 1.0617 & 1.0316  & 1.0323 & 0.9931  & 0.9963   & 0.9794       & \underline{0.9774} & \textbf{0.9740} \\ \hline
\multirow{2}{*}{Epinions(60\%)} & MAE     & 1.0211 & 0.9036  & 0.8550  & 0.9097 & 0.8520  & 0.8915 & 0.8602  & 0.8717   & 0.8441       & \underline{0.8435} & \textbf{0.8157} \\ \cline{2-13} 
                                & RMSE    & 1.2739 & 1.1431  & 1.1505  & 1.1645 & 1.1135  & 1.1258 & 1.1004  & 1.1103   & 1.0878       & \underline{1.0795} & \textbf{1.0685} \\ \hline
\multirow{2}{*}{Epinions(80\%)} & MAE     & 0.9952 & 0.8874  & 0.8410  & 0.9072 & 0.8383  & 0.8736 & 0.8590  & 0.8677   & \underline{0.8168} & 0.8201       & \textbf{0.8047} \\ \cline{2-13} 
                                & RMSE    & 1.2128 & 1.1422  & 1.1395  & 1.1476 & 1.0972  & 1.1052 & 1.0711  & 1.0801   & \underline{1.0631} & 1.0635       & \textbf{1.0566} \\ \hline
\end{tabular}
\end{table*}}

% \vspace{-1.5cm}
\subsection{Evaluation Metrics}
For evaluating the performance of the rating prediction of the proposed model, we adopt two well-known metrics, namely mean absolute error (MAE) and root mean square error (RMSE), to evaluate the predictive accuracy of the recommendation algorithms. The two metrics are defined as
\begin{align}
\text{MAE} = \frac{1}{\langle\mathcal{T}\rangle}\sum\limits_{u_i, v_j \in \mathcal{T}}|\hat{r}_{ij} - r_{ij}|,\\
\text{RMSE} = \sqrt{\frac{1}{\langle\mathcal{T}\rangle}\sum\limits_{u_i, v_j \in \mathcal{T}}(\hat{r}_{ij} - r_{ij})^2},
\end{align}
where $\mathcal{T}$ is the dataset of testing. Smaller values of MAE and RMSE indicate higher predictive accuracy.

In order to further validate the performance of the rating prediction, we extend it to item ranking evaluation. The testing set contains both positive (i.e., items whose score $\geq F$) and negative samples (items whose score $<F$). A ranked list of items in the testing set is assessed by using Recall and Normalized Discounted Cumulative Gain (NDCG) \cite{HeLiao17,WangHesigir19}. We compute Recall@5 by counting the number of positive samples contained in the top-5 positions of a ranked list. NDCG is a weighted version of Recall which assigns higher importance to the top positions in a list. Higher values of Recall and NDCG indicate better ranking performance. It should be noted that we only use the observed data to evaluate and do not rank all items in the item ranking evaluation. All the reported results are the average of five tests. 

% \vspace{-0.5cm}
\subsection{Baselines}
For comparison purposes, the following approaches are considered. We select four groups of representative methods including:
\begin{itemize}[leftmargin=*]
    \item Traditional recommendation algorithms: \textbf{PMF} \cite{MnihSalakhutdinov08}, it only uses rating information; \textbf{FunkSVD}\cite{koren2008factorization}, it considers user and item biases based on matrix factorization methods;
    \item Traditional social recommendation algorithm: \textbf{TrustMF} \cite{YangLei16}, which exploit social information on the basis of rating information;
    \item Deep neural 
    network based recommendation algorithms:
    \textbf{NeuMF} \cite{HeLiao17}, \textbf{DeepSoR} \cite{FanLi18}, which are classical deep and deep social recommendation, respectively.
    \item Graph neural network based recommendation algorithms:
    \textbf{GCMC}, \textbf{GCMC+SN} \cite{BergKipf17}, \textbf{GraphRec}\cite{FanMa19}, \textbf{LightGCN}\cite{he2020lightgcn} and \textbf{Diffnet++}\cite{wu2020diffnet++}.
\end{itemize}
%(1) traditional recommendation algorithms: \textbf{PMF} \cite{MnihSalakhutdinov08}, it only uses rating information; (2) traditional social recommendation algorithms: \textbf{SoRec} \cite{MaYang08}, \textbf{SoReg} \cite{MaZhou11}, \textbf{SocialMF} \cite{JamaliEster10} and \textbf{TrustMF} \cite{YangLei16}, these methods exploit social information on the basis of rating information; (3) deep neural network based recommendation algorithms: \textbf{NeuMF} \cite{HeLiao17}, \textbf{DeepSoR} \cite{FanLi18}, \textbf{GCMC+SN} \cite{BergKipf17}, \textbf{GraphRec} \cite{FanMa19}. 
% The baseline selection is the same with \cite{FanMa19}. Among the compared baselines, GraphRec is the state-of-the-art neural network-based social recommendation algorithm \cite{FanMa19}.

% \vspace{-0.5cm}
\subsection{Parameter Settings}
\label{paraset}
Our proposed model is implemented on the basis of Pytorch\footnote{http://pytorch.org/}. For two datasets, we select 80\% or 60\% as a training set to learn the parameters, and the rest are divided into a validation set and a testing set on average. This data split is consistent with \cite{FanMa19}. The validation set is used to tune hyper-parameters and the testing set is for the final performance comparisons. The threshold $\delta$ can be selected in $\{0,1,2,3\}$. We test the values of the embedding size $D$ in \{16, 32, 64, 128, 256, 512\}, and the interaction node reservation $K$ in \{5, 10, 15, 20\} on Ciao and \{15, 20, 25, 30\} on Epinions. The learning rate and the batch size are searched in \{$10^{-6}$, $10^{-5}$, $10^{-4}$, $5\times10^{-4}$\} and \{64, 128, 256\}, respectively. We stop the training if the sum of MAE and RMSE increases 10 successive epochs on the validation set. Model parameters and all the embedding vectors are initialized in default with a uniform distribution in Pytorch. For LightGCN\cite{he2020lightgcn} and Diffnet++\cite{wu2020diffnet++}, we adopt a setting of two-layer graph convolution. The hyper-parameters for these methods are tuned by grid search.

% \vspace{-0.5cm}
\subsection{Performance Comparison (RQ1)} 
% \vspace{-0.4cm}
\subsubsection{Rating prediction}
Table \ref{tabres} shows the performance comparison between different models for the task of rating prediction. Part of results of the compared methods are taken from \cite{FanMa19}.
%The rating prediction performance of the baseline algorithms are given in \cite{FanMa19} on Ciao and Epinions datasets, we show that in Table \ref{tabres}. The performance of our method GDSRec is given in the table at the same time. 
The values with underlines indicate the best performance between the baselines, to the best of our knowledge.
It can be seen from the table that FunkSVD outperforms PMF, which indicates that the user and item biases exist in practice. 
We can see that the traditional method TrustMF outperforms PMF and FunkSVD. When PMF and FunkSVD only use rating information, the traditional social recommender algorithm shows that the combination of rating and social information can effectively improve the recommendation performance. These results support that social network information can be leveraged when we solve the rating prediction problem using deep neural networks. 
 
NeuMF exploits neural network architecture to solve the problem, and it performs better than PMF. This shows the power of the neural network model in recommender algorithms. DeepSoR combines social information on the basis of the neural network, and performs better than NeuMF. In addition, comparing GCMC and GCMC+SN, the importance of social information also can be observed. 
LightGCN is the sate-of-the-art recommendation GNN-based model with implicit feedback, which models high-order user-item interaction but without exploiting social information. 
Generally, it outperforms GCMC but not as strong as GCMC+SN.
Both GraphRec and Diffnet++ take advantage of GNNs and combine them with the social network information for recommendations. These two approaches show that GNNs have good learning capabilities for representations. 
\begin{figure*}[]
% \setlength{\abovecaptionskip}{-0.00cm} %缩小caption和图像之间的距离
\centering
    \includegraphics[width=18cm]{Picture/ranking3.pdf}
	\caption{Performance of ranking on Ciao and Epinions datasets for $F=3$.}
	\label{figr6}
\end{figure*}
\begin{figure*}[]
\setlength{\abovecaptionskip}{-0.0cm} %缩小caption和图像之间的距离
	\centering
\includegraphics[width=18cm]{Picture/ranking4.pdf}
	\caption{Performance of ranking on Ciao and Epinions datasets for $F=4$.}
	\label{figr7}
\end{figure*}

From Table \ref{tabres} we can see that our model GDSRec outperforms all other baseline methods. Compared to GraphRec and Diffnet++, our model exploits the users and items statistics, which helps to obtain the rating prediction benchmarks. The preference rating prediction is then sought by learning the latent factor offsets of the users and the items. In addition, unlike GraphRec and Diffnet++ which use the social network information to learn the user representations, our model uses the social network information as a method of correcting the final rating prediction. When the training set accounts for 60\% of the dataset, it can be seen that our model has an average performance improvement of 1.75\% over Diffnet++. When the training data is 80\% of the dataset, our model can obtain more performance improvements. Although the percentage of relative improvements are small, Koren has pointed out in \cite{Koren08} that even small improvements in MAE and RMSE may lead to significant differences of recommendations in practice.

% \vspace{-0.4cm}
\subsubsection{Item ranking}
In this part, we evaluate the performance of item ranking for the proposed model. For comparison purpose, we select the traditional algorithm PMF and FunkSVD, the classical deep algorithm NeuMF, GNN-based models including LightGCN, GraphRec and Diffnet++ to compare with our GDSRec. 
The results are shown in Fig. \ref{figr6} and \ref{figr7}. From the figures we can see that the four models show similar and high performance on the Recall evaluation metric. This is because the positive label takes up a large proportion in the two datasets. The models' predictions are naturally biased and give positive results with high probabilities for negative samples. This makes it difficult to judge the performance of the models on the Recall. In contrast, the performance of the models on the NDCG is different. This demonstrates a difference in the ranking ability of the four models. In sum, the GDSRec performs better than other counterparts in terms of NDCG. It further demonstrates that our model is more effective to push the positive items to high ranking positions.%. Note that the GraphRec and GDSRec both exploit the explicit feedback (i.e., ratings) to learning the representation of users and items. It illustrates the importance of users having explicit preferences for recommender systems.


% \vspace{-0.5cm}
\subsection{Ablation Study (RQ2)}
In this subsection, we further investigate the impact of the model components of the proposed GDSRec.
\begin{figure*}[t]
\setlength{\abovecaptionskip}{-0.00cm} %缩小caption和图像之间的距离
	\centering
	\includegraphics[width=18cm]{Picture/variants.pdf}
	%
	\caption{Effect of social network and user ratings on Ciao and Epinions datasets.}
	\label{fig3}
\end{figure*}


\begin{figure}[!h]
\centering
\includegraphics[width=7.5cm]{Picture/hyper_alpha.pdf}
\caption{Effect of $\alpha$ on Ciao and Epinions datasets.}
\label{fig10}
\end{figure}
% \vspace{-0.5cm}

\begin{figure*}[t]
\setlength{\abovecaptionskip}{-0.00cm} %缩小caption和图像之间的距离
	\centering
\includegraphics[width=18cm]{Picture/dropout.pdf}
	\caption{Effect of node dropout on Ciao and Epinions datasets.}
	\label{fig5}
\end{figure*}
% \vspace{-0.5cm}

% \vspace{-0.5cm}
\subsubsection{Effect of Social Network and User Ratings}
The effectiveness of the proposed model is presented in this subsection. Our model incorporates three factors: 1) the addition of the relationship coefficient for the social relations; 2) using the social relations to adjust the rating prediction; 3) learning the latent factor offsets by employing the statistics of the users and the items. To better understand the proposed model, we make several variants of the model and compare the performance between them. These variants are defined as:
\begin{itemize}[leftmargin=*]
	
	\item GDSRec-RC: The relationship coefficients of the social relations are removed from the proposed framework. This variant implies that all social relationships are equal and undifferentiated. In other words, all relationship coefficients are 1.
	
	\item GDSRec-SN: The social network information of the GDSRec is removed. This variant ignores the preference rating prediction of the social relations, and only uses $\mathbf{h}_{u_i}$ and $\mathbf{h}_{v_j}$ to obtain $f(u_i, v_j)$, i.e., $f(u_i, v_j) = r^p_{ij}$.
	
	\item GDSRec-RD: The latent factor offsets are learned from the rating difference in our proposed framework. This variant means that the latent factor offsets are learned with original rating data, rather than the rating difference. In other words, the rating difference ($\bar r_{ij}$, $\tilde r_{ij}$) defined in \eqref{baruserrij} and \eqref{tildeitemrij} is replaced by $r_{ij}$. 
\end{itemize}
For simplicity, we conclude these variants in Table \ref{variantsofGDSRec}. In the following, we compare the performance of these variants with that of the GDSRec.

\begin{center}
\linespread{1.5}
    \begin{table}[h]
        \centering
        % \setlength{\abovecaptionskip}{0.1cm}
        \setlength{\belowcaptionskip}{0.2cm}
        \linespread{2}
        \caption{Modification of GDSRec}\label{variantsofGDSRec}
        \begin{tabular}{cc}
            \hline
            \multicolumn{2}{c}{Modification}                        \\ \hline
            \multicolumn{1}{c|}{GDSRec-RC} & \multicolumn{1}{c}{Eq. (\ref{303}) $\Rightarrow \lambda_{ik} = \frac{1}{\langle N(u_i) \rangle}$ } \\ \hline
            \multicolumn{1}{c|}{GDSRec-SN} & \multicolumn{1}{c}{Eq. (\ref{302}) $\Rightarrow f(u_i, v_j) = r^p_{ij} $ } \\ \hline
            \multicolumn{1}{c|}{GDSRec-RD} & \multicolumn{1}{c}{Eq. (\ref{baruserrij}) and (\ref{tildeitemrij}) $\Rightarrow  \bar{r}_{ij}, \tilde{r}_{ij} = r_{ij}$ } \\ \hline
        \end{tabular}
    \end{table}
\end{center}

The performance comparisons among the GDSRec and three variants regarding rating prediction are given in Fig. \ref{fig3}. The hyper-parameters in these models are set to be the same. From the results shown in the figure, we can conclude that:
\begin{itemize}[leftmargin=*]
	\item Impact of the Social Network: We now analyze the impact of the social network on the recommendation performance. First of all, we can see that the performance of the GDSRec-RC is slightly weaker than that of the GDSRec from the Fig. \ref{fig3}. Although the RMSE of the GDSRec-RC is similar to that of the GDSRec on Ciao, the MAE is 0.9\% higher than that of the GDSRec. For the dataset Epinions, it can be observed that while the MAE of the GDSRec-RC is close to that of the GDSRec, the RMSE of the GDSRec-RC is higher than that of the GDSRec. This verifies that the relationship coefficient is beneficial for the model. On the other hand, the RMSE of the GDSRec-SN is 0.79\% higher than that of the GDSRec while the MAE results of two models are close. This is to say, the social network is important for the recommendation performance.
	\item Impact of the Rating Difference: When we use the original rating data instead of the rating difference for training the latent factor offsets, we can see from Fig. \ref{fig3} that both MAE and RMSE of the GDSRec-RD on two datasets are much higher than that of the GDSRec. So the performance of the GDSRec-RD is much worse than that of the GDSRec. It validates that our core idea, processing on the original rating data, is very efficient, which helps to improve the performance of recommendation. We believe it can be applied directly to other models and lead to performance improvements, and we leave it for future works.
\end{itemize}


\linespread{1.5}
% \setlength{\abovecaptionskip}{1.0cm} %缩小caption和图像之间的距离
% 	\setlength{\tabcolsep}{2mm}{
\rule{0pt}{15pt}
\begin{table}[h]
\centering
    \setlength{\belowcaptionskip}{0.2cm}
	\caption{Effect of attention network on Ciao and Epinions datasets.}\label{tabatt}
	\begin{tabular}{|c|c|c|c|c|}
		\hline
		Training&Metrics&GDSRec-avg&GDSRec-max&GDSRec\\
		\hline
		{Ciao(60\%)} & MAE &0.7326 &0.7388 &0.7328 \\
		\cline{2-5}
		&RMSE &0.9871 &0.9884 &0.9846 \\
		
		
		\hline
		{Epinions(60\%)} & MAE &0.8155 &0.8183 &0.8157 \\
		\cline{2-5}
		&RMSE &1.0704 &1.0706 &1.0685 \\
		\cline{2-5}
		\hline
	\end{tabular}
\end{table}

% \vspace{-0.8cm}
\subsubsection{Effect of Attention Network}
In this subsection, the effectiveness of the attention network is evaluated. The proposed GDSRec use softmax to normalize the attention scores. %In our design, the attention weights are obtained by normalizing the attentive scores with Softmax function. 
Here, we design two variants of the attention weights. One variant is to rewrite \eqref{atteta} and \eqref{attxi} as
\begin{equation}
\begin{cases}
	\eta_{il} = \frac{1}{\langle R(u_i)\rangle},\\
	\xi_{jk} = \frac{1}{\langle R(v_j) \rangle},
\end{cases}
\end{equation}
respectively. The other is,
\begin{equation}
\label{attmax}
\begin{cases}
	\eta_{il} = \max\limits_{v_l \in R(u_i)}\left(\frac{\exp(\dot{\eta}_{il})}{\sum\limits_{v_l \in R(u_i)} \exp(\dot{\eta}_{il})}\right),\\
	\xi_{jk} = \max\limits_{u_k \in R(v_j)}\left(\frac{\exp(\dot{\xi}_{jk})}{\sum\limits_{u_k \in R(v_j)}\exp(\dot{\xi}_{jk})}\right).
\end{cases}
\end{equation}
We use GDSRec-avg and GDSRec-max to denote these two variants respectively. Note that there is no another variant similar to the GDSRec-max which replaces maximum of \eqref{attmax} with minimum. This is because it may result in the output of the attention network very small if there is a attention weight is close to zero.

The performance comparison regarding rating prediction is shown in Table \ref{tabatt}. We can observe that the GDSRec-avg achieves the same performance with the GDSRec on the MAE. The performance of the GDSRec-max is always the worst. We can put the GDSRec-avg and GDSRec-max in the same category as these two variants both have the same output weight for different input attention scores. We believe that the GDSRec-avg performs better than the GDSRec-max as the adjustment of the GDSRec-avg is more gentle. In summary, the GDSRec assigns different weights to users or items when learning the representations and therefore has better performance.


% \vspace{-0.3cm}
\subsubsection{Effect of Average Rating}
According to \eqref{301}, the final prediction depends on the average ratings (i.e., $E(u_i)$ and $E(v_j)$). Here we discuss what the performance will be if the average ratings are changed. Toward this end, we change the weight of the average ratings in the final prediction, the expression \eqref{301} is rewritten as
\begin{equation}
\label{401}
\hat{r}_{ij} =  \frac{\alpha}{2}[E(u_i) + E(v_j)] + f(u_i, v_j),    
\end{equation}
where $\alpha$ is a hyper-parameter. 

We test the values of $\alpha$ in \{0, 0.2, 0.4, 0.6, 0.8, 1, 1.2, 1.4, 1.6\} and give the results in Fig. \ref{fig10}. From the figure we can see that the performance degrades significantly as $\alpha$ decreases from 1 to 0. It's easy to explain that the model can be thought of as fitting the decentralized training data. Thus, once the average ratings changed, the final prediction loses this information directly. It inevitably leads to performance degradation. As $\alpha$ goes large, the performance relatively deteriorates. These results indicate the importance of users' personalized preferences in predicting.


% \vspace{-0.5cm}
\subsection{Effect of Node Dropout (RQ3)}
Now, we analyze the effect of the node dropout on the performance of recommendation. The node dropout is used to avoid overfitting problems caused by too many interactions for nodes. For a limited number $K$ of interaction nodes, we show the results in Fig. \ref{fig5}, where the training set accounts for 60\% of the dataset and $D=256$. On the dataset Ciao, the GDSRec achieves the best performance at $K=10$ when $K$ increases from 5 to 20. For the dataset Epinions, the results are somewhat different. As $K$ goes from 15 to 30, we can clearly see that both MAE and RMSE are minimal at $K=25$. It verifies that the interaction nodes number $K$ effects the performance of the proposed model. For a new dataset, a limited number of interaction nodes $K$ needs to be tested experimentally.



\linespread{1.5}
\begin{table}[]
\centering
\setlength{\belowcaptionskip}{0.2cm}
\caption{Effect of the threshold $\delta$ on Ciao and Epinions datasets.}\label{delta}
        \begin{tabular}{|c|c|c|c|c|c|}
        \hline
        Training                        & Metrics & $\delta=0$      & $\delta=1$      & $\delta=2$      & $\delta=3$      \\ \hline
        \multirow{2}{*}{Ciao(60\%)}     & MAE     & 0.7327 & 0.7328 & 0.7441 & 0.7446 \\ \cline{2-6} 
                                        & RMSE    & 0.9874 & 0.9846 & 0.9856 & 0.9879 \\ \hline
        \multirow{2}{*}{Epinions(60\%)} & MAE     & 0.8242 & 0.8157 & 0.8252 & 0.8271 \\ \cline{2-6} 
                                        & RMSE    & 1.0709 & 1.0685 & 1.0696 & 1.0726 \\ \hline
        \end{tabular}
\end{table}

% \vspace{-0.5cm}
\subsection{Effect of the Threshold $\delta$ (RQ4)}
In Table \ref{delta}, we give the results of the MAE and RMSE on two datasets for different $\delta$ thresholds. Generally, when $\delta$ is 1, the performance on Ciao and Epinions is the best. As $\delta=0$, the data of the social relation is very sparse. Therefore, it can not help the model to learn better. And as $\delta$ becomes larger than 1, it may introduce some noise into the social relation data and causes poor performance.


==> 5_conclusions.tex <==
\vspace{-0.5cm}
\section{Conclusions}
\label{sec5}
In this paper, we have proposed a novel framework GDSRec for the rating prediction problem in social recommendations. GDSRec treats rating biases as vectors and fuses them into the process of learning user and item representations. To the end, we have dealt with the original graph into the decentralized graph by utilizing the statistical information, and extracted bias information explicitly on the graph. It provides a decentralized perspective on learning the latent factor offsets for the users and the items. And the statistical information provides important benchmarks for the rating predictions. In addition, we have differentiated the explicit strengths of social relations for the users and added these strengths to the final predictions. Experiments on two real-world datasets have been conducted. The results have shown that our new method has better rating prediction performance than its counterparts. In addition, we have conducted experiments to verify the ability of ranking for the proposed model. To conclude, the proposed model achieves better performance on both rating prediction and item ranking.




==> Submit_ArXiv/abstract.tex <==



\begin{abstract}
The Electron-Ion Collider (EIC) is a cutting-edge accelerator facility that will study the nature of the ``glue'' that binds the building blocks of the visible matter in the universe. The proposed experiment will be realized at Brookhaven National Laboratory in approximately 10 years from now, with detector design and R\&D currently ongoing. 
%
Notably, EIC is one of the first large-scale facilities to leverage Artificial Intelligence (AI) %during the design and R\&D phases. 
 already starting from the design and R\&D phases. 
%The EIC Comprehensive Chromodynamics Experiment (ECCE) is a consortium that is proposing a detector design based on a 1.5T solenoid. Herein we describe a comprehensive optimization of the ECCE tracker using AI. 
The EIC Comprehensive Chromodynamics Experiment (ECCE) is a consortium that proposed a detector design based on a 1.5T solenoid. The EIC detector proposal review concluded that the ECCE design will serve as the reference design for an EIC detector. 
%
Herein we describe a comprehensive optimization of the ECCE tracker using AI. 
%
The work required a complex parametrization of the simulated detector system. % simulated with the Fun4All framework.  
%
Our approach dealt with an optimization problem in a multidimensional design space driven by multiple objectives that encode the detector performance, while satisfying several mechanical constraints. 
%
We describe our strategy and show results obtained for the ECCE tracking system. 
The AI-assisted design is agnostic to the simulation framework and can be extended to other sub-detectors or to a system of sub-detectors to further optimize the performance of the EIC detector.



\end{abstract}

==> Submit_ArXiv/authors/affiliations-test.tex <==
%
% Please fill in any missing information
%
%
% Example of the new format:
%
% \affiliation[]{organization={},
%	 addressline={},
%	 city={},
%	 postcode={},
%	 state={},
%	 country={}} 
%

\affiliation[AANL]{organization={A. Alikhanyan National Laboratory},
	 city={Yerevan},
	 country={Armenia}} 
 
\affiliation[AcademiaSinica]{organization={Institute of Physics, Academia Sinica},
	 city={Taipei},
	 country={Taiwan}} 
 
\affiliation[AUGIE]{organization={Augustana University},
	 addressline={},
	 city={Sioux Falls},
	 postcode={},
	 state={SD},
	 country={USA}} 
 
\affiliation[BNL]{organization={Brookhaven National Laboratory},
	 addressline={},
	 city={Upton},
	 postcode={11973},
	 state={NY},
	 country={USA}} 
 
\affiliation[BrunelUniversity]{organization={Brunel University London},
	 addressline={},
	 city={Uxbridge},
	 postcode={},
	 country={UK}} 
 
\affiliation[CanisiusCollege]{organization={Canisius College},
	 addressline={},
	 city={Buffalo},
	 postcode={},
	 state={NY},
	 country={USA}} 
 
\affiliation[CCNU]{organization={Central China Normal University},
	 city={Wuhan},
	 country={China}} 
 
\affiliation[Charles]{organization={Charles University},
	 city={Prague},
	 country={Czech Republic}} 
 
\affiliation[CIAE]{organization={China Institute of Atomic Energy, Fangshan},
	 city={Beijing},
	 country={China}} 
 
\affiliation[CNU]{organization={Christopher Newport University},
	 addressline={},
	 city={Newport News},
	 postcode={},
	 state={VA},
	 country={USA}} 
 
\affiliation[Columbia]{organization={Columbia University},
	 addressline={},
	 city={New York},
	 postcode={},
	 state={NY},
	 country={USA}} 
 
\affiliation[CUA]{organization={Catholic University of America},
	 addressline={620 Michigan Ave.},
	 city={Washington DC},
	 postcode={20064},
	 country={USA}} 
 
\affiliation[CzechTechUniv]{organization={Czech Technical University},
	 addressline={},
	 city={Prague},
	 country={Czech Republic}} 
 
\affiliation[Duquesne]{organization={Duquesne University},
	 addressline={},
	 city={Pittsburgh},
	 postcode={},
	 state={PA},
	 country={USA}} 
 
\affiliation[Duke]{organization={Duke University},
	 addressline={},
	 city={},
	 postcode={},
	 state={NC},
	 country={USA}} 
 
\affiliation[FIU]{organization={Florida International University},
	 addressline={},
	 city={Miami},
	 postcode={},
	 state={FL},
	 country={USA}} 
 
\affiliation[GeorgiaState]{organization={Georgia State University},
	 addressline={},
	 city={Atlanta},
	 postcode={},
	 state={GA},
	 country={USA}} 
 
\affiliation[Glasgow]{organization={University of Glasgow},
	 addressline={},
	 city={Glasgow},
	 postcode={},
	 country={UK}} 
 
\affiliation[GSI]{organization={GSI Helmholtzzentrum fuer Schwerionenforschung},
	 addressline={},
	 city={Darmstadt},
	 postcode={},
	 country={Germany}} 
 
\affiliation[GWU]{organization={The George Washington University},
	 addressline={},
	 city={Washington, DC},
	 postcode={},
	 country={USA}} 
 
\affiliation[Hampton]{organization={Hampton University},
	 addressline={},
	 city={Hampton},
	 postcode={},
	 state={VA},
	 country={USA}} 
 
\affiliation[HUJI]{organization={Hebrew University},
	 addressline={},
	 city={Jerusalem},
	 postcode={},
	 country={Isreal}} 
 
\affiliation[IMP]{organization={Chinese Academy of Sciences},
	 addressline={},
	 city={Lanzhou},
	 postcode={},
	 state={},
	 country={China}} 
 
\affiliation[IowaState]{organization={Iowa State University},
	 addressline={},
	 city={},
	 postcode={},
	 state={IA},
	 country={USA}} 
 
\affiliation[JazanUniversity]{organization={Jazan University},
	 city={Jazan},
	 country={Sadui Arabia}} 
 
\affiliation[JLab]{organization={Thomas Jefferson National Accelerator Facility},
	 addressline={12000 Jefferson Ave.},
	 city={Newport News},
	 postcode={24450},
	 state={VA},
	 country={USA}} 
 
\affiliation[JMU]{organization={James Madison University},
	 addressline={},
	 city={},
	 postcode={},
	 state={VA},
	 country={USA}} 
 
\affiliation[KobeUniversity]{organization={Kobe University},
	 city={Kobe},
	 country={Japan}} 
 
\affiliation[Kyungpook]{organization={Kyungpook National University},
	 city={Daegu},
	 country={Republic of Korea}} 
 
\affiliation[LANL]{organization={Los Alamos National Laboratory},
	 addressline={},
	 city={},
	 postcode={},
	 state={NM},
	 country={USA}} 
 
\affiliation[LBNL]{organization={Lawrence Berkeley National Lab},
	 addressline={},
	 city={Berkeley},
	 postcode={},
	 state={},
	 country={USA}} 
 
\affiliation[LehighUniversity]{organization={Lehigh University},
	 addressline={},
	 city={Bethlehem},
	 postcode={},
	 state={PA},
	 country={USA}} 
 
\affiliation[LLNL]{organization={Lawrence Livermore National Laboratory},
	 addressline={},
	 city={Livermore},
	 postcode={},
	 state={CA},
	 country={USA}} 
 
\affiliation[MoreheadState]{organization={Morehead State University, Morehad, KY, USA},
	 addressline={},
	 city={Morehead},
	 postcode={},
	 state={KY},
	 country={USA}} 
 
\affiliation[MIT]{organization={Massachusetts Institute of Technology},
	 addressline={77 Massachusetts Ave.},
	 city={Cambridge},
	 postcode={02139},
	 state={MA},
	 country={USA}} 
 
\affiliation[MSU]{organization={Mississippi State University},
	 addressline={},
	 city={Mississippi State},
	 postcode={},
	 state={MS},
	 country={USA}} 
 
\affiliation[NCKU]{organization={ National Cheng Kung University, Tainan, Taiwan},
	 addressline={},
	 city={},
	 postcode={},
	 state={},
	 country={}} 
 
\affiliation[NCU]{organization={National Central University},
	 city={Chungli},
	 country={Taiwan}} 
 
\affiliation[Nihon]{organization={Nihon University},
	 city={Tokyo},
	 country={Japan}} 
 
\affiliation[NMSU]{organization={New Mexico State University},
	 addressline={},
	 city={Las Cruces},
	 postcode={},
	 state={NM},
	 country={USA}} 
 
\affiliation[NRNUMEPhI]{organization={National Research Nuclear University MEPhI},
	 city={Moscow},
	 country={Russian Federation}} 
 
\affiliation[NRCN]{organization={Nuclear Research Center - Negev},
	 city={Beer-Sheva},
	 country={Isreal}} 
 
\affiliation[NTHU]{organization={National Tsing Hua University},
	 city={Hsinchu},
	 country={Taiwan}} 
 
\affiliation[NTU]{organization={National Taiwan University},
	 city={Taipei},
	 country={Taiwan}} 
 
\affiliation[ODU]{organization={Old Dominion University},
	 addressline={},
	 city={Norfolk},
	 postcode={},
	 state={VA},
	 country={USA}} 
 
\affiliation[Ohio]{organization={Ohio University},
	 addressline={},
	 city={Athens},
	 postcode={},
	 state={OH},
	 country={USA}} 
 
\affiliation[ORNL]{organization={Oak Ridge National Laboratory},
	 addressline={PO Box 2008},
	 city={Oak Ridge},
	 postcode={37831},
	 state={TN},
	 country={USA}} 
 
\affiliation[PNNL]{organization={Pacific Northwest National Laboratory},
	 addressline={},
	 city={Richland},
	 postcode={},
	 state={WA},
	 country={USA}} 
 
\affiliation[Pusan]{organization={Pusan National Univeristy, Busan, Republic of Korea},
	 addressline={},
	 city={},
	 postcode={},
	 state={},
	 country={}} 
 
\affiliation[Rice]{organization={Rice University, Houston, TX, USA},
	 addressline={},
	 city={},
	 postcode={},
	 state={},
	 country={}} 
 
\affiliation[RIKEN]{organization={RIKEN Nishina Center, Wako, Saitama, Japan},
	 addressline={},
	 city={},
	 postcode={},
	 state={},
	 country={}} 
 
\affiliation[Rutgers]{organization={ The State University of New Jersey, Department of Physics and Astronomy, Piscataway, NJ, USA},
	 addressline={},
	 city={},
	 postcode={},
	 state={},
	 country={}} 
 
 
\affiliation[CFNS]{organization={Center for Frontiers in Nuclear Science},
	 addressline={Stony Brook Univeristy},
	 city={Stony Brook},
	 postcode={},
	 state={NY},
	 country={USA}} 
 
\affiliation[StonyBrook]{organization={ Department of Physics and Astronomy, Stony Brook University, Stony Brook, NY, USA},
	 addressline={},
	 city={},
	 postcode={},
	 state={},
	 country={}} 
 
\affiliation[RBRC]{organization={ RIKEN BNL Research Center, Brookhaven National Laboratory, , NY, USA},
	 addressline={},
	 city={},
	 postcode={},
	 state={},
	 country={}} 
 
\affiliation[SCNU]{organization={PLACEHOLDER INSTITUE},
	 addressline={},
	 city={},
	 postcode={},
	 state={},
	 country={}} 
 
\affiliation[Seoul]{organization={ Seoul National University, Seoul, Republic of Korea},
	 addressline={},
	 city={},
	 postcode={},
	 state={},
	 country={}} 
 
\affiliation[Sejong]{organization={ Sejong University, Seoul, Republic of Korea},
	 addressline={},
	 city={},
	 postcode={},
	 state={},
	 country={}} 
 
\affiliation[Shinshu]{organization={ Shinshu University, Matsumoto, Nagano, Japan},
	 addressline={},
	 city={},
	 postcode={},
	 state={},
	 country={}} 
 
\affiliation[Sungkyunkwan]{organization={ Sungkyunkwan University, Suwon, Republic of Korea},
	 addressline={},
	 city={},
	 postcode={},
	 state={},
	 country={}} 
 
\affiliation[TAU]{organization={PLACEHOLDER INSTITUE},
	 addressline={},
	 city={},
	 postcode={},
	 state={},
	 country={}} 
 
\affiliation[Tokyo]{organization={PLACEHOLDER INSTITUE},
	 addressline={},
	 city={},
	 postcode={},
	 state={},
	 country={}} 
 
\affiliation[Tsinghua]{organization={ Tsinghua University, Beijing, China},
	 addressline={},
	 city={},
	 postcode={},
	 state={},
	 country={}} 
 
\affiliation[Tsukuba]{organization={ Tsukuba University of Technology, Tsukuba, Ibaraki, Japan.},
	 addressline={},
	 city={},
	 postcode={},
	 state={},
	 country={}} 
 
\affiliation[CUBoulder]{organization={ University of Colorado Boulder, Boulder, CO, USA},
	 addressline={},
	 city={},
	 postcode={},
	 state={},
	 country={}} 
 
\affiliation[UCAD]{organization={PLACEHOLDER INSTITUE},
	 addressline={},
	 city={},
	 postcode={},
	 state={},
	 country={}} 
 
\affiliation[UConn]{organization={ University of Connecticut, Storrs, CT, USA},
	 addressline={},
	 city={},
	 postcode={},
	 state={},
	 country={}} 
 
\affiliation[UH]{organization={ University of Houston, Houston, TX, USA},
	 addressline={},
	 city={},
	 postcode={},
	 state={},
	 country={}} 
 
\affiliation[UIUC]{organization={ University of Illinois, Urbana, IL, USA},
	 addressline={},
	 city={},
	 postcode={},
	 state={},
	 country={}} 
 
\affiliation[UKansas]{organization={PLACEHOLDER INSTITUE},
	 addressline={},
	 city={},
	 postcode={},
	 state={},
	 country={}} 
 
\affiliation[UKY]{organization={PLACEHOLDER INSTITUE},
	 addressline={},
	 city={},
	 postcode={},
	 state={},
	 country={}} 
 
\affiliation[Ljubljana]{organization={ Faculty of Mathematics and Physics, University of Ljubljana, Ljubljana, Slovenia},
	 addressline={},
	 city={},
	 postcode={},
	 state={},
	 country={}} 
 
\affiliation[NorthernGeorgia]{organization={PLACEHOLDER INSTITUE},
	 addressline={},
	 city={},
	 postcode={},
	 state={},
	 country={}} 
 
\affiliation[NewHampshire]{organization={ University of New Hampshire, Durham, NH, USA},
	 addressline={},
	 city={},
	 postcode={},
	 state={},
	 country={}} 
 
\affiliation[Oslo]{organization={ Department of Physics, University of Oslo, Norway},
	 addressline={},
	 city={},
	 postcode={},
	 state={},
	 country={}} 
 
\affiliation[Regina]{organization={ University of Regina, Regina, SK, Canada},
	 addressline={},
	 city={},
	 postcode={},
	 state={},
	 country={}} 
 
\affiliation[USeoul]{organization={ University of Seoul, Seoul, Republic of Korea},
	 addressline={},
	 city={},
	 postcode={},
	 state={},
	 country={}} 
 
\affiliation[USTC]{organization={PLACEHOLDER INSTITUE},
	 addressline={},
	 city={},
	 postcode={},
	 state={},
	 country={}} 
 
\affiliation[UTAustin]{organization={PLACEHOLDER INSTITUE},
	 addressline={},
	 city={},
	 postcode={},
	 state={},
	 country={}} 
 
\affiliation[UTsukuba]{organization={ University of Tsukuba, Tsukuba, Japan},
	 addressline={},
	 city={},
	 postcode={},
	 state={},
	 country={}} 
 
\affiliation[UTK]{organization={ University of Tennessee, Knoxville, TN, USA},
	 addressline={},
	 city={},
	 postcode={},
	 state={},
	 country={}} 
 
\affiliation[UTSM]{organization={PLACEHOLDER INSTITUE},
	 addressline={},
	 city={},
	 postcode={},
	 state={},
	 country={}} 
 
\affiliation[UVA]{organization={ University of Virginia, Charlottesville, VA, USA},
	 addressline={},
	 city={},
	 postcode={},
	 state={},
	 country={}} 
 
\affiliation[Vanderbilt]{organization={ Department of Physics and Astronomy, Vanderbilt University, Nashville, TN, USA},
	 addressline={},
	 city={},
	 postcode={},
	 state={},
	 country={}} 
 
\affiliation[VirginiaTech]{organization={PLACEHOLDER INSTITUE},
	 addressline={},
	 city={},
	 postcode={},
	 state={},
	 country={}} 
 
\affiliation[VirginiaUnion]{organization={ Virginia Union University, Richmond, VA, USA},
	 addressline={},
	 city={},
	 postcode={},
	 state={},
	 country={}} 
 
\affiliation[WayneState]{organization={ Wayne State University, Detroit, MI, USA},
	 addressline={},
	 city={},
	 postcode={},
	 state={},
	 country={}} 
 
\affiliation[WI]{organization={ Department of Particle Physics and Astrophysics, Weizmann Institute of Science, Rehovot, Israel},
	 addressline={},
	 city={},
	 postcode={},
	 state={},
	 country={}} 
 
\affiliation[WandM]{organization={ William and Mary, Williamsburg, VA, USA},
	 addressline={},
	 city={},
	 postcode={},
	 state={},
	 country={}} 
 
\affiliation[Yamagata]{organization={ Faculty of Science, Yamagata University, Yamagata, Japan},
	 addressline={},
	 city={},
	 postcode={},
	 state={},
	 country={}} 
 
\affiliation[Yarmouk]{organization={PLACEHOLDER INSTITUE},
	 addressline={},
	 city={},
	 postcode={},
	 state={},
	 country={}} 
 
\affiliation[Yonsei]{organization={Yonsei University},
	 city={Seoul},
	 country={Republic of Korea}} 
 
\affiliation[York]{organization={University of York},
	 city={York},
	 country={UK}} 
 
\affiliation[Zagreb]{organization={University of Zagreb},
	 city={Zagreb},
	 country={Croatia}} 
 


==> Submit_ArXiv/authors/affiliations.tex <==
%
% Full ECCE author list
% Click Refresh to get the latest version
%
% Goto the following to edit:
% https://www.overleaf.com/1234763137gmqgnzsrpsdj


%
% Please fill in any missing information
%
%
% Example of the format:
%
% \affiliation[]{organization={},
%	 addressline={},
%	 city={},
%	 postcode={},
%	 state={},
%	 country={}} 
%

\affiliation[AANL]{organization={A. Alikhanyan National Laboratory},
	 city={Yerevan},
	 country={Armenia}} 
 
\affiliation[AcademiaSinica]{organization={Institute of Physics, Academia Sinica},
	 city={Taipei},
	 country={Taiwan}} 
 
\affiliation[AUGIE]{organization={Augustana University},
	 city={Sioux Falls},
	 postcode={},
	 state={SD},
	 country={USA}} 
 
\affiliation[BNL]{organization={Brookhaven National Laboratory},
	 city={Upton},
	 postcode={11973},
	 state={NY},
	 country={USA}} 
 
\affiliation[BrunelUniversity]{organization={Brunel University London},
	 city={Uxbridge},
	 postcode={},
	 country={UK}} 
 
\affiliation[CanisiusCollege]{organization={Canisius College},
	 addressline={2001 Main St.},
	 city={Buffalo},
	 postcode={14208},
	 state={NY},
	 country={USA}} 
 
\affiliation[CCNU]{organization={Central China Normal University},
	 city={Wuhan},
	 country={China}} 
 
\affiliation[Charles]{organization={Charles University},
	 city={Prague},
	 country={Czech Republic}} 
 
\affiliation[CIAE]{organization={China Institute of Atomic Energy, Fangshan},
	 city={Beijing},
	 country={China}} 
 
\affiliation[CNU]{organization={Christopher Newport University},
	 city={Newport News},
	 postcode={},
	 state={VA},
	 country={USA}} 
 
\affiliation[Columbia]{organization={Columbia University},
	 city={New York},
	 postcode={},
	 state={NY},
	 country={USA}} 
 
\affiliation[CUA]{organization={Catholic University of America},
	 addressline={620 Michigan Ave. NE},
	 city={Washington DC},
	 postcode={20064},
	 country={USA}} 
 
\affiliation[CzechTechUniv]{organization={Czech Technical University},
	 city={Prague},
	 country={Czech Republic}} 
 
\affiliation[Duquesne]{organization={Duquesne University},
	 city={Pittsburgh},
	 postcode={},
	 state={PA},
	 country={USA}} 
 
\affiliation[Duke]{organization={Duke University},
	 city={},
	 postcode={},
	 state={NC},
	 country={USA}} 
 
\affiliation[FIU]{organization={Florida International University},
	 city={Miami},
	 postcode={},
	 state={FL},
	 country={USA}} 
 
\affiliation[GeorgiaState]{organization={Georgia State University},
	 city={Atlanta},
	 postcode={},
	 state={GA},
	 country={USA}} 
 
\affiliation[Glasgow]{organization={University of Glasgow},
	 city={Glasgow},
	 postcode={},
	 country={UK}} 
 
\affiliation[GSI]{organization={GSI Helmholtzzentrum fuer Schwerionenforschung},
	 addressline={Planckstrasse 1},
	 city={Darmstadt},
	 postcode={64291},
	 country={Germany}} 
 
\affiliation[GWU]{organization={The George Washington University},
	 city={Washington, DC},
	 postcode={20052},
	 country={USA}} 
 
\affiliation[Hampton]{organization={Hampton University},
	 city={Hampton},
	 postcode={},
	 state={VA},
	 country={USA}} 
 
\affiliation[HUJI]{organization={Hebrew University},
	 city={Jerusalem},
	 postcode={},
	 country={Isreal}} 
 
\affiliation[IJCLabOrsay]{organization={Universite Paris-Saclay, CNRS/IN2P3, IJCLab},
	 city={Orsay},
	 country={France}} 
	 
\affiliation[CEA]{organization={IRFU, CEA, Universite Paris-Saclay},
     cite= {Gif-sur-Yvette},
     country={France}
}


\affiliation[IMP]{organization={Chinese Academy of Sciences},
	 city={Lanzhou},
	 postcode={},
	 state={},
	 country={China}} 
 
\affiliation[IowaState]{organization={Iowa State University},
	 city={},
	 postcode={},
	 state={IA},
	 country={USA}} 
 
\affiliation[JazanUniversity]{organization={Jazan University},
	 city={Jazan},
	 country={Sadui Arabia}} 
 
\affiliation[JLab]{organization={Thomas Jefferson National Accelerator Facility},
	 addressline={12000 Jefferson Ave.},
	 city={Newport News},
	 postcode={24450},
	 state={VA},
	 country={USA}} 
 
\affiliation[JMU]{organization={James Madison University},
	 city={},
	 postcode={},
	 state={VA},
	 country={USA}} 
 
\affiliation[KobeUniversity]{organization={Kobe University},
	 city={Kobe},
	 country={Japan}} 
 
\affiliation[Kyungpook]{organization={Kyungpook National University},
	 city={Daegu},
	 country={Republic of Korea}} 
 
\affiliation[LANL]{organization={Los Alamos National Laboratory},
	 city={},
	 postcode={},
	 state={NM},
	 country={USA}} 
 
\affiliation[LBNL]{organization={Lawrence Berkeley National Lab},
	 city={Berkeley},
	 postcode={},
	 state={},
	 country={USA}} 
 
\affiliation[LehighUniversity]{organization={Lehigh University},
	 city={Bethlehem},
	 postcode={},
	 state={PA},
	 country={USA}} 
 
\affiliation[LLNL]{organization={Lawrence Livermore National Laboratory},
	 city={Livermore},
	 postcode={},
	 state={CA},
	 country={USA}} 
 
\affiliation[MoreheadState]{organization={Morehead State University},
	 city={Morehead},
	 postcode={},
	 state={KY},
	 }
 
\affiliation[MIT]{organization={Massachusetts Institute of Technology},
	 addressline={77 Massachusetts Ave.},
	 city={Cambridge},
	 postcode={02139},
	 state={MA},
	 country={USA}} 
 
\affiliation[MSU]{organization={Mississippi State University},
	 city={Mississippi State},
	 postcode={},
	 state={MS},
	 country={USA}} 
 
\affiliation[NCKU]{organization={National Cheng Kung University},
	 city={Tainan},
	 postcode={},
	 country={Taiwan}} 
 
\affiliation[NCU]{organization={National Central University},
	 city={Chungli},
	 country={Taiwan}} 
 
\affiliation[Nihon]{organization={Nihon University},
	 city={Tokyo},
	 country={Japan}} 
 
\affiliation[NMSU]{organization={New Mexico State University},
	 addressline={Physics Department},
	 city={Las Cruces},
	 state={NM},
	 postcode={88003},
	 country={USA}} 
 
\affiliation[NRNUMEPhI]{organization={National Research Nuclear University MEPhI},
	 city={Moscow},
	 postcode={115409},
	 country={Russian Federation}} 
 
\affiliation[NRCN]{organization={Nuclear Research Center - Negev},
	 city={Beer-Sheva},
	 country={Isreal}} 
 
\affiliation[NTHU]{organization={National Tsing Hua University},
	 city={Hsinchu},
	 country={Taiwan}} 
 
\affiliation[NTU]{organization={National Taiwan University},
	 city={Taipei},
	 country={Taiwan}} 
 
\affiliation[ODU]{organization={Old Dominion University},
	 city={Norfolk},
	 postcode={},
	 state={VA},
	 country={USA}} 
 
\affiliation[Ohio]{organization={Ohio University},
	 city={Athens},
	 postcode={45701},
	 state={OH},
	 country={USA}} 
 
\affiliation[ORNL]{organization={Oak Ridge National Laboratory},
	 addressline={PO Box 2008},
	 city={Oak Ridge},
	 postcode={37831},
	 state={TN},
	 country={USA}} 
 
\affiliation[PNNL]{organization={Pacific Northwest National Laboratory},
	 city={Richland},
	 postcode={},
	 state={WA},
	 country={USA}} 
 
\affiliation[Pusan]{organization={Pusan National University},
	 city={Busan},
	 country={Republic of Korea}} 
 
\affiliation[Rice]{organization={Rice University},
	 addressline={}P.O. Box 1892,
	 city={Houston},
	 postcode={77251},
	 state={TX},
	 country={USA}} 
 
\affiliation[RIKEN]{organization={RIKEN Nishina Center},
	 city={Wako},
	 state={Saitama},
	 country={Japan}} 
 
\affiliation[Rutgers]{organization={The State University of New Jersey},
	 city={Piscataway},
	 postcode={},
	 state={NJ},
	 country={USA}} 
 
 
\affiliation[CFNS]{organization={Center for Frontiers in Nuclear Science},
	 city={Stony Brook},
	 postcode={11794},
	 state={NY},
	 country={USA}} 
 
\affiliation[StonyBrook]{organization={Stony Brook University},
	 addressline={100 Nicolls Rd.},
	 city={Stony Brook},
	 postcode={11794},
	 state={NY},
	 country={USA}} 
 
\affiliation[RBRC]{organization={RIKEN BNL Research Center},
	 city={Upton},
	 postcode={11973},
	 state={NY},
	 country={USA}} 
\affiliation[Seoul]{organization={Seoul National University},
	 city={Seoul},
	 country={Republic of Korea}} 
 
\affiliation[Sejong]{organization={Sejong University},
	 city={Seoul},
	 country={Republic of Korea}} 
 
\affiliation[Shinshu]{organization={Shinshu University},
         city={Matsumoto},
	 state={Nagano},
	 country={Japan}} 
 
\affiliation[Sungkyunkwan]{organization={Sungkyunkwan University},
	 city={Suwon},
	 country={Republic of Korea}} 
 
\affiliation[TAU]{organization={Tel Aviv University},
	 addressline={P.O. Box 39040},
	 city={Tel Aviv},
	 postcode={6997801},
	 country={Israel}} 

\affiliation[Tsinghua]{organization={Tsinghua University},
	 city={Beijing},
	 country={China}} 
 
\affiliation[Tsukuba]{organization={Tsukuba University of Technology},
	 city={Tsukuba},
	 state={Ibaraki},
	 country={Japan}} 
 
\affiliation[CUBoulder]{organization={University of Colorado Boulder},
	 city={Boulder},
	 postcode={80309},
	 state={CO},
	 country={USA}} 
 
\affiliation[UConn]{organization={University of Connecticut},
	 city={Storrs},
	 postcode={},
	 state={CT},
	 country={USA}} 
 
\affiliation[UH]{organization={University of Houston},
	 city={Houston},
	 postcode={},
	 state={TX},
	 country={USA}} 
 
\affiliation[UIUC]{organization={University of Illinois}, 
	 city={Urbana},
	 postcode={},
	 state={IL},
	 country={USA}} 
 
\affiliation[UKansas]{organization={Unviersity of Kansas},
	 addressline={1450 Jayhawk Blvd.},
	 city={Lawrence},
	 postcode={66045},
	 state={KS},
	 country={USA}} 
 
\affiliation[UKY]{organization={University of Kentucky},
	 city={Lexington},
	 postcode={40506},
	 state={KY},
	 country={USA}} 
 
\affiliation[Ljubljana]{organization={University of Ljubljana, Ljubljana, Slovenia},
	 city={Ljubljana},
	 postcode={},
	 state={},
	 country={Slovenia}} 
 
\affiliation[NewHampshire]{organization={University of New Hampshire},
	 city={Durham},
	 postcode={},
	 state={NH},
	 country={USA}} 
 
\affiliation[Oslo]{organization={University of Oslo},
	 city={Oslo},
	 country={Norway}} 
 
\affiliation[Regina]{organization={ University of Regina},
	 city={Regina},
	 postcode={},
	 state={SK},
	 country={Canada}} 
 
\affiliation[USeoul]{organization={University of Seoul},
	 city={Seoul},
	 country={Republic of Korea}} 
 
\affiliation[UTsukuba]{organization={University of Tsukuba},
	 city={Tsukuba},
	 country={Japan}} 
 
\affiliation[UTK]{organization={University of Tennessee},
	 city={Knoxville},
	 postcode={37996},
	 state={TN},
	 country={USA}} 
 
\affiliation[UVA]{organization={University of Virginia},
	 city={Charlottesville},
	 postcode={},
	 state={VA},
	 country={USA}} 
 
\affiliation[Vanderbilt]{organization={Vanderbilt University},
	 addressline={PMB 401807,2301 Vanderbilt Place},
	 city={Nashville},
	 postcode={37235},
	 state={TN},
	 country={USA}} 
 
\affiliation[VirginiaTech]{organization={Virginia Tech},
	 city={Blacksburg},
	 postcode={},
	 state={VA},
	 country={USA}} 
 
\affiliation[VirginiaUnion]{organization={Virginia Union University},
	 city={Richmond},
	 postcode={},
	 state={VA},
	 country={USA}} 
 
\affiliation[WayneState]{organization={Wayne State University},
	 addressline={666 W. Hancock St.},
	 city={Detroit},
	 postcode={48230},
	 state={MI},
	 country={USA}} 
 
\affiliation[WI]{organization={Weizmann Institute of Science},
	 city={Rehovot},
	 country={Israel}} 
 
\affiliation[WandM]{organization={The College of William and Mary},
	 city={Williamsburg},
	 state={VA},
	 country={USA}} 
 
\affiliation[Yamagata]{organization={Yamagata University},
	 city={Yamagata},
	 country={Japan}} 
 
\affiliation[Yarmouk]{organization={Yarmouk University},
	 city={Irbid},
	 country={Jordan}} 
 
\affiliation[Yonsei]{organization={Yonsei University},
	 city={Seoul},
	 country={Republic of Korea}} 
 
\affiliation[York]{organization={University of York},
	 city={York},
	 country={UK}} 
 
\affiliation[Zagreb]{organization={University of Zagreb},
	 city={Zagreb},
	 country={Croatia}} 
 


==> Submit_ArXiv/authors/authorlist_new.tex <==
\author[MIT]{C.~Fanelli}
\author[Regina]{Z~Papandreou}
\author[Regina]{K.~Suresh}
\author[MoreheadState]{J.~K.~Adkins}
\author[RIKEN]{Y.~Akiba}
\author[UKansas]{A.~Albataineh}
\author[ODU]{M.~Amaryan}
\author[Oslo]{I.~C.~Arsene}
\author[Sungkyunkwan]{J.~Bae}
\author[UVA]{X.~Bai}
\author[Yonsei]{M.~Bashkanov}
\author[UH]{R.~Bellwied}
\author[Duquesne]{F.~Benmokhtar}
\author[CFNS,StonyBrook,RBRC]{J.~C.~Bernauer}
\author[ORNL]{F.~Bock}
\author[FIU]{W.~Boeglin}
\author[WI]{M.~Borysova}
\author[CNU]{E.~Brash}
\author[JLab]{P.~Brindza}
\author[GWU]{W.~J.~Briscoe}
\author[LANL]{M.~Brooks}
\author[ODU]{S.~Bueltmann}
\author[JazanUniversity]{M.~H.~S.~Bukhari}
\author[UKansas]{A.~Bylinkin}
\author[UConn]{R.~Capobianco}
\author[AcademiaSinica]{W.-C.~Chang}
\author[Sejong]{Y.~Cheon}
\author[CCNU]{K.~Chen}
\author[NTU]{K.-F.~Chen}
\author[NCU]{K.-Y.~Cheng}
\author[BNL]{M.~Chiu}
\author[UTsukuba]{T.~Chujo}
\author[BGU]{Z.~Citron}
\author[CFNS,StonyBrook]{E.~Cline}
\author[NRCN]{E.~Cohen}
\author[ORNL]{T.~Cormier}
\author[LANL]{Y.~Corrales~Morales}
\author[UVA]{C.~Cotton}
\author[UKY]{C.~Crawford}
\author[ORNL]{S.~Creekmore}
\author[JLab]{C.Cuevas}
\author[ORNL]{J.~Cunningham}
\author[BNL]{G.~David}
\author[LANL]{C.~T.~Dean}
\author[ORNL]{M.~Demarteau}
\author[UConn]{S.~Diehl}
\author[Yamagata]{N.~Doshita}
\author[IJCLabOrsay]{R.~Dupr\'{e}}
\author[LANL]{J.~M.~Durham}
\author[GSI]{R.~Dzhygadlo}
\author[ORNL]{R.~Ehlers}
\author[MSU]{L.~El~Fassi}
\author[UVA]{A.~Emmert}
\author[JLab]{R.~Ent}
\author[UKY]{R.~Fatemi}
\author[Yonsei]{S.~Fegan}
\author[Charles]{M.~Finger}
\author[Charles]{M.~Finger~Jr.}
\author[Ohio]{J.~Frantz}
\author[HUJI]{M.~Friedman}
\author[York]{I.~Friscic}
\author[UH]{D.~Gangadharan}
\author[Glasgow]{S.~Gardner}
\author[Glasgow]{K.~Gates}
\author[Rice]{F.~Geurts}
\author[Rutgers]{R.~Gilman}
\author[Glasgow]{D.~Glazier}
\author[ORNL]{E.~Glimos}
\author[RIKEN]{Y.~Goto}
\author[AUGIE]{N.~Grau}
\author[Vanderbilt]{S.~V.~Greene}
\author[IMP]{A.~Q.~Guo}
\author[FIU]{L.~Guo}
\author[Yarmouk]{S.~K.~Ha}
\author[BNL]{J.~Haggerty}
\author[UConn]{T.~Hayward}
\author[GeorgiaState]{X.~He}
\author[MIT]{O.~Hen}
\author[JLab]{D.~W.~Higinbotham}
\author[IJCLabOrsay]{M.~Hoballah}
\author[NTHU]{P.-h.~J.~Hsu}
\author[BNL]{J.~Huang}
\author[Regina]{G.~Huber}
\author[UH]{A.~Hutson}
\author[Yarmouk]{K.~Y.~Hwang}
\author[ODU]{C.~Hyde}
\author[Tsukuba]{M.~Inaba}
\author[Yamagata]{T.~Iwata}
\author[Kyungpook]{H.-S.~Jo}
\author[UConn]{K.~Joo}
\author[VirginiaUnion]{N.~Kalantarians}
\author[Shinshu]{K.~Kawade}
\author[Regina]{S.~Kay}
\author[UConn]{A.~Kim}
\author[Sungkyunkwan]{B.~Kim}
\author[Pusan]{C.~Kim}
\author[RIKEN]{M.~Kim}
\author[Pusan]{Y.~Kim}
\author[Sejong]{Y.~Kim}
\author[BNL]{E.~Kistenev}
\author[UConn]{V.~Klimenko}
\author[Seoul]{S.~H.~Ko}
\author[MIT]{I.~Korover}
\author[UKY]{W.~Korsch}
\author[UKansas]{G.~Krintiras}
\author[ODU]{S.~Kuhn}
\author[NCU]{C.-M.~Kuo}
\author[MIT]{T.~Kutz}
\author[IowaState]{J.~Lajoie}
\author[JLab]{D.~Lawrence}
\author[IowaState]{S.~Lebedev}
\author[Seoul]{J.~S.~H.~Lee}
\author[Kyungpook]{S.~W.~Lee}
\author[MIT]{Y.-J.~Lee}
\author[Rice]{W.~Li}
\author[CFNS,StonyBrook,WandM]{W.~Li}
\author[CIAE]{X.~Li}
\author[LANL]{X.~Li}
\author[IMP]{Y.~T.~Liang}
\author[Pusan]{S.~Lim}
\author[AcademiaSinica]{C.-h.~Lin}
\author[IMP]{D.~X.~Lin}
\author[LANL]{K.~Liu}
\author[LANL]{M.~X.~Liu}
\author[Glasgow]{K.~Livingston}
\author[UVA]{N.~Liyanage}
\author[WayneState]{W.~J.~Llope}
\author[ORNL]{C.~Loizides}
\author[NewHampshire]{E.~Long}
\author[NTU]{R.-S.~Lu}
\author[CIAE]{Z.~Lu}
\author[Yonsei]{W.~Lynch}
\author[IJCLabOrsay]{D.~Marchand}
\author[CzechTechUniv]{M.~Marcisovsky}
\author[FIU]{P.~Markowitz}
\author[LANL]{P.~McGaughey}
\author[Ljubljana]{M.~Mihovilovic}
\author[MIT]{R.~G.~Milner}
\author[WI]{A.~Milov}
\author[Yamagata]{Y.~Miyachi}
\author[CNU]{P.~Monaghan}
\author[Glasgow]{R.~Montgomery}
\author[BNL]{D.~Morrison}
\author[IJCLabOrsay]{C.~Munoz~Camacho}
\author[UKansas]{M.~Murray}
\author[LANL]{K.~Nagai}
\author[CUBoulder]{J.~Nagle}
\author[RIKEN]{I.~Nakagawa}
\author[UTK]{C.~Nattrass}
\author[JLab]{D.~Nguyen}
\author[IJCLabOrsay]{S.~Niccolai}
\author[BNL]{R.~Nouicer}
\author[RIKEN]{G.~Nukazuka}
\author[UVA]{M.~Nycz}
\author[NRNUMEPhI]{V.~A.~Okorokov}
\author[Regina]{S.~Ore\v{s}i\'{c}}
\author[ORNL]{J.D.~Osborn}
\author[LANL]{C.~O'Shaughnessy}
\author[NTU]{S.~Paganis}
\author[NMSU]{S.~Pate}
\author[IowaState]{M.~Patel}
\author[MIT]{C.~Paus}
\author[Glasgow]{G.~Penman}
\author[UIUC]{M.~G.~Perdekamp}
\author[CUBoulder]{D.~V.~Perepelitsa}
\author[LANL]{H.~Periera~da~Costa}
\author[GSI]{K.~Peters}
\author[CNU]{W.~Phelps}
\author[TAU]{E.~Piasetzky}
\author[BNL]{C.~Pinkenburg}
\author[Charles]{I.~Prochazka}
\author[LehighUniversity]{T.~Protzman}
\author[BNL]{M.~Purschke}
\author[WayneState]{J.~Putschke}
\author[MIT]{J.~R.~Pybus}
\author[JLab]{R.~Rajput-Ghoshal}
\author[ORNL]{J.~Rasson}
\author[FIU]{B.~Raue}
\author[ORNL]{K.~Read}
\author[Oslo]{K.~R\o{}ed}
\author[LehighUniversity]{R.~Reed}
\author[FIU]{J.~Reinhold}
\author[LANL]{E.~L.~Renner}
\author[UConn]{J.~Richards}
\author[UIUC]{C.~Riedl}
\author[BNL]{T.~Rinn}
\author[Ohio]{J.~Roche}
\author[MIT]{G.~M.~Roland}
\author[HUJI]{G.~Ron}
\author[IowaState]{M.~Rosati}
\author[UKansas]{C.~Royon}
\author[Pusan]{J.~Ryu}
\author[Rutgers]{S.~Salur}
\author[MIT]{N.~Santiesteban}
\author[UConn]{R.~Santos}
\author[GeorgiaState]{M.~Sarsour}
\author[ORNL]{J.~Schambach}
\author[GWU]{A.~Schmidt}
\author[ORNL]{N.~Schmidt}
\author[GSI]{C.~Schwarz}
\author[GSI]{J.~Schwiening}
\author[RIKEN]{R.~Seidl}
\author[UIUC]{A.~Sickles}
\author[UConn]{P.~Simmerling}
\author[Ljubljana]{S.~Sirca}
\author[GeorgiaState]{D.~Sharma}
\author[LANL]{Z.~Shi}
\author[Nihon]{T.-A.~Shibata}
\author[NCU]{C.-W.~Shih}
\author[RIKEN]{S.~Shimizu}
\author[UConn]{U.~Shrestha}
\author[NewHampshire]{K.~Slifer}
\author[LANL]{K.~Smith}
\author[LLNL]{R.~Soltz}
\author[LANL]{W.~Sondheim}
\author[CIAE]{J.~Song}
\author[Pusan]{J.~Song}
\author[GWU]{I.~I.~Strakovsky}
\author[BNL]{P.~Steinberg}
\author[WandM]{J.~Stevens}
\author[PNNL]{J.~Strube}
\author[CIAE]{P.~Sun}
\author[CCNU]{X.~Sun}
\author[NCU]{W.-C.~Tang}
\author[IowaState]{S.~Tapia~Araya}
\author[Vanderbilt]{S.~Tarafdar}
\author[BrunelUniversity]{L.~Teodorescu}
\author[UH]{A.~Timmins}
\author[CzechTechUniv]{L.~Tomasek}
\author[UConn]{N.~Trotta}
\author[Oslo]{T.~S.~Tveter}
\author[IowaState]{E.~Umaka}
\author[Regina]{A.~Usman}
\author[LANL]{H.~W.~van~Hecke}
\author[Vanderbilt]{J.~Velkovska}
\author[IJCLabOrsay]{E.~Voutier}
\author[IJCLabOrsay]{P.K.~Wang}
\author[UKansas]{Q.~Wang}
\author[CCNU]{Y.~Wang}
\author[Tsinghua]{Y.~Wang}
\author[Yonsei]{D.~P.~Watts}
\author[ODU]{L.~Weinstein}
\author[MIT]{M.~Williams}
\author[LANL]{C.-P.~Wong}
\author[PNNL]{L.~Wood}
\author[CanisiusCollege]{M.~H.~Wood}
\author[BNL]{C.~Woody}
\author[MIT]{B.~Wyslouch}
\author[Tsinghua]{Z.~Xiao}
\author[KobeUniversity]{Y.~Yamazaki}
\author[NCKU]{Y.~Yang}
\author[Tsinghua]{Z.~Ye}
\author[Yarmouk]{H.~D.~Yoo}
\author[LANL]{M.~Yurov}
\author[Yonsei]{N.~Zachariou}
\author[Columbia]{W.A.~Zajc}
\author[UVA]{J.~Zhang}
\author[Tsinghua]{Y.~Zhang}
\author[IMP]{Y.~X.~Zhao}
\author[UVA]{X.~Zheng}
\author[Tsinghua]{P.~Zhuang}

==> Submit_ArXiv/authors/authors-alphabetical-static.tex <==
\author[MoreheadState]{J.~K.~Adkins}
\author[RIKEN]{Y.~Akiba}
\author[UKansas]{A.~Albataineh}
\author[ODU]{M.~Amaryan}
\author[Oslo]{I.~C.~Arsene}
\author[Sungkyunkwan]{J.~Bae}
\author[UVA]{X.~Bai}
\author[Yonsei]{M.~Bashkanov}
\author[UH]{R.~Bellwied}
\author[Duquesne]{F.~Benmokhtar}
\author[CFNS,StonyBrook,RBRC]{J.~C.~Bernauer}
\author[ORNL]{F.~Bock}
\author[FIU]{W.~Boeglin}
\author[WI]{M.~Borysova}
\author[CNU]{E.~Brash}
\author[JLab]{P.~Brindza}
\author[GWU]{W.~J.~Briscoe}
\author[LANL]{M.~Brooks}
\author[ODU]{S.~Bueltmann}
\author[JazanUniversity]{M.~H.~S.~Bukhari}
\author[UKansas]{A.~Bylinkin}
\author[UConn]{R.~Capobianco}
\author[AcademiaSinica]{W.-C.~Chang}
\author[Sejong]{Y.~Cheon}
\author[CCNU]{K.~Chen}
\author[NTU]{K.-F.~Chen}
\author[NCU]{K.-Y.~Cheng}
\author[BNL]{M.~Chiu}
\author[UTsukuba]{T.~Chujo}
\author[BGU]{Z.~Citron}
\author[CFNS,StonyBrook]{E.~Cline}
\author[NRCN]{E.~Cohen}
\author[ORNL]{T.~Cormier}
\author[LANL]{Y.~Corrales~Morales}
\author[UVA]{C.~Cotton}
\author[UKY]{C.~Crawford}
\author[ORNL]{S.~Creekmore}
\author[JLab]{C.Cuevas}
\author[ORNL]{J.~Cunningham}
\author[BNL]{G.~David}
\author[LANL]{C.~T.~Dean}
\author[ORNL]{M.~Demarteau}
\author[UConn]{S.~Diehl}
\author[Yamagata]{N.~Doshita}
\author[IJCLabOrsay]{R.~Dupr\'{e}}
\author[LANL]{J.~M.~Durham}
\author[GSI]{R.~Dzhygadlo}
\author[ORNL]{R.~Ehlers}
\author[MSU]{L.~El~Fassi}
\author[UVA]{A.~Emmert}
\author[JLab]{R.~Ent}
\author[MIT]{C.~Fanelli}
\author[UKY]{R.~Fatemi}
\author[Yonsei]{S.~Fegan}
\author[Charles]{M.~Finger}
\author[Charles]{M.~Finger~Jr.}
\author[Ohio]{J.~Frantz}
\author[HUJI]{M.~Friedman}
\author[York]{I.~Friscic}
\author[UH]{D.~Gangadharan}
\author[Glasgow]{S.~Gardner}
\author[Glasgow]{K.~Gates}
\author[Rice]{F.~Geurts}
\author[Rutgers]{R.~Gilman}
\author[Glasgow]{D.~Glazier}
\author[ORNL]{E.~Glimos}
\author[RIKEN]{Y.~Goto}
\author[AUGIE]{N.~Grau}
\author[Vanderbilt]{S.~V.~Greene}
\author[IMP]{A.~Q.~Guo}
\author[FIU]{L.~Guo}
\author[Yarmouk]{S.~K.~Ha}
\author[BNL]{J.~Haggerty}
\author[UConn]{T.~Hayward}
\author[GeorgiaState]{X.~He}
\author[MIT]{O.~Hen}
\author[JLab]{D.W.~Higinbotham}
\author[IJCLabOrsay]{M.~Hoballah}
\author[NTHU]{P.-h.~J.~Hsu}
\author[BNL]{J.~Huang}
\author[Regina]{G.~Huber}
\author[UH]{A.~Hutson}
\author[Yarmouk]{K.~Y.~Hwang}
\author[ODU]{C.~Hyde}
\author[Tsukuba]{M.~Inaba}
\author[Yamagata]{T.~Iwata}
\author[Kyungpook]{H.-S.~Jo}
\author[UConn]{K.~Joo}
\author[VirginiaUnion]{N.~Kalantarians}
\author[Shinshu]{K.~Kawade}
\author[Regina]{S.~Kay}
\author[UConn]{A.~Kim}
\author[Sungkyunkwan]{B.~Kim}
\author[Pusan]{C.~Kim}
\author[RIKEN]{M.~Kim}
\author[Pusan]{Y.~Kim}
\author[Sejong]{Y.~Kim}
\author[BNL]{E.~Kistenev}
\author[UConn]{V.~Klimenko}
\author[Seoul]{S.~H.~Ko}
\author[MIT]{I.~Korover}
\author[UKY]{W.~Korsch}
\author[UKansas]{G.~Krintiras}
\author[ODU]{S.~Kuhn}
\author[NCU]{C.-M.~Kuo}
\author[MIT]{T.~Kutz}
\author[IowaState]{J.~Lajoie}
\author[JLab]{D.~Lawrence}
\author[IowaState]{S.~Lebedev}
\author[Seoul]{J.~S.~H.~Lee}
\author[Kyungpook]{S.~W.~Lee}
\author[MIT]{Y.-J.~Lee}
\author[Rice]{W.~Li}
\author[CFNS,StonyBrook,WandM]{W.~Li}
\author[CIAE]{X.~Li}
\author[LANL]{X.~Li}
\author[IMP]{Y.~T.~Liang}
\author[Pusan]{S.~Lim}
\author[AcademiaSinica]{C.-h.~Lin}
\author[IMP]{D.~X.~Lin}
\author[LANL]{K.~Liu}
\author[LANL]{M.~X.~Liu}
\author[Glasgow]{K.~Livingston}
\author[UVA]{N.~Liyanage}
\author[WayneState]{W.~J.~Llope}
\author[ORNL]{C.~Loizides}
\author[NewHampshire]{E.~Long}
\author[NTU]{R.-S.~Lu}
\author[CIAE]{Z.~Lu}
\author[Yonsei]{W.~Lynch}
\author[IJCLabOrsay]{D.~Marchand}
\author[CzechTechUniv]{M.~Marcisovsky}
\author[FIU]{P.~Markowitz}
\author[LANL]{P.~McGaughey}
\author[Ljubljana]{M.~Mihovilovic}
\author[MIT]{R.~G.~Milner}
\author[WI]{A.~Milov}
\author[Yamagata]{Y.~Miyachi}
\author[CNU]{P.~Monaghan}
\author[Glasgow]{R.~Montgomery}
\author[BNL]{D.~Morrison}
\author[IJCLabOrsay]{C.~Munoz~Camacho}
\author[UKansas]{M.~Murray}
\author[LANL]{K.~Nagai}
\author[CUBoulder]{J.~Nagle}
\author[RIKEN]{I.~Nakagawa}
\author[UTK]{C.~Nattrass}
\author[JLab]{D.~Nguyen}
\author[IJCLabOrsay]{S.~Niccolai}
\author[BNL]{R.~Nouicer}
\author[RIKEN]{G.~Nukazuka}
\author[UVA]{M.~Nycz}
\author[NRNUMEPhI]{V.~A.~Okorokov}
\author[Regina]{S.~Ore$\check{s}$i$\acute{c}$}
\author[ORNL]{J.~Osborn}
\author[LANL]{C.~O'Shaughnessy}
\author[NTU]{S.~Paganis}
\author[Regina]{Z~Papandreou}
\author[NMSU]{S.~Pate}
\author[IowaState]{M.~Patel}
\author[MIT]{C.~Paus}
\author[Glasgow]{G.~Penman}
\author[UIUC]{M.~G.~Perdekamp}
\author[CUBoulder]{D.~V.~Perepelitsa}
\author[LANL]{H.~Periera~da~Costa}
\author[GSI]{K.~Peters}
\author[CNU]{W.~Phelps}
\author[TAU]{E.~Piasetzky}
\author[BNL]{C.~Pinkenburg}
\author[Charles]{I.~Prochazka}
\author[LehighUniversity]{T.~Protzman}
\author[BNL]{M.~Purschke}
\author[WayneState]{J.~Putschke}
\author[MIT]{J.~R.~Pybus}
\author[JLab]{R.~Rajput-Ghoshal}
\author[ORNL]{J.~Rasson}
\author[FIU]{B.~Raue}
\author[ORNL]{K.~Read}
\author[Oslo]{K.~R$\o$ed}
\author[LehighUniversity]{R.~Reed}
\author[FIU]{J.~Reinhold}
\author[LANL]{E.~L.~Renner}
\author[UConn]{J.~Richards}
\author[UIUC]{C.~Riedl}
\author[BNL]{T.~Rinn}
\author[Ohio]{J.~Roche}
\author[MIT]{G.~M.~Roland}
\author[HUJI]{G.~Ron}
\author[IowaState]{M.~Rosati}
\author[UKansas]{C.~Royon}
\author[Pusan]{J.~Ryu}
\author[Rutgers]{S.~Salur}
\author[MIT]{N.~Santiesteban}
\author[UConn]{R.~Santos}
\author[GeorgiaState]{M.~Sarsour}
\author[ORNL]{J.~Schambach}
\author[GWU]{A.~Schmidt}
\author[ORNL]{N.~Schmidt}
\author[GSI]{C.~Schwarz}
\author[GSI]{J.~Schwiening}
\author[RIKEN]{R.~Seidl}
\author[UIUC]{A.~Sickles}
\author[UConn]{P.~Simmerling}
\author[Ljubljana]{S.~Sirca}
\author[GeorgiaState]{D.~Sharma}
\author[LANL]{Z.~Shi}
\author[Nihon]{T.-A.~Shibata}
\author[NCU]{C.-W.~Shih}
\author[RIKEN]{S.~Shimizu}
\author[UConn]{U.~Shrestha}
\author[NewHampshire]{K.~Slifer}
\author[LANL]{K.~Smith}
\author[LLNL]{R.~Soltz}
\author[LANL]{W.~Sondheim}
\author[CIAE]{J.~Song}
\author[Pusan]{J.~Song}
\author[GWU]{I.~I.~Strakovsky}
\author[BNL]{P.~Steinberg}
\author[WandM]{J.~Stevens}
\author[PNNL]{J.~Strube}
\author[CIAE]{P.~Sun}
\author[CCNU]{X.~Sun}
\author[Regina]{K.~Suresh}
\author[NCU]{W.-C.~Tang}
\author[IowaState]{S.~Tapia~Araya}
\author[Vanderbilt]{S.~Tarafdar}
\author[BrunelUniversity]{L.~Teodorescu}
\author[UH]{A.~Timmins}
\author[CzechTechUniv]{L.~Tomasek}
\author[UConn]{N.~Trotta}
\author[Oslo]{T.~S.~Tveter}
\author[IowaState]{E.~Umaka}
\author[Regina]{A.~Usman}
\author[LANL]{H.~W.~van~Hecke}
\author[Vanderbilt]{J.~Velkovska}
\author[IJCLabOrsay]{E.~Voutier}
\author[IJCLabOrsay]{P.K.~Wang}
\author[UKansas]{Q.~Wang}
\author[CCNU]{Y.~Wang}
\author[Tsinghua]{Y.~Wang}
\author[Yonsei]{D.~P.~Watts}
\author[ODU]{L.~Weinstein}
\author[MIT]{M.~Williams}
\author[LANL]{C.-P.~Wong}
\author[PNNL]{L.~Wood}
\author[CanisiusCollege]{M.~H.~Wood}
\author[BNL]{C.~Woody}
\author[MIT]{B.~Wyslouch}
\author[Tsinghua]{Z.~Xiao}
\author[KobeUniversity]{Y.~Yamazaki}
\author[NCKU]{Y.~Yang}
\author[Tsinghua]{Z.~Ye}
\author[Yarmouk]{H.~D.~Yoo}
\author[LANL]{M.~Yurov}
\author[Yonsei]{N.~Zachariou}
\author[Columbia]{W.A.~Zajc}
\author[UVA]{J.~Zhang}
\author[Tsinghua]{Y.~Zhang}
\author[IMP]{Y.~X.~Zhao}
\author[UVA]{X.~Zheng}
\author[Tsinghua]{P.~Zhuang}


==> Submit_ArXiv/authors/authors-alphabetical.tex <==
\author[MoreheadState]{J.~K.~Adkins}
\author[RIKEN]{Y.~Akiba}
\author[UKansas]{A.~Albataineh}
\author[ODU]{M.~Amaryan}
\author[Oslo]{I.~C.~Arsene}
\author[Sungkyunkwan]{J.~Bae}
\author[UVA]{X.~Bai}
\author[Yonsei]{M.~Bashkanov}
\author[UH]{R.~Bellwied}
\author[Duquesne]{F.~Benmokhtar}
\author[CFNS,StonyBrook,RBRC]{J.~C.~Bernauer}
\author[ORNL]{F.~Bock}
\author[FIU]{W.~Boeglin}
\author[WI]{M.~Borysova}
\author[CNU]{E.~Brash}
\author[JLab]{P.~Brindza}
\author[GWU]{W.~J.~Briscoe}
\author[LANL]{M.~Brooks}
\author[ODU]{S.~Bueltmann}
\author[JazanUniversity]{M.~H.~S.~Bukhari}
\author[UKansas]{A.~Bylinkin}
\author[UConn]{R.~Capobianco}
\author[AcademiaSinica]{W.-C.~Chang}
\author[Sejong]{Y.~Cheon}
\author[CCNU]{K.~Chen}
\author[NTU]{K.-F.~Chen}
\author[NCU]{K.-Y.~Cheng}
\author[BNL]{M.~Chiu}
\author[UTsukuba]{T.~Chujo}
\author[BGU]{Z.~Citron}
\author[CFNS,StonyBrook]{E.~Cline}
\author[NRCN]{E.~Cohen}
\author[ORNL]{T.~Cormier}
\author[LANL]{Y.~Corrales~Morales}
\author[UVA]{C.~Cotton}
\author[UKY]{C.~Crawford}
\author[ORNL]{S.~Creekmore}
\author[JLab]{C.Cuevas}
\author[ORNL]{J.~Cunningham}
\author[BNL]{G.~David}
\author[LANL]{C.~T.~Dean}
\author[ORNL]{M.~Demarteau}
\author[UConn]{S.~Diehl}
\author[Yamagata]{N.~Doshita}
\author[IJCLabOrsay]{R.~Dupr\'{e}}
\author[LANL]{J.~M.~Durham}
\author[GSI]{R.~Dzhygadlo}
\author[ORNL]{R.~Ehlers}
\author[MSU]{L.~El~Fassi}
\author[UVA]{A.~Emmert}
\author[JLab]{R.~Ent}
\author[MIT]{C.~Fanelli}
\author[UKY]{R.~Fatemi}
\author[Yonsei]{S.~Fegan}
\author[Charles]{M.~Finger}
\author[Charles]{M.~Finger~Jr.}
\author[Ohio]{J.~Frantz}
\author[HUJI]{M.~Friedman}
\author[York]{I.~Friscic}
\author[UH]{D.~Gangadharan}
\author[Glasgow]{S.~Gardner}
\author[Glasgow]{K.~Gates}
\author[Rice]{F.~Geurts}
\author[Rutgers]{R.~Gilman}
\author[Glasgow]{D.~Glazier}
\author[ORNL]{E.~Glimos}
\author[RIKEN]{Y.~Goto}
\author[AUGIE]{N.~Grau}
\author[Vanderbilt]{S.~V.~Greene}
\author[IMP]{A.~Q.~Guo}
\author[FIU]{L.~Guo}
\author[Yarmouk]{S.~K.~Ha}
\author[BNL]{J.~Haggerty}
\author[UConn]{T.~Hayward}
\author[GeorgiaState]{X.~He}
\author[MIT]{O.~Hen}
\author[JLab]{D.~W.~Higinbotham}
\author[IJCLabOrsay]{M.~Hoballah}
\author[NTHU]{P.-h.~J.~Hsu}
\author[BNL]{J.~Huang}
\author[Regina]{G.~Huber}
\author[UH]{A.~Hutson}
\author[Yarmouk]{K.~Y.~Hwang}
\author[ODU]{C.~Hyde}
\author[Tsukuba]{M.~Inaba}
\author[Yamagata]{T.~Iwata}
\author[Kyungpook]{H.-S.~Jo}
\author[UConn]{K.~Joo}
\author[VirginiaUnion]{N.~Kalantarians}
\author[Shinshu]{K.~Kawade}
\author[Regina]{S.~Kay}
\author[UConn]{A.~Kim}
\author[Sungkyunkwan]{B.~Kim}
\author[Pusan]{C.~Kim}
\author[RIKEN]{M.~Kim}
\author[Pusan]{Y.~Kim}
\author[Sejong]{Y.~Kim}
\author[BNL]{E.~Kistenev}
\author[UConn]{V.~Klimenko}
\author[Seoul]{S.~H.~Ko}
\author[MIT]{I.~Korover}
\author[UKY]{W.~Korsch}
\author[UKansas]{G.~Krintiras}
\author[ODU]{S.~Kuhn}
\author[NCU]{C.-M.~Kuo}
\author[MIT]{T.~Kutz}
\author[IowaState]{J.~Lajoie}
\author[JLab]{D.~Lawrence}
\author[IowaState]{S.~Lebedev}
\author[Seoul]{J.~S.~H.~Lee}
\author[Kyungpook]{S.~W.~Lee}
\author[MIT]{Y.-J.~Lee}
\author[Rice]{W.~Li}
\author[CFNS,StonyBrook,WandM]{W.~Li}
\author[CIAE]{X.~Li}
\author[LANL]{X.~Li}
\author[IMP]{Y.~T.~Liang}
\author[Pusan]{S.~Lim}
\author[AcademiaSinica]{C.-h.~Lin}
\author[IMP]{D.~X.~Lin}
\author[LANL]{K.~Liu}
\author[LANL]{M.~X.~Liu}
\author[Glasgow]{K.~Livingston}
\author[UVA]{N.~Liyanage}
\author[WayneState]{W.~J.~Llope}
\author[ORNL]{C.~Loizides}
\author[NewHampshire]{E.~Long}
\author[NTU]{R.-S.~Lu}
\author[CIAE]{Z.~Lu}
\author[Yonsei]{W.~Lynch}
\author[IJCLabOrsay]{D.~Marchand}
\author[CzechTechUniv]{M.~Marcisovsky}
\author[FIU]{P.~Markowitz}
\author[LANL]{P.~McGaughey}
\author[Ljubljana]{M.~Mihovilovic}
\author[MIT]{R.~G.~Milner}
\author[WI]{A.~Milov}
\author[Yamagata]{Y.~Miyachi}
\author[CNU]{P.~Monaghan}
\author[Glasgow]{R.~Montgomery}
\author[BNL]{D.~Morrison}
\author[IJCLabOrsay]{C.~Munoz~Camacho}
\author[UKansas]{M.~Murray}
\author[LANL]{K.~Nagai}
\author[CUBoulder]{J.~Nagle}
\author[RIKEN]{I.~Nakagawa}
\author[UTK]{C.~Nattrass}
\author[JLab]{D.~Nguyen}
\author[IJCLabOrsay]{S.~Niccolai}
\author[BNL]{R.~Nouicer}
\author[RIKEN]{G.~Nukazuka}
\author[UVA]{M.~Nycz}
\author[NRNUMEPhI]{V.~A.~Okorokov}
\author[Regina]{S.~Ore\v{s}i\'{c}}
\author[ORNL]{J.D.~Osborn}
\author[LANL]{C.~O'Shaughnessy}
\author[NTU]{S.~Paganis}
\author[Regina]{Z~Papandreou}
\author[NMSU]{S.~Pate}
\author[IowaState]{M.~Patel}
\author[MIT]{C.~Paus}
\author[Glasgow]{G.~Penman}
\author[UIUC]{M.~G.~Perdekamp}
\author[CUBoulder]{D.~V.~Perepelitsa}
\author[LANL]{H.~Periera~da~Costa}
\author[GSI]{K.~Peters}
\author[CNU]{W.~Phelps}
\author[TAU]{E.~Piasetzky}
\author[BNL]{C.~Pinkenburg}
\author[Charles]{I.~Prochazka}
\author[LehighUniversity]{T.~Protzman}
\author[BNL]{M.~Purschke}
\author[WayneState]{J.~Putschke}
\author[MIT]{J.~R.~Pybus}
\author[JLab]{R.~Rajput-Ghoshal}
\author[ORNL]{J.~Rasson}
\author[FIU]{B.~Raue}
\author[ORNL]{K.~Read}
\author[Oslo]{K.~R\o{}ed}
\author[LehighUniversity]{R.~Reed}
\author[FIU]{J.~Reinhold}
\author[LANL]{E.~L.~Renner}
\author[UConn]{J.~Richards}
\author[UIUC]{C.~Riedl}
\author[BNL]{T.~Rinn}
\author[Ohio]{J.~Roche}
\author[MIT]{G.~M.~Roland}
\author[HUJI]{G.~Ron}
\author[IowaState]{M.~Rosati}
\author[UKansas]{C.~Royon}
\author[Pusan]{J.~Ryu}
\author[Rutgers]{S.~Salur}
\author[MIT]{N.~Santiesteban}
\author[UConn]{R.~Santos}
\author[GeorgiaState]{M.~Sarsour}
\author[ORNL]{J.~Schambach}
\author[GWU]{A.~Schmidt}
\author[ORNL]{N.~Schmidt}
\author[GSI]{C.~Schwarz}
\author[GSI]{J.~Schwiening}
\author[RIKEN]{R.~Seidl}
\author[UIUC]{A.~Sickles}
\author[UConn]{P.~Simmerling}
\author[Ljubljana]{S.~Sirca}
\author[GeorgiaState]{D.~Sharma}
\author[LANL]{Z.~Shi}
\author[Nihon]{T.-A.~Shibata}
\author[NCU]{C.-W.~Shih}
\author[RIKEN]{S.~Shimizu}
\author[UConn]{U.~Shrestha}
\author[NewHampshire]{K.~Slifer}
\author[LANL]{K.~Smith}
\author[LLNL]{R.~Soltz}
\author[LANL]{W.~Sondheim}
\author[CIAE]{J.~Song}
\author[Pusan]{J.~Song}
\author[GWU]{I.~I.~Strakovsky}
\author[BNL]{P.~Steinberg}
\author[WandM]{J.~Stevens}
\author[PNNL]{J.~Strube}
\author[CIAE]{P.~Sun}
\author[CCNU]{X.~Sun}
\author[Regina]{K.~Suresh}
\author[NCU]{W.-C.~Tang}
\author[IowaState]{S.~Tapia~Araya}
\author[Vanderbilt]{S.~Tarafdar}
\author[BrunelUniversity]{L.~Teodorescu}
\author[UH]{A.~Timmins}
\author[CzechTechUniv]{L.~Tomasek}
\author[UConn]{N.~Trotta}
\author[Oslo]{T.~S.~Tveter}
\author[IowaState]{E.~Umaka}
\author[Regina]{A.~Usman}
\author[LANL]{H.~W.~van~Hecke}
\author[Vanderbilt]{J.~Velkovska}
\author[IJCLabOrsay]{E.~Voutier}
\author[IJCLabOrsay]{P.K.~Wang}
\author[UKansas]{Q.~Wang}
\author[CCNU]{Y.~Wang}
\author[Tsinghua]{Y.~Wang}
\author[Yonsei]{D.~P.~Watts}
\author[ODU]{L.~Weinstein}
\author[MIT]{M.~Williams}
\author[LANL]{C.-P.~Wong}
\author[PNNL]{L.~Wood}
\author[CanisiusCollege]{M.~H.~Wood}
\author[BNL]{C.~Woody}
\author[MIT]{B.~Wyslouch}
\author[Tsinghua]{Z.~Xiao}
\author[KobeUniversity]{Y.~Yamazaki}
\author[NCKU]{Y.~Yang}
\author[Tsinghua]{Z.~Ye}
\author[Yarmouk]{H.~D.~Yoo}
\author[LANL]{M.~Yurov}
\author[Yonsei]{N.~Zachariou}
\author[Columbia]{W.A.~Zajc}
\author[UVA]{J.~Zhang}
\author[Tsinghua]{Y.~Zhang}
\author[IMP]{Y.~X.~Zhao}
\author[UVA]{X.~Zheng}
\author[Tsinghua]{P.~Zhuang}


==> Submit_ArXiv/authors/authors.tex <==
%
% Full list of ECCE Collaboratotions
%
% Click Refresh to get the latest version
%
% Goto the following to edit:
% https://www.overleaf.com/1234763137gmqgnzsrpsdj

\author[MIT]{C.~Fanelli}
\author[Regina]{Z.~Papandreou}
\author[Regina]{K.~Suresh}
\author[MoreheadState]{J.~K.~Adkins}
\author[RIKEN,RBRC]{Y.~Akiba}
\author[UKansas]{A.~Albataineh}
\author[ODU]{M.~Amaryan}
\author[Oslo]{I.~C.~Arsene}
\author[MSU]{C. Ayerbe Gayoso}
\author[Sungkyunkwan]{J.~Bae}
\author[UVA]{X.~Bai}
\author[BNL,JLab]{M.D.~Baker}
\author[York]{M.~Bashkanov}
\author[UH]{R.~Bellwied}
\author[Duquesne]{F.~Benmokhtar}
\author[CUA]{V.~Berdnikov}
\author[CFNS,StonyBrook,RBRC]{J.~C.~Bernauer}
\author[ORNL]{F.~Bock}
\author[FIU]{W.~Boeglin}
\author[WI]{M.~Borysova}
\author[CNU]{E.~Brash}
\author[JLab]{P.~Brindza}
\author[GWU]{W.~J.~Briscoe}
\author[LANL]{M.~Brooks}
\author[ODU]{S.~Bueltmann}
\author[JazanUniversity]{M.~H.~S.~Bukhari}
\author[UKansas]{A.~Bylinkin}
\author[UConn]{R.~Capobianco}
\author[AcademiaSinica]{W.-C.~Chang}
\author[Sejong]{Y.~Cheon}
\author[CCNU]{K.~Chen}
\author[NTU]{K.-F.~Chen}
\author[NCU]{K.-Y.~Cheng}
\author[BNL]{M.~Chiu}
\author[UTsukuba]{T.~Chujo}
\author[BGU]{Z.~Citron}
\author[CFNS,StonyBrook]{E.~Cline}
\author[NRCN]{E.~Cohen}
\author[ORNL]{T.~Cormier}
\author[LANL]{Y.~Corrales~Morales}
\author[UVA]{C.~Cotton}
\author[CUA]{J.~Crafts}
\author[UKY]{C.~Crawford}
\author[ORNL]{S.~Creekmore}
\author[JLab]{C.Cuevas}
\author[ORNL]{J.~Cunningham}
\author[BNL]{G.~David}
\author[LANL]{C.~T.~Dean}
\author[ORNL]{M.~Demarteau}
\author[UConn]{S.~Diehl}
\author[Yamagata]{N.~Doshita}
\author[IJCLabOrsay]{R.~Dupr\'{e}}
\author[LANL]{J.~M.~Durham}
\author[GSI]{R.~Dzhygadlo}
\author[ORNL]{R.~Ehlers}
\author[MSU]{L.~El~Fassi}
\author[UVA]{A.~Emmert}
\author[JLab]{R.~Ent}
%\author[MIT]{C.~Fanelli}
\author[UKY]{R.~Fatemi}
\author[York]{S.~Fegan}
\author[Charles]{M.~Finger}
\author[Charles]{M.~Finger~Jr.}
\author[Ohio]{J.~Frantz}
\author[HUJI]{M.~Friedman}
\author[York]{I.~Friscic}
\author[UH]{D.~Gangadharan}
\author[Glasgow]{S.~Gardner}
\author[Glasgow]{K.~Gates}
\author[Rice]{F.~Geurts}
\author[Rutgers]{R.~Gilman}
\author[Glasgow]{D.~Glazier}
\author[ORNL]{E.~Glimos}
\author[RIKEN,RBRC]{Y.~Goto}
\author[AUGIE]{N.~Grau}
\author[Vanderbilt]{S.~V.~Greene}
\author[IMP]{A.~Q.~Guo}
\author[FIU]{L.~Guo}
\author[Yarmouk]{S.~K.~Ha}
\author[BNL]{J.~Haggerty}
\author[UConn]{T.~Hayward}
\author[GeorgiaState]{X.~He}
\author[MIT]{O.~Hen}
\author[JLab]{D.~W.~Higinbotham}
\author[IJCLabOrsay]{M.~Hoballah}
\author[CUA]{T.~Horn}
\author[AANL]{A.~Hoghmrtsyan}
\author[NTHU]{P.-h.~J.~Hsu}
\author[BNL]{J.~Huang}
\author[Regina]{G.~Huber}
\author[UH]{A.~Hutson}
\author[Yonsei]{K.~Y.~Hwang}
\author[ODU]{C.~Hyde}
\author[Tsukuba]{M.~Inaba}
\author[Yamagata]{T.~Iwata}
\author[Kyungpook]{H.S.~Jo}
\author[UConn]{K.~Joo}
\author[VirginiaUnion]{N.~Kalantarians}
\author[CUA]{G.~Kalicy}
\author[Shinshu]{K.~Kawade}
\author[Regina]{S.~J.~D.~Kay}
\author[UConn]{A.~Kim}
\author[Sungkyunkwan]{B.~Kim}
\author[Pusan]{C.~Kim}
\author[RIKEN]{M.~Kim}
\author[Pusan]{Y.~Kim}
\author[Sejong]{Y.~Kim}
\author[BNL]{E.~Kistenev}
\author[UConn]{V.~Klimenko}
\author[Seoul]{S.~H.~Ko}
\author[MIT]{I.~Korover}
\author[UKY]{W.~Korsch}
\author[UKansas]{G.~Krintiras}
\author[ODU]{S.~Kuhn}
\author[NCU]{C.-M.~Kuo}
\author[MIT]{T.~Kutz}
\author[IowaState]{J.~Lajoie}
\author[JLab]{D.~Lawrence}
\author[IowaState]{S.~Lebedev}
\author[Sungkyunkwan]{H.~Lee}
\author[USeoul]{J.~S.~H.~Lee}
\author[Kyungpook]{S.~W.~Lee}
\author[MIT]{Y.-J.~Lee}
\author[Rice]{W.~Li}
\author[CFNS,StonyBrook,WandM]{W.B.~Li}
\author[USTC]{X.~Li}
\author[CIAE]{X.~Li}
\author[LANL]{X.~Li}
\author[MIT]{X.~Li}
\author[IMP]{Y.~T.~Liang}
\author[Pusan]{S.~Lim}
\author[AcademiaSinica]{C.-h.~Lin}
\author[IMP]{D.~X.~Lin}
\author[LANL]{K.~Liu}
\author[LANL]{M.~X.~Liu}
\author[Glasgow]{K.~Livingston}
\author[UVA]{N.~Liyanage}
\author[WayneState]{W.J.~Llope}
\author[ORNL]{C.~Loizides}
\author[NewHampshire]{E.~Long}
\author[NTU]{R.-S.~Lu}
\author[CIAE]{Z.~Lu}
\author[York]{W.~Lynch}
\author[IJCLabOrsay]{D.~Marchand}
\author[CzechTechUniv]{M.~Marcisovsky}
\author[FIU]{P.~Markowitz}
\author[AANL]{H.~Marukyan}
\author[LANL]{P.~McGaughey}
\author[Ljubljana]{M.~Mihovilovic}
\author[MIT]{R.~G.~Milner}
\author[WI]{A.~Milov}
\author[Yamagata]{Y.~Miyachi}
\author[AANL]{A.~Mkrtchyan}
\author[CNU]{P.~Monaghan}
\author[Glasgow]{R.~Montgomery}
\author[BNL]{D.~Morrison}
\author[AANL]{A.~Movsisyan}
\author[AANL]{H.~Mkrtchyan}
\author[AANL]{A.~Mkrtchyan}
\author[IJCLabOrsay]{C.~Munoz~Camacho}
\author[UKansas]{M.~Murray}
\author[LANL]{K.~Nagai}
\author[CUBoulder]{J.~Nagle}
\author[RIKEN]{I.~Nakagawa}
\author[UTK]{C.~Nattrass}
\author[JLab]{D.~Nguyen}
\author[IJCLabOrsay]{S.~Niccolai}
\author[BNL]{R.~Nouicer}
\author[RIKEN]{G.~Nukazuka}
\author[UVA]{M.~Nycz}
\author[NRNUMEPhI]{V.~A.~Okorokov}
\author[Regina]{S.~Ore\v{s}i\'{c}}
\author[ORNL]{J.D.~Osborn}
\author[LANL]{C.~O'Shaughnessy}
\author[NTU]{S.~Paganis}
%\author[Regina]{Z.~Papandreou}
\author[NMSU]{S.~F.~Pate}
\author[IowaState]{M.~Patel}
\author[MIT]{C.~Paus}
\author[Glasgow]{G.~Penman}
\author[UIUC]{M.~G.~Perdekamp}
\author[CUBoulder]{D.~V.~Perepelitsa}
\author[LANL]{H.~Periera~da~Costa}
\author[GSI]{K.~Peters}
\author[CNU]{W.~Phelps}
\author[TAU]{E.~Piasetzky}
\author[BNL]{C.~Pinkenburg}
\author[Charles]{I.~Prochazka}
\author[LehighUniversity]{T.~Protzman}
\author[BNL]{M.~L.~Purschke}
\author[WayneState]{J.~Putschke}
\author[MIT]{J.~R.~Pybus}
\author[JLab]{R.~Rajput-Ghoshal}
\author[ORNL]{J.~Rasson}
\author[FIU]{B.~Raue}
\author[ORNL]{K.F.~Read}
\author[Oslo]{K.~R\o{}ed}
\author[LehighUniversity]{R.~Reed}
\author[FIU]{J.~Reinhold}
\author[LANL]{E.~L.~Renner}
\author[UConn]{J.~Richards}
\author[UIUC]{C.~Riedl}
\author[BNL]{T.~Rinn}
\author[Ohio]{J.~Roche}
\author[MIT]{G.~M.~Roland}
\author[HUJI]{G.~Ron}
\author[IowaState]{M.~Rosati}
\author[UKansas]{C.~Royon}
\author[Pusan]{J.~Ryu}
\author[Rutgers]{S.~Salur}
\author[MIT]{N.~Santiesteban}
\author[UConn]{R.~Santos}
\author[GeorgiaState]{M.~Sarsour}
\author[ORNL]{J.~Schambach}
\author[GWU]{A.~Schmidt}
\author[ORNL]{N.~Schmidt}
\author[GSI]{C.~Schwarz}
\author[GSI]{J.~Schwiening}
\author[RIKEN,RBRC]{R.~Seidl}
\author[UIUC]{A.~Sickles}
\author[UConn]{P.~Simmerling}
\author[Ljubljana]{S.~Sirca}
\author[GeorgiaState]{D.~Sharma}
\author[LANL]{Z.~Shi}
\author[Nihon]{T.-A.~Shibata}
\author[NCU]{C.-W.~Shih}
\author[RIKEN]{S.~Shimizu}
\author[UConn]{U.~Shrestha}
\author[NewHampshire]{K.~Slifer}
\author[LANL]{K.~Smith}
\author[Glasgow,CEA]{D.~Sokhan}
\author[LLNL]{R.~Soltz}
\author[LANL]{W.~Sondheim}
\author[CIAE]{J.~Song}
\author[Pusan]{J.~Song}
\author[GWU]{I.~I.~Strakovsky}
\author[BNL]{P.~Steinberg}
\author[CUA]{P.~Stepanov}
\author[WandM]{J.~Stevens}
\author[PNNL]{J.~Strube}
\author[CIAE]{P.~Sun}
\author[CCNU]{X.~Sun}
%\author[Regina]{K.~Suresh}
\author[AANL]{V.~Tadevosyan}
\author[NCU]{W.-C.~Tang}
\author[IowaState]{S.~Tapia~Araya}
\author[Vanderbilt]{S.~Tarafdar}
\author[BrunelUniversity]{L.~Teodorescu}
\author[UH]{A.~Timmins}
\author[CzechTechUniv]{L.~Tomasek}
\author[UConn]{N.~Trotta}
\author[CUA]{R.~Trotta}
\author[Oslo]{T.~S.~Tveter}
\author[IowaState]{E.~Umaka}
\author[Regina]{A.~Usman}
\author[LANL]{H.~W.~van~Hecke}
\author[IJCLabOrsay]{C.~Van~Hulse}
\author[Vanderbilt]{J.~Velkovska}
\author[IJCLabOrsay]{E.~Voutier}
\author[IJCLabOrsay]{P.K.~Wang}
\author[UKansas]{Q.~Wang}
\author[CCNU]{Y.~Wang}
\author[Tsinghua]{Y.~Wang}
\author[York]{D.~P.~Watts}
\author[CUA]{N.~Wickramaarachchi}
\author[ODU]{L.~Weinstein}
\author[MIT]{M.~Williams}
\author[LANL]{C.-P.~Wong}
\author[PNNL]{L.~Wood}
\author[CanisiusCollege]{M.~H.~Wood}
\author[BNL]{C.~Woody}
\author[MIT]{B.~Wyslouch}
\author[Tsinghua]{Z.~Xiao}
\author[KobeUniversity]{Y.~Yamazaki}
\author[NCKU]{Y.~Yang}
\author[Tsinghua]{Z.~Ye}
\author[Yonsei]{H.~D.~Yoo}
\author[LANL]{M.~Yurov}
\author[York]{N.~Zachariou}
\author[Columbia]{W.A.~Zajc}
\author[USTC]{W.~Zha}
\author[UVA]{J.~Zhang}
\author[Tsinghua]{Y.~Zhang}
\author[IMP]{Y.~X.~Zhao}
\author[UVA]{X.~Zheng}
\author[Tsinghua]{P.~Zhuang}


==> Submit_ArXiv/commands.tex <==
\newcommand{\filenamedot}{.}

\def\consortium{ECCE consortium}
\newcommand{\martinimusic}{\mbox{\sc Martini+Music}\xspace}
\newcommand{\hic}{\mbox{$A$$+$$A$}\xspace}
\newcommand{\pA}{\mbox{$p$$+$$A$}\xspace}
\newcommand{\AuAu}{\mbox{Au$+$Au}\xspace}
\newcommand{\auau}{\mbox{Au$+$Au}\xspace} 
\newcommand{\raa}{\mbox{$R_\mathrm{AA}$}\xspace}
\newcommand{\pbpb}{\mbox{Pb$+$Pb}\xspace} 
\newcommand{\pdau}{\mbox{$p(d)$$+$Au}\xspace} 
\newcommand{\pau}{\mbox{$p$$+$Au}\xspace} 
\newcommand{\aj}{\mbox{$A_J$}\xspace} 
\newcommand {\pp}{\mbox{$p$$+$$p$}\xspace}
\newcommand {\ppbar}{\mbox{$p$$+$$\overline{p}$}\xspace}
\newcommand{\pT}{\mbox{${p_T}$}\xspace}
\newcommand{\jpsi}{\mbox{$J/\psi$}}
\newcommand{\sqrtsnn}{\mbox{$\sqrt{s_{\scriptscriptstyle NN}}$}}
\newcommand{\npart}{$N_\mathrm{part}$}
\newcommand{\ncoll}{$N_\mathrm{coll}$}
\newcommand{\qgp}{\mbox{quark-gluon plasma}\xspace}
\newcommand{\jt}{\mbox{$J_T$}} \newcommand{\qhat}{\mbox{$\hat{q}$}}
\newcommand{\Qsqr}{\mbox{$Q^2$}} \newcommand{\CuCu}{\mbox{Cu$+$Cu}}
\newcommand{\PbPb}{\mbox{Pb$+$Pb}} \newcommand{\pPb}{\mbox{$p$$+$Pb}}
\newcommand{\gjet}{\mbox{$\gamma$-jet}}
\newcommand{\Qmax}{\mbox{$Q_{\max}$}} \newcommand{\ET}{\mbox{$E_T$}}
\newcommand{\Et}{\mbox{$E_T$}} \newcommand{\kt}{\mbox{$k_T$}}
\newcommand{\RAA}{\mbox{$R_{AA}$}\xspace} \newcommand{\IAA}{\mbox{$I_{AA}$}}
\newcommand{\pt}{\mbox{${p_T}$}\xspace}
\newcommand{\highpt}{high-${\rm p_{_{T}}}$}
\newcommand{\lessim}{{\stackrel{<}{\sim}}} \newcommand{\eqnpt}{p_T}
\newcommand{\eA}{\mbox{$e-{\rm A}$}}
\newcommand{\dAu}{\mbox{$d$$+$Au}\xspace}
\newcommand{\pAu}{\mbox{$p$$+$Au}\xspace}
\newcommand{\GeVSQ}{\mbox{${\rm GeV}^2$}}
\newcommand{\fastjet}{\mbox{\sc FastJet}\xspace}
\newcommand{\geant}{\mbox{\sc Geant4}\xspace}
\newcommand{\antikt}{\mbox{anti-$k_T$}\xspace}
\newcommand{\pythia}{\mbox{\sc Pythia}\xspace}
\newcommand{\opera}{\mbox{\sc Opera}\xspace}
\newcommand{\rapgap}{\mbox{\sc Rapgap}\xspace}
\newcommand{\milou}{\mbox{\sc Milou}\xspace}
\newcommand{\pyquen}{\mbox{\sc Pyquen}\xspace}
\newcommand{\hijing}{\mbox{\sc Hijing}\xspace}
\newcommand{\roofit}{\mbox{\sc RooFit}\xspace}
\newcommand{\roounfold}{\mbox{\sc RooUnfold}\xspace}
\newcommand{\beetle}{\mbox{\sc Beetle}\xspace}
\newcommand{\gj}{\mbox{$\gamma$+jet}\xspace}
\newcommand{\gh}{\mbox{$\gamma$+hadron}\xspace}
\newcommand{\martini}{\mbox{\sc Martini}\xspace}
\newcommand{\music}{\mbox{\sc Music}\xspace}

\newcommand{\refdesign}{reference design\xspace}
\newcommand{\refconfig}{reference configuration\xspace}
\newcommand{\dijet}{\mbox{dijet}\xspace}
\newcommand{\fake}{\mbox{fake}\xspace}
\newcommand{\fast}{\mbox{fast}\xspace}
\newcommand{\veryfast}{\mbox{very fast}\xspace}
\newcommand{\epem}{\mbox{$e^+e^-$}\xspace}
\newcommand{\onewidth}{0.6\linewidth}
\newcommand{\twowidth}{0.48\linewidth}
\newcommand{\threewidth}{0.32\linewidth}
\newcommand{\egoing}{\mbox{electron-going}\xspace}
\newcommand{\hgoing}{\mbox{hadron-going}\xspace}
\newcommand{\egodir}{electron-going direction\xspace}
\newcommand{\hgodir}{hadron-going direction\xspace}

\newcommand{\red}{\color{red}}
\newcommand{\blue}{\color{blue}}	 
\newcommand{\green}{\color{green}}	 
\newcommand{\magenta}{\color{magenta}}

\newcommand{\lyxdot}{.}


==> Submit_ArXiv/sections/1_introduction.tex <==
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
\section{Introduction}\label{sec:intro}
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%


The Electron Ion Collider (EIC) \cite{khalek2021science} is a future cutting-edge discovery machine that will unlock the secrets of the gluonic force binding the building blocks of the visibile matter in the universe. The EIC will consist of two intersecting accelerators, one producing an intense beam of electrons and the other a beam of protons or heavier atomic nuclei; it will be the only electron-nucleus collider operating in the world. 
The EIC Comprehensive Chromodynamics Experiment (ECCE) \cite{ecce} is an international consortium assembled to develop a detector that can offer full energy coverage and an optimized far forward detection region.
ECCE has investigated a detector design based on the existing BABAR 1.5T magnet; %solenoid in both EIC interaction points %(namely IP6 and IP8 with 25 and $\sim$35 mrad crossing angle, respectively),
 this detector will be ready for the beginning of EIC operations. 
 More details on the ECCE detector design and what is described in the following can be found in \cite{ecce-paper-det-2022-01}. 

ECCE is an integrated detector that extends for about 40~m, and includes a central detector built around the interaction point and far-forward (hadron-going direction) and far-backward (electron-going direction) regions \cite{khalek2021science}. To fulfill the physics goals of the EIC, the central detector needs to be hermetic and provide good particle identification (PID) over a large phase space. 
The central detector itself consists of multiple sub-detectors: a tracking system made by inner and outer tracker stations allows the reconstruction of charged particles moving in the magnetic field; a system of PID sub-detectors will cover the barrel and the electron-going and hadron-going directions; electromagnetic and hadronic calorimeters are used to detect showers and provide complete information on the particle flow which is essential for certain event topologies, \textit{e.g.}, those containing jets. 
%
%The optimization of the EIC detector is of utmost importance during the design and R\&D phases \cite{ent_eic_schedule_2021}.

As outlined in \cite{khalek2021science}, Artificial Intelligence (AI) can provide dedicated strategies for complex combinatorial searches and can handle multi-objective problems characterized by a multidimensional design space, allowing the identification of hidden correlations among the design parameters. 
ECCE included these techniques in the design workflow during the detector proposal. 
At first this AI-assisted design strategy was used to steer the design. 
%
%After the technology choice is selected (based also on the important insights provided by AI), it can be further utilized to eventually fine-tune the detector parameters. 
After the base technology is selected using insights provided by AI, its detector parameters can be further fine-tuned using AI.  
%
During the ECCE detector proposal stage, the design of the detector underwent a continual optimization process \cite{ent_eic_schedule_2021}. % that evolved in time. %
 %In the following we describe the role played by the AI-assisted workflow and highlight this as a novel aspect introduced during the design process of an experiment.  

%This technical note is therefore structured as follows: in Sec. \ref{sec:ai_assisted} we describe the implemented AI pipeline that supported the design optimization in a sequential strategy the fosters the interplay between the different working groups in a post hoc decision making process; in Sec. \ref{conclusions} we will present our conclusions and provide a summary with future directions. 


The article is structured as follows: in Sec.~\ref{sec:ai_assisted} we provide an overview of design optimization and describe the AI-assisted strategy; 
in Sec.~\ref{sec:simulation} we introduce the ECCE tracker and describe the software stack utilized in this work to which AI is coupled for the optimization;
in Sec.~\ref{sec:analysis} we describe the implemented pipeline that results in a sequential strategy, fostering the interplay between the different working groups in a post hoc decision making process; 
in Sec.~\ref{sec:computing} we present perspectives and planned activities. 

The ECCE detector at the EIC will be one of the first examples of detectors that will be realized leveraging AI during the design and R\&D phases.

%Detector optimization is an essential part of the R\&D and design process that involves mechanical design and budget to realize the best performance possible. This process is anticipated to continue in the months following the detector proposal towards CD-2 and CD-3.



==> Submit_ArXiv/sections/2_AI_assisted.tex <==

%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
\section{AI-assisted Detector Design}\label{sec:ai_assisted}
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%

Detector optimization with AI is 
%an essential part of the ECCE R\&D and design process and it is 
anticipated to continue in the months following the detector proposal towards CD-2 and CD-3. %according to the official EIC schedule \cite{ent_eic_schedule_2021}. 
%
Optimizing the design of large-scale detectors such as ECCE---that are made of multiple sub-detector systems---is a complex problem. 
Each sub-detector system is characterized by a multi-dimensional design parameter space. 
In addition, detector simulations are typically computationally intensive, and rely on advanced simulation platforms used in our community such as \geant \cite{agostinelli2003geant4} to simulate the interaction of radiation with matter.
%
Additional computationally expensive steps are present along the  data reconstruction and analysis pipeline.  
The software stack that is utilized in the detector design process involves three main steps:
(i) generation of events, (ii) detector simulations
and (iii) reconstruction and analysis. 


%Another level of complexity to consider in detector design is the reconstruction of features from the detector response and eventually physics events analysis which allows to build objectives that drive the detector design.  

%%of complexity when it comes to detector design is added by the reconstruction and analysis of events, where certain tasks like pattern recognition for particle identification can be computationally expensive.

As pointed out in \cite{fanelli2022design}, the above bottlenecks render the generation and exploration of mutliple design points cumbersome. 
%
This in turn represents an obstacle for deep learning (DL)-based approaches that learn the mapping between the design space and the functional space \cite{zhou2019optimization,guo2021artificial,sanchez2018inverse}, which could facilitate the identification of optimal design points. 
%
In principle fast simulations with DL can reduce the most CPU-intensive parts of the simulation and provide accurate results \cite{atlas2021atlfast3}, although   several design points need to be produced with \geant before injection in any DL architecture. Similar considerations exist in deploying DL for reconstruction during the design optimization process. 

In this context, a workflow for detector design that has gained popularity in recent years \cite{cisbani2020ai} is represented by the schematic in Fig.~\ref{fig:design_AI}. 
%
\begin{figure}[!]
    \centering
    %\includegraphics[scale = 0.18]{figs/design_workflow.png}
    \includegraphics[width=0.45\textwidth]{figs/design_workflow_2.pdf}
    
    \caption{%(top) 
     \textbf{Workflow of detector design assisted by AI:} physics events are injected in a detector characterized by given design parameters. Reconstructed events are analyzed and figures of merit are quantified and passed to an AI-based strategy, which in turn suggests the next design point in this sequential approach; note that AI can also intervene in the simulation and reconstruction steps. 
    }
    \label{fig:design_AI}
\end{figure}
%
It consists of a sequential AI-based strategy that collects information associated to previously generated design points, in the form of figures of merit (called \textit{objectives} in the following) that quantify the goodness of the design, and which suggests promising new design points for the next iteration. 

The ECCE AI Working Group achieved a continual multi-objective optimization (MOO) of the tracker design. 
%
Our approach deals with a complex optimization in a multidimensional design space (describing, \textit{e.g.}, geometry, mechanics, optics, etc) driven by multiple objectives that encode the detector performance, while satisfying several mechanical constraints. 
This framework has been developed in a way that can be easily extended to other sub-detectors or to a system of sub-detectors. 

The definition of a generic MOO problem can be formulated as follows:
%
\begin{equation}\label{eq:moo}
\begin{aligned}
        min \ \mathbf{f_{m}}(\mathbf{x})  & \ \ \ \ \ \ m = 1, \cdots, M \\
       s.t. \ \ \ \mathbf{g_{j}}(\mathbf{x})\leq 0, & \ \ \ \ \ \ j = 1, \cdots, J \\ 
       \ \ \ \ \  \mathbf{h_{k}}(\mathbf{x})=0,     & \ \ \ \ \ \ k = 1, \cdots, K \\
       x_{i}^{L} \leq x_{i} \leq x_{i}^{U},         & \ \ \ \ \ \ i = 1, \cdots, N \\
\end{aligned}
\end{equation}
%
 where one has $M$ objective functions $f_{m}$ to optimize (\textit{e.g.}, detector resolution, efficiency, costs), subject to $J$ inequalities $g_{j}(x)$ and $K$ equality constraints $h_{k}(z)$ (\textit{e.g.}, mechanical constraints), in a design space of $N$ dimensions (\textit{e.g.}, geometry parameters that change the \geant design) with lower and upper bounds on each dimension.\footnote{Constraints are described later in Table \ref{tab:constraints}.} 
 %
  Notice that overlaps in the design are checked before and during the optimization and are excluded by the constraints and ranges of the parameters.
  %
 In solving these problems, one can come up with a set of \textit{non-dominated} or \textit{trade-off} solutions \cite{debreu1954valuation}, popularly known as Pareto-optimal solutions (see also Fig.~\ref{fig:pareto_front}). 
 %


%
\begin{figure}
    \centering
    %\includegraphics[width=0.21\textwidth]{figs/pareto_front2.png}
    %\includegraphics[width=0.21\textwidth]{figs/hypervolume.png}
    \includegraphics[width=0.5\textwidth]{figs/Pareto_Front2.pdf}
    \caption{\textbf{Example of \textit{Pareto frontier} in a two-dimensional objective space:} The point C is not on the frontier and is dominated by both point A and point B. All the other points which are dominated by the Pareto frontier and that satisfy any constraints in the optimization problem are called \textit{feasible} solutions;
    The hypervolume is used as a metric for convergence, and is calculated with respect to a reference point $r$.
    }
    \label{fig:pareto_front}
\end{figure}

In this setting, we used a recently developed framework for MOO called pymoo \cite{blank2020pymoo} which supports evolutionary MOO algorithms such as Non-Dominated Sorting Genetic Algorithm (or NSGA-II, \cite{deb2002fast}).\footnote{The pymoo framework also supports other MOO approaches and a full list is documented in \cite{blank2020pymoo}.} The rationale behind this choice instead of, for example, principled approaches such as Bayesian Optimization \cite{cisbani2020ai}, emanates from the ECCE needs at the time of the detector proposal, such as the capability to quickly implement and run multiple parallel optimization pipelines implementing different technology choices and the possibility of dealing with non-differentiable objectives at the exploratory stage.  

%
The NSGA workflow is described in Fig.~\ref{fig:NSGA_workflow}.
%
\begin{figure}[!]
    \centering
    %\includegraphics[scale=0.5,trim={0 2cm 0 0},clip]{figs/NSGA_workflow.pdf}
    \includegraphics[width=0.45\textwidth, trim={0 2cm 0 0},clip]{figs/NSGA_workflow.pdf}
    \caption{\textbf{The NSGA Workflow:} At time $t$, an offspring $Q(t)$ is created through a genetic algorithm~\cite{whitley1994genetic} from an $N-$sized population of design points $P(t)$. 
    The two populations are combined into an augmented population which is classified into different non-dominated classes $F_{i}$, starting from the first front $F_{1}$. 
    To restore the initial size of the population, the augmented space of solutions is trimmed. A metric called crowding distance is used to reject solutions and eventually provide an updated population of size $N$ at time $t+1$. 
    %Image taken from \cite{deb2002fast}.
    }
    \label{fig:NSGA_workflow}
\end{figure}
%
The main features of NSGA-II are (i) the usage of an elitist principle, (ii) an explicit diversity preserving mechanism, and (iii) ability of determining non-dominated solutions. 
 %
The latter feature is of great importance for problems where objectives are of conflict with each other: that is an improved performance in an objective results in worse performance in another objective.
%
 %The pymoo framework also supports other MOO approaches and a full list is documented in \cite{blank2020pymoo}. 
 %
 For our purposes, we also tested NSGA-III which is suitable for the optimization of large number of objectives \cite{ishibuchi2016performance}.\footnote{For $\geq$ 4 objectives, NSGA-III is expected to perform better than NSGA-II.}
 
  
%As described in Sec.~\ref{sec:simulation}, the  simulation and reconstruction rely on the Fun4All framework \cite{fun4allGithub}. 
During the design optimization process of the tracking system, we used full \geant simulations of the entire ECCE detector. 
%In Sec.~\ref{sec:analysis} the reader can find a detailed description of the different parametrizations that have been utilized for several optimization pipelines of the inner tracker design optimization.
%
%Eventually the parametrization has been extended to include also the support structure in the design optimization problem.   
%Notice that overlaps in the design are checked before and during the optimization and are excluded by the constraints and ranges of the parameters.
%
%At least three objective functions characterizing the tracker performance (intrinsic detector response such as resolutions and efficiency) have been optimized simultaneously. The different designs have been optimized using particle gun samples of pions; after the optimization we used Pythia \cite{Sjostrand:2006za} samples to evaluate the improvement in the reconstruction of physics events (see Sec. \ref{subsec:physics_analysis}). 
%
AI played a crucial role in helping choose a combination of technologies for the inner tracker and was used as input to multiple iterations of the ECCE tracker design, which led to the current tracker layout. 
%
This was the result of a continual optimization process that evolved in time:
%
results were validated by looking at figures of merit that do not enter as objective functions in the optimization process (more details can be found in Sec. \ref{subsec:validation}); the decision making is left post hoc and discussed among the Computing, Detector and Physics teams.
%Fig.~\ref{fig:pipeline_workflow} displays a flowchart describing this continued optimization process that integrates AI and the interplay between the ECCE teams that took place during the detector proposal. 
A flowchart describing this continual optimization process is shown in Fig.~\ref{fig:pipeline_workflow}. 


 \begin{figure}[!]
    \centering
    \includegraphics[width=0.48\textwidth]{figs/interplay_groups_v3.pdf}
    \caption{
    \textbf{Flowchart of continual optimization during proposal:} AI assists the design optimization process by providing insights and capturing hidden correlations among the design parameters. 
    This has been used during the entire detector proposal process to steer the design. At a given instant in time, N alternative candidate configurations are studied. For each we create an optimization pipeline, which results in a Pareto front of solutions. This new information helps steering the design: some configurations are rejected, while other ones (also dubbed `new references') are identified to potentially improve the design. New optimization pipelines are defined inspired by the new results and the process is iterated. During the design process, AI propelled the fundamental interplay between the ECCE Teams working on Physics, Detector and Computing. 
}
    \label{fig:pipeline_workflow}
\end{figure}


%
%AI provided insights in the design of the ECCE tracker by showing each time by how much the tracking system with different technology choices could be optimized. 
Ultimately this continual AI-assisted optimization led to a projective design after having extended the parametrized design to include the support structure of the inner tracker. The latter represents an ongoing R\&D project that is discussed in the next sections. 



\begin{comment}
An example of these improvements is summarized in Fig. \ref{fig:improved_with_AI}.

\begin{figure}[!ht]
    \centering
    \includegraphics[width=0.45\textwidth]{figs/Proposal_AI_Improvement_2x2.pdf}
    \caption{The momentum dependence of the tracker momentum resolution for the ECCE reference tracker design (ECCE Simulation, blue solid circles) and for the projective mechanical support design of the ECCE ongoing project R\&D that will continue after the proposal (red solid circles). The latter shows a reduction of the impact of readout and services on the tracking resolution in the regions $1<\eta<1.5$ and $-1.5<\eta<1$. Note that the backward region relies on the EM calorimeter, and thus a resolution larger than the PWG requirement is acceptable. 
    \label{fig:improved_with_AI}
    }
\end{figure}
\end{comment}

 % Example of improvement of the ECCE tracker obtained with the AI-assisted design optimization strategy, compared to the 1$^{st}$ simulation campaign: (left) the momentum dependent momentum resolution in $|\eta|$ $<$ 0.5 for the costed ECCE Simulation and for the Projective design described in this section; (right) similarly, in 1.0 $<$ $|\eta|$ $<$ 1.5. The benchmark curve is taken from the Yellow Report and corresponds to an all silicon tracker with a 1.4 T magnetic field; more details can be found in~\cite{khalek2021science}.  

==> Submit_ArXiv/sections/3_simulations.tex <==

%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
\section{ECCE Tracking System Simulation}\label{sec:simulation}
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%

%\subsection{subsec:Software stack}


%\subsection{subsec:ECCE Central Detector }

\begin{figure*}[h!]
    \centering
    \includegraphics[trim=6em 0em 5em 0em, clip, width=0.48\textwidth]{figs/GeomNonProjective_Slanted_V4.pdf}    
    \includegraphics[trim=6em 0em 5em 0em, clip, width=0.48\textwidth]{figs/GeomProjective_Slanted_V4.pdf}
 
    \caption{\textbf{Tracking and PID system in the non-projective (left) and the ongoing R\&D projective (right) designs:} the two figures show the different geometry and parametrization of the ECCE non-projective design (left) and of the ongoing R\&D projective design to optimize the support structure (right). 
    Labels in red indicate the sub-detector systems that were optimized, while the labels in blue are the sub-detector systems that were kept fixed due to geometrical constraint. The non-projective geometry (left) is a result of an optimization on the inner tracker layers (labeled in red) while keeping the support structure fixed, The angle made by the support structure to the IP is fixed at about $36.5\degree$. The projective geometry (right) is the result of an ongoing project R\&D to reduce the impact of readout and services on tracking resolution. 
    }
    \label{fig:ECCE_Tracking_non_proj_and_proj}
\end{figure*}

%“we created a Geant4~\cite{geant4} simulation based on the ECCE detector proposal~\cite{ecce-proposal}. The fun4all framework~\cite{f4a} was used to interface Geant4 with event generators”. And then authors could add another line saying what generator they used and any specific tunes.


The simulation and detector response shown in this document is based on \geant \cite{Agostinelli:2002hh} and was carried out using the Fun4All framework \cite{fun4allGithub, ecce-note-comp-2021-01}. 
%The ECCE-EIC core software utilizes daily, weekly builds and tagged production releases \cite{ecce_eic_sw}. 
%%
%%Development of the framework was driven by reconstruction and analysis needs where the incoming data had to be processed quickly. The framework is extremely modular such that simulations of various detector subsystems can be independently developed and can be integrated within the framework with ease.

%%Fig.~\ref{fig:ECCE_Workflow} represents a schematic of the ECCE Software. 

%Various repositories hold relevant Fun4All analysis code. The macros combine the needed packages into one root script to run jobs. 
%Default macros can run a wide variety of event generators, detector configurations, etc.
%One can pick and choose what to run depending on the analysis needs. The framework also allows the creation of the relevant module and registers it with Fun4All. 



%A wide range of event generators (\textit{e.g.}, HIJING \cite{wang1991hijing}, PYTHIA \cite{sjostrand2008brief}, Sartre \cite{toll2014dipole}, single particle, etc) is supported through the EIC-smear interface and Fun4All. 
The optimization pipelines are based on particle gun samples of pions, where we used $\pi^{-}$ and tested that the performance with $\pi^{+}$ were consistent. Performance in the electron-going direction was also checked post-hoc with particle gun samples of electrons. 
The improved performance is further validated with physics analyses,  using the datasets generated during the ECCE simulation campaigns; in Sec.~\ref{sec:analysis} we show in particular results based on semi-inclusive deep inelastic scattering (SIDIS) events. 


The ECCE tracking detector \cite{ecce-paper-det-2022-03}, represented in Fig. \ref{fig:ECCE_Tracking_non_proj_and_proj} (left), consists of different layers in the barrel and the two end-caps, and is tightly integrated with the PID detectors:

(i) The silicon vertex/tracking detector is an ALICE ITS-3 type high precision cylindrical/disk vertex tracker \cite{ALICEITSproject:2021kcd, colella2021alice}) based on the new Monolithic Active Pixel Sensor (MAPS); the barrel detector consists of 5 MAPS layers; the silicon hadron endcap consists of 5 MAPS disks; and the silicon electron endcap has 4 MAPS disks.

(ii) A gas tracking system is based on $\mu$Rwell technology, that is a single-stage amplification Micro Pattern Gaseous Detector (MPGD) that is a derivative of the Gas Electron Multiplier (GEM) technology. In ECCE $\mu$Rwell layers will form three barrel tracking layers further out from the beam-pipe than the silicon layers; namely, two inner-barrel layers and a single  outer-barrel $\mu$Rwell  layer.   All $\mu$Rwell detectors will have 2D strip based readout. The strip pitch for all three layers will be 400 $\mu$m.

(iii) The tracking system is completed by AC-LGAD-based time of flight (TOF) detectors providing additional  hit information for  track reconstruction as well. In the central region a TOF (dubbed CTTL) is placed behind the high-performance DIRC (hpDIRC); in the hadron-going side a TOF (dubbed FTTL) is placed before the dual RICH (dRICH) and a $\mu$Rwell placed after the dRICH; in the electron-going direction a $\mu$Rwell layer is placed before the modular RICH (mRICH), which is followed by a TOF later (dubbed ETTL).

%The simulation of the ECCE tracking system is shown in Fig.~\ref{fig:ECCE_Tracking_non_proj_and_proj}. %
An important consideration for all large-scale detectors is the provision of readout (power and signal cables) and other services (e.g., cooling). Clearly the aim is to minimize the impact of readout and services in terms of affecting the detector's acceptance or tracking resolution, for example.  This effort is ongoing R\&D for the project. 


In the following sections, the reader can find more details on the implementation of the optimization pipelines and utilized computing resources. 




%\cris{
%The reader can find more details in Fig. \ref{fig:ECCE_Tracking_non_proj_and_proj}, where a comparison between two designs is shown. 

%projective design of the inner tracker obtained with AI after studies have been made to extend the parametrization of the design to the support structure. 
%This design concentrates the material in a smaller dead area resulting in better resolution on a wider range of the pseudo-rapidity. 
%More details on the optimization pipelines, the parametrization, and the detector performance are discussed in Sec.~\ref{sec:analysis}.
%}



%A parallel setup for the tracking system based on the same detector technology described in Sec.~\ref{sec:ecce_tracker} is maintained in a branch of the ECCE software repository and has been proposed with the support of the multi-objective optimization framework developed by the ECCE AI working group \cite{fanelli2021ai}.
%This is a projective design characterized by a conical support structure with a polar angle of 25.5 degrees on both endcaps, see Fig.~\ref{fig:projective_design}. 


%\cris{ %---- start comment 




%As discussed in Sec.~\ref{sec:analysis}, a set of analysis macros has been developed that utilize the final ROOT files produced by the software stack described above. These macros calculate for each design points the values of the objectives and the constraints that need to be encoded in the MOO procedure following Eq.~\eqref{eq:moo}. 
%Following the scheme of Fig.~\ref{fig:design_AI}, the AI optimization is coupled as an additional layer to the software stack to control and distribute new points to simulate based on the results of the analysis of the previously generated points, in a sequential way. 
%These optimization pipelines ran interactively on  nodes of scicomp at Jefferson Laboratory \cite{scicomp}. %% where we distributed the offspring of design points on different physical cores, see Tab.~\ref{tab:complexity}.\footnote{Simulations are currently run single-threaded.}  
%
%Notice that the optimization framework natively supports parallelization with workers using Dask \cite{rocklin2015dask}.
%


%} %---- end comment 






==> Submit_ArXiv/sections/4_analysis_pipeline.tex <==

%\cris{@Joe: Working on polishing Sec. 4.1 and 4.2; feel free to send us comments on these sections too.}

%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
\section{Analysis Workflow}\label{sec:analysis}
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%



The optimization of the ECCE-tracking system \cite{ecce-paper-det-2022-01, ecce-paper-det-2022-03} has been characterized by two main phases during which the sub-detectors composing the tracker evolved into more advanced renditions. 


\paragraph{Phase I optimization}\footnote{Phase I corresponds to a timeline between June-2021 to Sept-2021. Preliminary studies done between March-2021 to May-2021 are not reported here.} The \geant implementation of the detectors were at first simplified, \textit{e.g.}, detector modules were mounted on a simplified conical support structure made of aluminum. 
%The support structure was initially not implemented in the optimization. 
The optimization pipelines consisted of symmetric arrangement of detectors in the electron-going and hadron-going directions (5 disks on each side). The DIRC detector for PID in the barrel region was modelled with a simple geometry made by a cylinder and conical mirrors.
AC-LGAD-based TOF detectors were modelled as simplified silicon disks at first; %more detailed simulations of the outer trackers have been developed during this phase.
the outer trackers had more fine-grained simulations implemented, with realistic support structures and services implemented.
%
The optimization pipelines included various combinations of detector technologies for the inner trackers. At the end of this phase, a decision on the choice of the barrel technology and the disk technologies was made using the AI results. 

%\cris{At the end of this section show the two figures of the non-projective and R\&D projective obtained with this work.}

%\cris{
%The ECCE tracking and PID system during Phase-I is shown in Fig.~\ref{fig:Phase-I_ECCEDetector}, which also displays the non-projective geometry of the support structure. 
%}


\begin{comment}
DIRC bars were simulated. Before that it was a simple cylinder and G4Tub
CTTL, ETTL, FTTL
I am not so sure of the details here but this was fine grained simulations (a new class called as g4ttl/PHG4TTLSubsystem was introduced) ,  But before (phase-1) it was just silicon layers and resembled to that of FSTs (but with 30micron resolution)
uRwell
Mainly had support rings
\end{comment}


\paragraph{Phase II optimization}\footnote{Phase II corresponds to optimization pipelines that run from Sept-2021 to Nov-2021.} 
%
These pipelines had a more realistic implementation of the support structure incorporating cabling, support carbon fiber, cooling system, etc. 
More detailed simulation of the PID Detectors (\textit{e.g.}, DIRC bars and dRICH sub-systems) were integrated as well as fine-grained simulations of TTL layers (CTTL, ETTL, FTTL) previously simulated as simple silicon layers modules. %
More stringent engineering constraints were considered such as the sensor size for MAPS detector (ITS3). This phase also considered an asymmetric arrangement of the detectors in the endcap regions, with a maximum of 4 EST disks in the electron-going end-cap and 5 FST disks in the hadron-going endcap: 
%The placement of detectors in the endcap regions are asymmetric for the pipelines that were done during Phase-II. 
due to this asymmetric spatial arrangement, the angle subtended by detectors in the two endcap regions could be varied. %An optimization was carried out with asymmetric spatial arrangement of EST and FST disks. 
This eventually developed into the idea of a projective geometry in a pipeline that characterizes an ongoing R\&D project for optimizing the design of the support structure. 


A detailed description of the most recent parametrization used for the detector proposal can be found in \ref{app:par_tracking}, 
%Such parametrization has been used for the optimization of the non-projective design, which had the inner tracker support structure fixed. 
 along with the parametrization used in an ongoing R\&D project to optimize the support structure of the inner tracker. %;
 %has been modified to explore the possibility of including in the optimization the design of the support structure. This resulted in the R\&D project always described in \ref{app:par_tracking}; 
% a schematic representation is displayed in Fig.~\ref{fig:SupportStructureparametrization}. 

Fig.~\ref{fig:ECCE_Tracking_non_proj_and_proj} shows a comparison of the ECCE reference non-projective design and the projective design from the ongoing R\&D, both of which resulted from the AI-assisted procedure described in this paper.

\begin{comment}
\begin{figure*}[!]
    \centering
    \includegraphics[trim=6em 0em 5em 0em, clip, width=0.48\textwidth]{figs/GeomNonProjective_Slanted_V4.pdf}    
    \includegraphics[trim=6em 0em 5em 0em, clip, width=0.48\textwidth]{figs/GeomProjective_Slanted_V4.pdf}
 
    \caption{\textbf{Tracking and PID system in the non-projective (left) and the ongoing R\&D projective (right) designs:} the two figures show the different geometry and parametrization of the ECCE non-projective design (left) and of the ongoing R\&D projective design to optimize the support structure (right). 
    Labels in red indicate the sub-detector systems that were optimized, while the labels in blue are the sub-detector systems that were kept fixed due to geometrical constraint. The non-projective geometry (left) is a result of an optimization on the inner tracker layers (labeled in red) while keeping the support structure fixed, The angle made by the support structure to the IP is fixed at about $36.5\degree$. The projective geometry (right) is the result of an ongoing project R\&D to reduce the impact of readout and services on tracking resolution. 
    }
    \label{fig:ECCE_Tracking_non_proj_and_proj}
\end{figure*}
\end{comment}


%\cris{Details on the parametrizations can be found; mention projective. 
%In what follows...}

%A new implementation of the framework was needed for Phase-II given the  more realistic simulation of the detectors and the more stringent engineering constraints that have been considered.  

%The procedure to optimize the ECCE-tracking system involves a complex parameterization of various detector systems. 



%The implementation of the simulation setup for the projective geometry of the inner tracker is explained in detail in this section. The ECCE tracking and PID systems are shown in Fig. \ref{fig:ECCE_TrackingPID_Detailed}.


%\cris{The parametrization was more complex for some of the previous pipelines which were run during the process of optimization. --- Improve text. It is unclear. }



%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
\subsection{Encoding of Design Criteria}\label{subsec:encoding}
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%

%\cris{Talk about only phase-II optimization; phase I mention only it had a symmetric parametrization and perhaps point to the analysis note for details. This reduces also the tables later.}

Design criteria need to be encoded to steer the design during the optimization process. 
For each design point we need to compute the corresponding objectives $f_m$, namely the momentum resolution, angular resolution, and Kalman filter efficiency.  


We will refer in the following only to the more recent Phase II optimization.\footnote{Similar considerations apply also for Phase I optimization.} 
Phase II has been characterized by two types of optimization pipelines: the first used a parametrization of the inner tracker during the optimization process and led to the ECCE tracker non-projective design; the second branched off the first as an independent R\&D effort that included the parametrization of the support structure and led to a projective design.


Details on the two types of optimization pipelines can be found in the following tables: 
Table~\ref{tab:hyperparameters} describes the main hyperparameters and the dimensionality of the optimization problem, in particular of the design space and the objective space;  Table~\ref{tab:ranges} reports the range of each design parameter\footnote{The design points are normalized in the range [0-1], using a min-max scaler $x_{i} = x (x_{max} - x_{min}) + x_{min}$, where $x_i$ is the normalized design point with a un-normalized design point $x$ generated between the range $[x_{min}, x_{max}]$.};
Table~\ref{tab:constraints} summarizes the constraints for both the non-projective and projective geometries. 
We also considered in our design a safe minimum distance between the disks of 10 cm and include a constraint on the difference between the outer and inner radii of each disk, namely R$_{out}$ - R$_{in}$, to be a multiple of the sensor cell size (17.8 mm $\times$ 30.0 mm), see Table~\ref{tab:constraints}.
These constraints are common to the non-projective and the projective designs.
For more details on the parametrizations and on the corresponding detector performance the reader can refer to \ref{app:par_tracking} and  \ref{app:comparison}, respectively. 
%In what follows we provide a thorough description of the design criteria that have been encoded in the optimization strategy. 


%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%

\begin{table}[!bh!]
   
    \centering
    \begin{tabular}{|M{3.cm} | M{1.5cm}| M{2.0cm}|}
        \hline
        \textbf{description} & \textbf{symbol} & \textbf{value}\\ 
        \hline
        \hline
        \small{population size} & N & 100 \\
        \small{\# objectives}   & M & 3\\ 
        \small{offspring} & O & 30\\
        \small{design size} & D & 11 (9) \\
        \small{\# calls (tot. budget)} & $-$ & 200\\
        \small{\# cores} & $-$ & \small{same as offspring} \\
        \small{\# charged $\pi$ tracks} & N$_{\textup{trk}}$ & 120k\\
        \small{\# bins in $\eta$} & N$_{\eta}$ & 5\\
        \small{\# bins in p} & N$_{\textup{p}}$ & 10\\
        \hline
    \end{tabular}
    \caption{\textbf{Summary of the hyperparameters of the design optimization:}
    the values reported in the table have been used during the optimization of the non-projective design of the ECCE tracker. For completeness and when they differ from the non-projective case, we also report in parentheses the values corresponding to the ongoing R\&D project for the projective design of the support structure. 
    \label{tab:hyperparameters}
    }
    
\end{table}

\begin{comment}
\begin{table}[!]
    \centering
    \resizebox{\columnwidth}{!}{%
    \begin{tabular}{M{2.5cm}|M{3.cm}|M{3.cm}|M{3.5cm}}
        \hline
        & \textbf{design pars} &  \textbf{objectives}\\
        \hline
        \hline
           %\textbf{\#} &  4(11) &  3 (4) &  4(5) %\\
        %\hline
           \textbf{ECCE tracker design (non-projective)} & \small{
           %(Phase-I symmetric design) 5 disks $z$-location (hadron endcap) and 6 barrel layers radii;
           5 disks $z$ (hadron endcap) and 4 disks $z$ (electron end cap) location,  2 $\mu$Rwell layers Radius} & \small{momentum resolution; angular resolution; Kalman filter efficiency; (pointing resolution)}
            \\
        \hline
        \hline
           \textbf{ECCE ongoing R\&D design (projective)} & \small{Angle Tracking Support ($\theta$), 2 TTL $z$-location, 1 uRwell-1 Radius, 3 FST disks, 2 EST disks (9 parameters);} & \small{momentum resolution; angular resolution; Kalman filter efficiency; (angular resolution at dRICH; pointing resolution)}
           %\cris{larger! It was smaller...} 
           \\
        \hline
        \hline
        
    \end{tabular}
    }
    \caption{ \textbf{Dimensionality of the optimization pipelines:} 
    Notice that two additional constraints are implicitly taken into account, that is: (i) the inner radii of the disks in the endcap and the inner vertex layer in the barrel have to be compatible with the beam envelope dimensions; (ii) the barrel layers lengths and the outer radii of the disks have to be compatible with an Al-shell support structure provided by the LBNL design \cite{arrington2021eic}. Conditions (i) and (ii) are provided by internal parametrization and reflected in the \geant design. Potential overlaps among modules are checked before and during the optimization. Also, additional objectives that were used as a part of exploration are given in parenthesis.
    \cris{Just drop it?}
    }
    \label{tab:dimensionality}
\end{table}
\end{comment}

%
\begin{table}[!]
    \centering
    %\resizebox{\columnwidth}{!}{
    \begin{adjustbox}{width=0.9\columnwidth}
    %\begin{tabular}{| c | c | c |}
    \begin{tabular}{|M{5.cm}|M{3.5cm}|}
        \hline 
        \rowcolor{blue!15}\multicolumn{2}{|c|}{  \textbf{ECCE design (non-projective)}}\\
        \hline
        \textbf{Design Parameter} & \textbf{Range} \\
        \hline
        $\mu$RWELL 1 (Inner) ($r$) Radius  & [17.0, 51.0 cm] \\
        \hline
        $\mu$RWELL 2 (Inner) ($r$) Radius  & [18.0, 51.0 cm] \\
        \hline
        EST 4 $z$ position &   [-110.0, -50.0 cm] \\
        \hline
        EST 3 $z$ position &   [-110.0, -40.0 cm] \\
        \hline
        EST 2 $z$ position &   [-80.0, -30.0 cm] \\
        \hline
        EST 1 $z$ position &   [-50.0, -20.0 cm] \\
        \hline
        FST 1 $z$ position &  [20.0, 50.0 cm] \\
        \hline 
        FST 2 $z$ position &  [30.0, 80.0 cm] \\
        \hline
        FST 3 $z$ position &  [40.0, 110.0 cm] \\
        \hline
        FST 4 $z$ position &  [50.0, 125.0 cm] \\
        \hline
        FST 5 $z$ position &  [60.0, 125.0 cm] \\
        \hline
        \rowcolor{blue!15}\multicolumn{2}{|c|}{  \textbf{ECCE ongoing R\&D (projective)}}\\
        \hline
        \textbf{Design Parameter}  & \textbf{Range} \\
        \hline
        Angle (Support Cone)   & [25.0$\degree$, 30.0$\degree$] \\
        \hline
        $\mu$RWELL 1 (Inner) Radius  & [25.0, 45.0 cm] \\
        \hline
        ETTL $z$ position  & [-171.0, -161.0 cm] \\
        \hline
        EST 2 $z$ position  & [45, 100 cm] \\
        \hline
        EST 1 $z$ position  & [35, 50 cm] \\
        \hline
        FST 1 $z$ position  & [35, 50 cm] \\
        \hline 
        FST 2 $z$ position  & [45, 100 cm] \\
        \hline
        FST 5 $z$ position  & [100, 150 cm] \\
        \hline
        FTTL $z$ postion  & [156, 183 cm] \\
        \hline
        
    \end{tabular}
    \end{adjustbox}
    \caption{\textbf{Ranges of the design parameters:}  the table summarises the design points that are optimized for the non-projective and the projective case. The optimization range is also given for each parameter. The parameters corresponding to the non-projective case were optimized sequentially over at least three iterations, with each iteration having a set of parameters fixed. For instance, the EST/FST disks were optimized during the first iteration assuming symmetric design, and for the subsequent iterations the EST disks were optimized further in the electron endcap region.  
    %The other geometric parameter for each of the detector systems are calculated based on the parametrization discussed above. 
    Along with the design parameters the design comes with geometrical constraints too. 
    These are implemented as strong and soft constraints in the Table \ref{tab:constraints}. 
    \label{tab:ranges}
    }
\end{table}

\begin{table}[!]
    \centering
    \resizebox{\columnwidth}{!}{%
    \begin{tabular}{|M{3.0cm}|M{5.7cm}|M{4.8cm}|}
        \hline
         \textbf{sub-detector} & \textbf{constraint} & \textbf{description} \\
        \hline
        \hline
        EST/FST disks  & %$\sum_{i} \frac{(RMax_{i} - RMin_{i})}{L} = \mathbb{N}$ 
        
        $$min \Bigg\{ \sum_{i}^{disks} \Bigg| \frac{R^{i}_{out} - R^{i}_{in}}{d} - \floor*{\frac{R^{i}_{out} - R^{i}_{in}}{d}} \Bigg| \Bigg\}$$
        
        & \textbf{soft constraint}: sum of residuals in sensor coverage for disks; sensor dimensions: $d$ = 17.8 (30.0) mm\\
        \hline 
        
        %FST/EST Disks & $\sum_{i} \frac{(RMax_{i} - RMin_{i})}{1.8} = \mathbb{N}$ & MAPS sensor width is 1.78 cm. Soft Constraint\\
        \hline
        EST/FST disks & $z_{n+1} - z_{n} >= 10.0$ cm & \textbf{strong constraint}: minimum distance between 2 consecutive disks   \\
        %
        \hline
        sagitta layers & $$ min\Bigg\{ \Bigg| \frac{2 \pi r_{sagitta}}{w} - \floor*{\frac{2 \pi r_{sagitta}}{w}} \Bigg| \Bigg\}$$ &  \textbf{soft constraint}: residual in sensor coverage for every layer; sensor strip width: $w$ = 17.8 mm\\
        %
        \hline
        $\mu$RWELL & $r_{n+1} - r_{n} >= 5.0$ cm &  \textbf{strong constraint}: minimum distance between $\mu$Rwell barrel layers\\
        \hline
        
    \end{tabular}
    }
    \caption{\textbf{Constraints in the design optimization:} the table summarises constraints for both the projective and the non-projective designs. 
    %The constraints are from the FST/EST disks since they are made by tiling up MAPS pixels. 
    %The pixels will have fixed dimensions. 
    Soft constraints are constraints that can be violated to a certain degree by the MOO and then one can quantify the degree of unfeasibility (see \cite{blank2020pymoo}). Also, minor adjustments on tiling up the pixels can be done post hoc optimization such that the detector geometry is realisable. Strong constraints during the optimization designs rest in high penalties since these constraints cannot be violated. %\textit{e.g.}, the distance between the disks cannot be closer than 10 cm for servicing requirement.
    %The constraints in this table are common to all designs.
    Two additional constraints are implicitly taken into account by internal parametrization and reflected in the \geant design: the inner radii of the disks in the endcap and the inner vertex layer in the barrel have to be compatible with the beam envelope dimensions; the barrel layers lengths and the outer radii of the disks have to be compatible with an tracking support structure \cite{arrington2021eic}. %These are provided by internal parametrization and reflected in the Geant4 design.
    Potential overlaps among modules are checked before and during the optimization.
    }
    \label{tab:constraints}
\end{table}

%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%

The objectives depend on the kinematics and are calculated in 5 main bins in pseudorapidity ($\eta$):  (i) -3.5 $ \leq \eta < $ -2.0 (corresponding to the  electron-going direction), (ii) -2.0 $ \leq \eta <$ -1.0 (the transition region in electron-going direction), (iii) -1 $ \leq \eta <$ 1 (the central barrel),  (iv) 1 $ \leq \eta <$ 2.0 (the transition region in the hadron-going direction) and (v) 2.0 $ \leq \eta <$ 3.5 (the hadron-going direction). 
 %
The rationale behind this binning is a combination of different aspects: the correspondence with the binning in the EIC Yellow Report \cite{khalek2021science}, the asymmetric arrangement of detectors in electron-going and hadron-going directions and the division in pseudorapidity between the barrel region and the endcap. %\footnote{A finer binning is of course possible but it comes at an increase of computing time needed to run the simulations.} 
%
Particular attention is given to the transition region between barrel and endcaps as well as at large $|\eta| \sim$ 3.5 close to the beamline. 

Charged pions are generated uniformly in the phase-space that covers the range in momentum magnitude $p$~$\in$~[0,20]~GeV/c and the range in pseudorapidity $\eta$~$\in$~(-3.5,3.5). 
Each bin in $\eta$ is further subdivided in 15 bins in momentum $p$. 
%
%Studies have been performed to determine the number of tracks (N$_{trk}$) that we need to simulate in order to get sufficiently small statistical uncertainty
 For each design point we simulated N$_{trk}=$120k charged pions.\footnote{From Phase I to Phase II, the design became asymmetric in the two endcaps, therefore we needed to extend the $\eta$-coverage and increase the statistics. The momentum range was reduced to [0,20] GeV/c to optimize the computing budget.} 
This number ensured large enough statistics over the entire phase space and the stability of the fits in all of the bins of Eqs.~\eqref{eq:objectives_reso}.


In order to calculate the relative momentum (cf. Fig.~\ref{fig:Phase-II_Momentum_res}) and absolute angular resolution (cf. Fig~\ref{fig:Phase-II_dth_res}) we fit the following objectives: 

\begin{equation}\label{eq:obj_definition}
\begin{split}
    \frac{\Delta p}{p} &= \frac{p_{reco}-p_{true}}{p_{true}} \\ 
    \Delta \theta  &= \theta_{reco}-\theta_{true} 
\end{split}
\end{equation}


\begin{comment}
To calculate the angular resolution at the PID location (cf. Fig.~\ref{}) we do fit the following objectives:

\begin{equation}\label{eq:obj_definition_PID}
\begin{split}
    d\phi_{proj} &= \tan^{-1}{\Big(\frac{(\Vec{p}_{reco} - \Vec{p}_{true}) \cdot (\Vec{p}_{true}\times \Vec{z}) \times \Vec{p}_{true}}{|\Vec{p}_{true}| |(\Vec{p}_{true}\times \Vec{z}) \times \Vec{p}_{true}|}\Big)} \\ 
   d\theta_{proj} &= \tan^{-1}{\Big(\frac{(\Vec{p}_{reco} - \Vec{p}_{true}) \cdot (\Vec{p}_{true}\times \Vec{z})}{|\Vec{p}_{true}| |(\Vec{p}_{true}\times \Vec{z})|}\Big)} \\
   \Vec{p}_{true} &= True~\Vec{p}~at~PID \\
   \Vec{p}_{reco} &= Reconstructed~\Vec{p}~at~PID
\end{split}
\end{equation}
\end{comment}

Following the definitions of Eq.~\eqref{eq:obj_definition}, histograms of the relative momentum resolution and the absolute angular resolution are produced for each bin in $\eta$ and $p$ and the corresponding fits are calculated. % as shown in Fig.~\ref{fig:fit_results}.
%
Using single-Gaussian (SG) fits (also utilized in the Yellow Report \cite{khalek2021science}) implies systematically better resolutions but worse reduced $\chi^{2}$: therefore we decided to utilize double-Gaussian (DG) fits, as shown in Fig.~\ref{fig:double_gauss}. 
This provided a more robust fit strategy. 
The reduced $\chi^{2}$ range with DG fits ranges from 1.2 to 2.8 at most, with the majority of the fits stable at lower values. 
%
The largest numbers correspond either to the transition between the barrel and endcaps---where tracks cross more material in the non-projective design---or to large pseudorapidity, particularly close to the inner radii of the disks. By using SG fits, the reduced $\chi^{2}$ values can be as large as 10-20 in the transition region. A detailed study comparing SG to DG fits is shown in Fig.~\ref{fig:Phase-II_Momentum_res}.


\begin{figure}[!]
    \centering
    %\includegraphics[scale = 0.23]{figs/double_gaussian.png}
    %\includegraphics[width = 0.4\textwidth]{figs/analysis/dpp_9.pdf}
    \includegraphics[width = 0.4\textwidth]{figs/snapshot_double_gauss.png}
    \caption{\textbf{Fit strategy: } a double-Gaussian fit function is utilized to extract the resolutions. Such a fit function provided good reduced $\chi^{2}$ and more stable extractions compared to single-Gaussian fits. The resolution is obtained as an average of the two $\sigma$'s weighted by the relative areas of the two Gaussians according to Eq.~\eqref{eq:DG}. The figure represents the results corresponding to a particular bin in $\eta$ and $p$. 
    }
    \label{fig:double_gauss}
\end{figure}


The final DG resolution has been defined as an average of the two $\sigma$'s weighted by the relative areas of the two Gaussians:\footnote{A different definition could be based on the weighted average of the variances $\sigma_{1,2}^{2}$ to obtain the final variance $\sigma_{DG}^{2}$. This typically implied a few \% relative difference on the final value of $\sigma_{DG}$ which has been considered a negligible effect.}
%
\begin{equation}\label{eq:DG}
    \sigma_{DG} \sim \frac{A_{1}\sigma_{1}+A_{2}\sigma_{2}}{A_{1}+A_{2}}
\end{equation}

The results obtained for the resolutions in each bin corresponding to each new design point are divided by the values corresponding to the baseline design, so that in each bin a ratio $R(f)_{p,\eta}$ is provided. 
Finally a weighted sum of these ratios is performed to build a global figure of merit (for both the relative momentum and the angular resolutions):  
%
\begin{equation}\label{eq:objectives_reso}
    R(f) = \frac{1}{N_{\eta}}\sum_{\eta} \left( \frac{\sum_{p} w_{p,\eta} \cdot R(f)_{p,\eta}}{\sum_{p} w_{p,\eta}} \right)
\end{equation}
%
where the objective function $f$ is either the momentum or the angular resolution described by Eq.~\eqref{eq:obj_definition}, and the weight $w_{p,\eta} = 1/\sigma^{2}(f_{p,\eta})$ is calculated in each $\eta, p$ bin and it is proportional to the inverse of the variance corresponding to the objective functions $f$.
%%either Eq.~\eqref{eq:obj_definition_PID} or

An additional objective function has been included in the optimization problem: this is a global objective function corresponding to the fraction of tracks that are not reconstructed by the Kalman filter (KF \cite{FRUHWIRTH1987444}), or equivalently the KF inefficiency:
%
\begin{equation}\label{eq:objective_KF}
    R(\textup{KF}) = \frac{\textup{N(tracks \ not \ reconstructed)}}{\textup{N(total number of tracks)}}
\end{equation}
%

Following the above definitions, the design problem corresponds to minimizing the objective functions defined in Eqs.~\eqref{eq:objectives_reso}, \eqref{eq:objective_KF}: a weighted average ratio smaller than one and a KF inefficiency as close as possible to zero correspond to an improvement in performance compared to the baseline design.
%; as for the KF inefficiency, we ideally want to find a design point that pushes this value as close as possible to zero. 



%\vspace{5cm}

%\clearpage
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%\subsection{Results}
\subsection{Convergence and Performance at Pareto Front}
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%


%-------------------------------------------
%\paragraph{Convergence and Pareto solutions:}
%
 We remind the reader that the Pareto front is the set of trade-off solutions of our problem. Fig.~\ref{fig:convergence} shows the convergence plot obtained utilizing the hypervolume as metric in the objective space.\footnote{Early stopping can occur if no change in the hypervolume is observed after a certain number of evaluations.} A petal diagram is used to visualize the values of three objectives corresponding to one of the solutions extracted from the Pareto front. 
 
\begin{figure}[!]
    \centering
    \includegraphics[width=0.48\textwidth]{figs/MOGA_PerformanceMetric.pdf}
    \caption{\textbf{Metric for convergence and performance at Pareto front:} (left) The hypervolume can be used as a metric for convergence. Checkpoints are created during the optimization and snapshots of the evolving designs are saved. (right) A petal diagram with the three objectives corresponding to one solution in the Pareto front. The momentum and angular resolutions are expressed as ratios with respect to a baseline design to improve; the KF inefficiency is taken as an absolute value. An optimal design optimizes all of the above defined objectives. 
}
    \label{fig:convergence}
\end{figure}

Checkpoints are created to store the NSGA-II-updated population of design points. A survey of the detector performance is created after each call to monitor potential anomaly behavior of the fits. 
%
The fitting procedure is quite stable: if an exception occurs the analysis has been automated to adjust the fitting parameters and ranges. In case of persistent anomalous behavior a flag is raised, the critical design point purged from the population and examined.  

%A two-level parallelization is implemented to speed-up the computation time as explained in Sec.~\ref{subsec:computing}.



%A comparison between the non-projective and projective designs of the inner tracker is also shown in Fig.~\ref{fig:tracking_projective}, where the projective design concentrates the material in a smaller dead area resulting in better resolution on a wider range of the pseudorapidity.
%

The improvement obtained with the continual multi-objective optimization process is summarized in Fig. \ref{fig:continued_optimization}, where the momentum resolution obtained during phase-I optimization using a preliminary detector concept is compared to both the non-projective and the projective R\&D designs which are instead derived from fully developed simulations in phase-II optimization.

\begin{figure*}[!]
    \centering
    \includegraphics[width=0.245\textwidth]{figs/OptimizationResultsMomentumCompare_dp_p_p_eta_0.pdf}
    \includegraphics[width=0.245\textwidth]{figs/OptimizationResultsMomentumCompare_dp_p_p_eta_1.pdf}
    \includegraphics[width=0.245\textwidth]{figs/OptimizationResultsMomentumCompare_dp_p_p_eta_2.pdf}
    \includegraphics[width=0.245\textwidth]{figs/OptimizationResultsMomentumCompare_dp_p_p_eta_3.pdf}
    \caption{\textbf{Evolution of momentum resolution driven by the continued MOO:} Momentum resolutions in four bins of $\eta$. From left to right, respectively: $|\eta|<$ 1.0 corresponding to the barrel, 1.0 $|\leq \eta<|$ 1.5 corresponding to the transition region, and 1.5 $\leq |\eta| <$ 2.5 and 2.5 $\leq \eta <$ 3.5 corresponding to the two end-caps. Black points represent the first simulation campaign, and a preliminary detector concept in phase-I optimization which did not have a developed support structure; blue points represent the fully developed simulations for the final ECCE detector proposal concept; red points the ongoing R\&D for the optimization of the support structure. Compared to black, there is an improvement in performance in all $\eta$ bins with the exception of the transition region, an artifact that depends on the fact that black points do not include a realistic simulation of the material budget in the transition region. In the transition region, it can be also appreciate the improvement provided by the projective design. %\cris{polish text; reference in the document; move figures and reduce blank spaces}
    }
    \label{fig:continued_optimization}
\end{figure*}

A detailed description of the optimized performance for all the objectives (momentum, angular resolutions and Kalman Filter efficiency) can be found in~\ref{app:comparison}.



%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
\subsection{Physics Analysis}\label{subsec:physics_analysis}

To show a comparison in physics performance between the non-projective and projective designs, we analysed ${D}^{0}$ meson decay into $\pi^{+}K^{-}$. 
Data have been produced utilizing SIDIS events generated with Pythia6 \cite{Sjostrand:2006za},  corresponding to $ep$ events with 18 GeV $\times$ 275 GeV and high Q$^{2}$.\footnote{production: prop.5/prop.5.1;  generator: pythia6; kinematics: ep-18x275-q2-high. More info can be found in \cite{ecce_simulation_WG}.} 

In Fig.~\ref{fig:physics_analysis_DSCB}, the $\pi^{+}K^{-}$ invariant mass is fitted with a double-sided Crystal Ball function \cite{aaboud2016search,lhcb2020first}. 

\begin{figure}[!]
    \centering
    \includegraphics[width=0.48\textwidth]{figs/D0_Pi+K-_DSCBFunc.pdf} 
    \caption{\textbf{Analysis of SIDIS events with AI-assisted detector designs: } The $\pi^{+}K^{-}$ invariant mass obtained from the SIDIS events reconstructed in ECCE. A comparison of the resolution on the ${D}^{0}$ meson obtained with the non-projective and the projective design of the ECCE tracker is shown. 
    In order to emphasize the improvement in the region between $1.0 < |\eta| < 1.5$, a selection was made such that both the tracks $\pi^{+}$ or the $K^{-}$ are within the region of interest. The resolution with the projective design is improved by more than 10\% relative to the resolution obtained with the non-projective design. 
    \label{fig:physics_analysis_DSCB}
    }
\end{figure}

The decay events are selected in such a way to have at least one particle (either $\pi$ or $K$, or both) in the pseudorapidity bin 1.0$<$$|\eta|$$<$1.5, where the projective design is expected to improve the performance by concentrating all the material in a smaller dead area compared to the non-projective design. 

The analysis shows that the resolution obtained with the projective design is improved by more than 10\% relative to that obtained with the non-projective design. 
We also calculate the efficiency, defined as the number of reconstructed ${D}^{0}$ mesons divided by the number of true ${D}^{0}$ mesons. 
The efficiency obtained with the two designs  is consistent within the statistical uncertainties. 












==> Submit_ArXiv/sections/5_computing.tex <==

\section{Computing Resources}\label{sec:computing}



%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%\subsection{Computing Resources}\label{subsec:computing}
\paragraph{Parallelization}
%
A two-level parallelization has been implemented in the MOO framework: the first level creates the parallel simulations of design points, the second level parallelizes each design point (see Fig.~\ref{fig:parallelization}). 
%
The evaluation itself can be distributed to several workers or a whole cluster with libraries like Dask \cite{dask}.

\begin{figure}[!]
    \centering
    \includegraphics[width=0.48\textwidth]{figs/full_parametrization-new2.pdf}
    \caption{\textbf{Flowchart of the two-level parallelization implemented for detector design:}  Multiple design points are produced in parallel, and each design point is parallelized. The design is assisted by an AI-strategy, in this case MOO with evolutionary algorithms supported by pymoo \cite{blank2020pymoo}.
    \label{fig:parallelization}
    }
\end{figure}

%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
\paragraph{Computing Budget}
%
Computing time studies have been carried out to evaluate the simulation time of each single design point as a function of the number of tracks generated. 
We made this study with simulations that included the tracking system and the PID system and estimated an effective simulation time of 0.2 s/track after removing an initial latency time. 
Similarly we made studies of the computing time taken by the AI-based algorithm in generating a new population of design points. 
Results of these studies are summarized in Fig.~\ref{fig:computing-times}.  

A larger population allows to approximate the Pareto front with larger accuracy. Extension of the design parameter space and the objective space to larger dimensionality implies a larger amount of CPU time which is mainly dominated by simulations if the population size remains smaller than 10$^{4}$--10$^{5}$, see Fig.~\ref{fig:computing-times}. 
%An interesting trend in recent years when the sorting time becomes dominant compared to simulations is that of implementing evolutionary MOO in supercomputers (see, \textit{e.g.}, \cite{liu2020parallelization}). 

For our goals the optimization pipelines of the ECCE tracking system were parametrized with 10--20 design parameters and 3--4 objectives; this allowed us to achieve good convergence with evolutionary MOO using a two-level parallelization strategy, and deployment on single nodes of 128 CPU cores available on the sci-comp farm at Jefferson Lab \cite{scicomp}.\footnote{Work is in progress to efficiently distribute the optimization pipeline to multiple nodes.}.
%
\begin{figure}[h!]
    \centering
    %\includegraphics[width=0.2\textwidth]{figs/TimeHistROOT.pdf}
    \includegraphics[trim=7.5em 0em 7.8em 0em, clip, width=0.45\textwidth]{figs/PyMOOTimeStudy_V4.pdf}
    \caption{\textbf{The computing time taken by the genetic algorithm and the sorting in NSGA-II:}. Performance has been benchmarked with test problems like DTLZ1 \cite{ishibuchi2016performance} (red points) and the scaling $\sim MN^{2}$ (see Table~\ref{tab:hyperparameters}) has been verified with convergence to the Pareto front. The simulation time dominates the AI time during the optimization process (blue point). A two-level parallelization has been introduced in the framework to reduce this bottleneck.  
    The AI contribution typically becomes dominant when very large population size is needed to accurately approximate the Pareto front (cf.\cite{liu2020parallelization}). 
}
    \label{fig:computing-times}
\end{figure}


%\paragraph{Estimated Resources}





\paragraph{Planned Activities}
%
As described in this document, detector optimization with AI is an essential part of the R\&D and design process and it is anticipated to continue after the detector proposal.
%
%AI assisted in steering the design of the ECCE Tracker and can be utilized to fine-tune its design.
%Activities in this regard are anticipated to further extend the parametrization of the ECCE tracker. 
%
The AI-assisted design optimization of the ECCE inner tracker was based on evolutionary algorithms. During the detector proposal multiple optimization pipelines were run each with a population size of 100, representing different detector design configurations. At each iteration, AI updated the population. The total computing budget for an individual pipeline amounted to approximately 10k CPU-core hours. 
This number depends on the dimensionality of the problem.
%
Larger populations may need to be simulated to cope with the increased complexity in order to improve the accuracy of the approximated Pareto front. Different AI-based strategies will be compared. 

Activities are planned to continue the detector optimization: new optimization pipelines can deal with a larger parameter space to include a system of sub-detectors such %as the whole ECCE tracker 
 or to combine tracking and PID in the optimization process. We also plan to optimize other sub-detectors like, \textit{e.g.}, the dRICH, leveraging on the expertise internal to the ECCE collaboration regarding specifically the design of the dRICH with AI-based techniques \cite{cisbani2020ai}. 
%
%For the tracker we used as driving criteria figures of merit that embody the performance of the tracking detector: momentum and angular resolution, Kalman filter efficiency. 
%After the detector optimization, we validate the performance on other figures of merit not utilized during the optimization process.
%We also completed these studies by analysing the performance of the optimized detector on physics channels, particularly we made an analysis of the $D^{0}\rightarrow \pi^{+}K^{-}$ that showed an improved resolution by at least 10\% with the projective tracker design as compared to the non-projective geometry. 
As a future activity we aim to encode physics-driven objectives in the MOO problem. 
%
A thorough comparison of results obtained with different AI-based strategies (\textit{e.g.}, MOO based on genetic algorithms or bayesian approaches) can be also studied. 

We anticipate for 2022 roughly 1M CPU-core hours for these activities.



==> Submit_ArXiv/sections/acknowledgments.tex <==
\section*{Acknowledgements}
\label{acknowledgements}

We thank the EIC Silicon Consortium for cost estimate methodologies concerning silicon tracking systems, technical discussions, and comments.  We acknowledge the important prior work of projects eRD16, eRD18, and eRD25 concerning research and development of MAPS silicon tracking technologies.

We thank the EIC LGAD Consortium for technical discussions and acknowledge the prior work of project eRD112.

We thank (list of individuals who are not coauthors) for their useful discussions, advice, and comments.

We acknowledge support from the Office of Nuclear Physics in the Office of Science in the Department of Energy, the National Science Foundation, and the Los Alamos National Laboratory Laboratory Directed Research and Development (LDRD) 20200022DR.
%



==> Submit_ArXiv/sections/backup.tex <==
\begin{comment}
\begin{figure}[!]
    \centering
    \includegraphics[width=0.45\textwidth]{figs/dRICH_BO_scheme.png}
    \caption{
    Bayesian optimization framework for the optimization of the dual-RICH. N detector design points are created in parallel and passed to the BO which uses Gaussian processes, which collects the points, updates the surrogate model (a 2D visualization is shown in the bottom right corner considering all pairs of design parameters). A cheap acquisition function suggests a new set of design points to query at the next iteration. Convergence criteria are implemented on both the design space and on the objective (in this case, the $\pi$/K separation power of the dual-RICH) and early stopping is activated when convergence is observed in both spaces. Figure taken from \cite{fanelli_jluo2021}. More details can be found in \cite{cisbani2020ai}.   
    }
    \label{fig:dRICH_BO_scheme}
\end{figure}
\end{comment}

%identify the solutions that can approximate the sought performance in the functional space (see, \textit{e.g.}, \cite{sanchez2018inverse}). 




%Leveraging on the expertise internal to the ECCE proto-collaboration --- see, \textit{e.g.}, the optimization of imaging Cherenkov detectors with AI-based techniques \cite{cisbani2020ai} with a workflow described in Fig. \ref{fig:dRICH_BO_scheme} --- 



%The first parallelized, automated and self-consistent AI-supported strategy for detector optimization has been demonstrated for the dual-RICH in a work led by  \cite{cisbani2020ai}.

%leveraging Bayesian optimization (BO) \cite{snoek2012practical}. 
%A workflow of this framework is shown in Fig.~\ref{fig:dRICH_BO_scheme}, where more details can be found. 

 % see Fig. \ref{fig:pipeline_workflow} (bottom).

\begin{comment}
 \begin{figure}[!]
    \centering
    \includegraphics[width=0.45\textwidth]{figs/interplay_groups.png}
    \caption{
    A workflow describing the iterative process of detector design. AI assisted this process, provided insights and helped capturing hidden correlations among the design parameters. 
    This has been used during the detector technology choice to steer the design. At a given instant in time, N alternative candidate configurations are studied. For each we create an optimization pipeline, which results in a Pareto front of solutions. This new information helps the proto-collaboration steering the design: some configurations are rejected, while alternative ones (also dubbed `new references') are identified to potentially improve the design. New optimization pipelines (we typically handled a maximum of 4-5 pipelines each time) are defined based on these alternatives and the process is iterated. 
    The fundamental interplay between the ECCE Teams working on Physics(PWG), Detector(DWG) and Computing(CWG) is clearly propelled by AI during the design process. 
}
    \label{fig:pipeline_workflow}
\end{figure}
\end{comment}



%----------------------- slanted figures ----------------------%


\begin{comment}
\begin{figure}[!]
    \centering
    \includegraphics[width=0.45\textwidth]{figs/NonProjectiveGeom_Detailed_Slanted.pdf}
    \caption{\textbf{The ECCE tracking and PID system during Phase-I optimisation:} This is one of the studied configurations. Multiple pipelines corresponding to different combinations of technology for the barrels and the disks have been studied. Since the arrangement is symmetric, optimisations are done in $\eta$ corresponding only to the barrel region and the forward-region. The labels given in red are considered for optimisation, and the labels in blue are fixed in their locations. The geometry displays a non-projective design of the support structure.}
    \label{fig:Phase-I_ECCEDetector}
\end{figure}
\end{comment}


\begin{comment}
\begin{figure}[!]
    \centering
    \includegraphics[width=0.45\textwidth]{figs/ProjectiveGeom_Detailed_Slanted.pdf}
    \caption{\textbf{Tracking and PID systems in the ongoing R\&D projective design:} Starting from the IP, angle of the conical support structure ($\theta$) which defines the angle of the projective geometry. Followed by 3 vertex barrel layers (ITS3 technology), followed by 2 sagitta layers (ITS3 techonology), 2 $\mu$Rwell layers, ACLGAD based CTTL Time Of Flight (TOF) detector, DIRC (for PID) detector and finally another layer of $\mu$Rwell. In the electron-going direction there are 4 EST disks (silicon disks) followed by MPGD, mRICH (PID) detector and ACLGAD based ETTL TOF disk. In the hadron-going direction there are 5 FST disks (silicon disks) followed by a layer of ACLGAD based FTTL TOF disk, the dRICH (PID) detector and finally a layer of MPGD disk. The labels in red are the detector systems that are considered for optimisation. The labels in blue are the detector systems that are not free parameters and are not optimised during the optimisation. Some of the detectors parameters given in blue are parameterised such that they change as the design varies The Tracking support cone comprises copper and plastic insulation along with carbon fiber and the cooling system (water). The support cone is relatively thick up to 1cm for over the optimisation.  %\cris{sentence not clear} The labels in blue are the detector systems that either have their dimensions fixed or is parameterised during the optimisation as they are not free parameter
    }
    \label{fig:ECCE_TrackingPID_Detailed}
\end{figure}
\end{comment}




\begin{table}[bh!]
   
    \centering
    \begin{tabular}{|M{3.cm} | M{1.5cm}| M{2.0cm}|}
        \hline
        \textbf{description} & \textbf{symbol} & \textbf{value} \\ 
        \hline
        \hline
        \small{population size} & N & 100 \\
        \small{\# objectives}   & M & 3(4)\\ 
        \small{offspring} & O & 30(50)\\
        \small{design size} & D & 4(11) \\
        \small{\# calls (tot. budget)} & $-$ & 50(200)\\
        \small{\# cores} & $-$ & \small{same as offspring} \\
        \small{\# charged $\pi$ tracks} & N$_{\textup{trk}}$ & 80k\\
        \small{\# bins in $\eta$} & N$_{\eta}$ & 3 (5)\\
        \small{\# bins in P} & N$_{\textup{P}}$ & 10 (15) \\
        \hline
    \end{tabular}
    \caption{ Summary of the hyperparameters used for the non-projective tracker design. Symbols used throughout the document to describe these quantities are also reported to facilitate the reader. %For each parameter, in parentheses one can find the maximum value that has been explored. 
     Values in parentheses are the largest ones utilized in the optimization pipelines. The total number of design vary between Phase-I and Phase-II. Phase-II optimization involved accommodating realistic support structure and therefore constraining the overall design space. Checkpoints are created allowing to take a snapshot of the optimization while ongoing. A survey of the detector performance is created after each call. At each call an offspring of 30 or 50 new design points has been created through a genetic algorithm. A two-level parallelization is implemented as explained in Sec.~\ref{subsec:computing}. %The framework ran on the JLab computing farm which currently host nodes with a maximum number of 128 cores.
     \cris{merge with Table~\ref{tab:Complexity_Proj}.}
     \label{tab:Complexity_NonProj}
    }
    
\end{table}



\begin{table}[h!]
    \centering
    \begin{tabular}{|M{3.cm} | M{1.5cm}| M{2.0cm}|}
        \hline
        \textbf{description} & \textbf{symbol} & \textbf{value} \\ 
        \hline
        \hline
        \small{population size} & N & 100 \\
        \small{\# objectives}   & M & 3(4)\\ 
        \small{offspring} & O & 30(50)\\
        \small{design size} & D & 11(16) \\
        \small{\# calls (tot. budget)} & $-$ & 200\\
        \small{\# cores} & $-$ & \small{same as offspring} \\
        \small{\# charged $\pi$ tracks} & N$_{\textup{trk}}$ & 120k\\
        \small{\# bins in $\eta$} & N$_{\eta}$ & 5 \\
        \small{\# bins in P} & N$_{\textup{P}}$ & 10 \\
        \hline
    \end{tabular}
    \caption{Summary of the hyperparameters utilized for the projective design. Values in parentheses are the largest ones utilized in other optimization pipelines. Checkpoints are created allowing to take a snapshot of the optimization while ongoing. A survey of the detector performance is created after each call. At each call an offspring of new design points is created through a genetic algorithm. %A two-level parallelization is implemented as explained in the text. The framework ran on the JLab computing farm which currently host nodes with a maximum number of 128 cores.
    }
    \label{tab:Complexity_Proj}
\end{table}
%



\begin{table}[!]
    \centering
    \resizebox{\columnwidth}{!}{%
    \begin{tabular}{M{2.5cm}|M{3.cm}|M{3.cm}|M{3.5cm}}
        \hline
        & \textbf{design pars} &  \textbf{objectives} &  \textbf{constraints} \\
        \hline
        \hline
           \textbf{\#} &  4(11) &  3 (4) &  4(5) \\
        \hline
           \textbf{description} & \small{(Phase-I symmetric design) 5 disks $z$-location (hadron beam) and 6 barrel layers radii; (Phase-II asymmertic design) 3 disks $z$ location (endcap region) 1 barrel layer} & \small{momentum resolution; angular resolution; Kalman filter efficiency; (pointing resolution)}
           & \small{(i) inner 2$^{nd}$ vtx barrel radius $\leq$ 15 cm; (ii) outermost barrel radius $<$ 51 cm; (iii) outermost $z$ disk $<$ 125 cm; (iv) 4$^{th}$ barrel radius $\leq$ 45 cm; (v) Minimum distance between any 2 layers $>=$ 1 cms (Additional constraints for Phase-II)} \\
        \hline
        \hline
    \end{tabular}
    }
    \caption{Dimensionality of the non-projective design and objective space. Following Eq.~\eqref{eq:moo}, constraints are also included. For each category, a description has been added.  Values in parentheses are the largest ones utilized in the optimization pipelines.
    The Phase-II optimization had less number of parameters to optimize due to the fixed support cone structure.  Notice that two additional constraints are implicitly taken into account, that is: (i) the inner radii of the disks in the endcap and the inner vertex layer in the barrel have to be compatible with the beam envelope dimensions; (ii) the barrel layers lengths and the outer radii of the disks have to be compatible with an Al-shell support structure provided by the LBNL design \cite{arrington2021eic}. Conditions (i) and (ii) are provided by internal parametrization and reflected in the Geant4 design. Potential overlaps among modules are checked before and during the optimization.}
    \label{tab:Problem_NonProj}
\end{table}


\begin{comment}
\begin{table}[!]
    \centering
    \resizebox{\columnwidth}{!}{%
    \begin{tabular}{M{2.5cm}|M{3.cm}|M{3.cm}|M{3.5cm}}
    %\begin{tabular}{c|c|c|c}
        \hline
        & \textbf{design pars} &  \textbf{objectives} &  \textbf{constraints} \\
        \hline
        \hline
           \textbf{\#} &  11 (16) &  4 &  3 (5)\\
        \hline
           \textbf{description} & \small{(symmetric design) Angle Tracking Support ($\theta$), 2 TTL $z$-location, 2 MPGD $z$-location, 1 uRwell-1 Radius, 5 EST/FST disks; (asymmetric design) total of 16 params} & \small{momentum resolution; angular resolution; Kalman filter efficiency; angular resolution at dRICH; (pointing resolution)}
           & \small{(i) FST/EST Disks $(R_{Max}-R_{Min})\%(30.0 \ mm)=0$; (ii) FST/EST Disks $(R_{Max}-R_{Min})\%(17.8 \ mm)=0$; (iii) FST/EST $z_{n+1} - z_{n} \geq 10$; (iv) Length of vertex support structure $\leq$ 30 cms; (v) distance between any 2 $\mu$Rwell barrel layers have to be atleast 5 cms; } 
           %\cris{larger! It was smaller...} 
           \\
        \hline
        \hline
    \end{tabular}
    }
    \caption{Dimensionality of the problem in the projective design and objective space. Following Eq.~\eqref{eq:moo}, constraints are also included. For each category, a description has been added. Number in parentheses are for optimizations pipelines utilizing an asymmetric design with both the cone angle in e-going and h-going side to vary. However, the set up with different angles in e-going and h-going directions was not preferred as it would be difficult to realise such a design.
    }
    \label{tab:Problem_Proj}
\end{table}
\end{comment}


\begin{comment}
\begin{table}[!]
    \centering
    \begin{tabular}{|M{1.5cm}|M{4.5cm}|M{4.5cm}|}
        \hline
        $\#$ & Objectives & Ratio \\
        \hline
        \hline
        1 & Momentum Resolution Eq.~\eqref{eq:obj_definition} & Eq.~\eqref{eq:objectives_reso}\\
        \hline
        2 & Angular Resolution ($d\theta$) Eq.~\eqref{eq:obj_definition} & Eq.~\eqref{eq:objectives_reso}\\
        \hline
        3 & Kalman Filter InEfficiency & Ratio: Eq.~\eqref{eq:objective_KF} \\
        \hline
        4 & Angular Resolution $@$ dRICH (PID) Eq.~\eqref{eq:obj_definition_PID} & Ratio Equation: Eq.~\eqref{eq:Objectives_Reso} \\
        \hline
    \end{tabular}
    \caption{
    \cris{add caption; this table is for the projective case.};
    %The table summarises constraints on the design problem. Mainly the constraints are on the FST/EST disks are made by tiling up the MAPS pixels. The pixels will be made are of fixed dimensions. Soft constraints are constraints that can be violated but the MOO will evolve to minimally violate the constraints. Also, minor adjustments on tiling up the pixels can be done post hoc optimization such that the Detector geometry is realisable. Strong constraints penalises the MOO with high penalities since these constraints cannot be violated.
    }
    \label{tab:Objectives_proj}
\end{table}
\end{comment}



\begin{comment}
\begin{figure*}[!]
\centering
\begin{tabular}{|c|c|c|c|c|}
\hline
\subf{\includegraphics[width=22mm]{figs/analysis/dpp_1.pdf}}
    {}
    %{text}
&
\subf{\includegraphics[width=22mm]{figs/analysis/dpp_2.pdf}}
    {}
&
\subf{\includegraphics[width=22mm]{figs/analysis/dpp_3.pdf}}
    {}
&
\subf{\includegraphics[width=22mm]{figs/analysis/dpp_4.pdf}}
    {}
&
\subf{\includegraphics[width=22mm]{figs/analysis/dpp_5.pdf}}
    {}
\\
\hline
\subf{\includegraphics[width=22mm]{figs/analysis/dpp_6.pdf}}
    {}
    %{text}
&
\subf{\includegraphics[width=22mm]{figs/analysis/dpp_7.pdf}}
    {}
&
\subf{\includegraphics[width=22mm]{figs/analysis/dpp_8.pdf}}
    {}
&
\subf{\includegraphics[width=22mm]{figs/analysis/dpp_9.pdf}}
    {}
&
\subf{\includegraphics[width=22mm]{figs/analysis/dpp_10.pdf}}
    {}
\\
\hline
\subf{\includegraphics[width=22mm]{figs/analysis/dpp_11.pdf}}
    {}
&
\subf{\includegraphics[width=22mm]{figs/analysis/dpp_12.pdf}}
    {}
&
\subf{\includegraphics[width=22mm]{figs/analysis/dpp_13.pdf}}
    {}
&
\subf{\includegraphics[width=22mm]{figs/analysis/dpp_14.pdf}}
    {}
&
\subf{\includegraphics[width=22mm]{figs/analysis/dpp_15.pdf}}
    {}
\\
\hline
\subf{\includegraphics[width=22mm]{figs/analysis/dpp_16.pdf}}
    {}
&
\subf{\includegraphics[width=22mm]{figs/analysis/dpp_17.pdf}}
    {}
&
\subf{\includegraphics[width=22mm]{figs/analysis/dpp_18.pdf}}
    {}
&
\subf{\includegraphics[width=22mm]{figs/analysis/dpp_19.pdf}}
    {}
&
\subf{\includegraphics[width=22mm]{figs/analysis/dpp_20.pdf}}
    {}
\\
\hline
\subf{\includegraphics[width=22mm]{figs/analysis/dpp_21.pdf}}
    {}
&
\subf{\includegraphics[width=22mm]{figs/analysis/dpp_22.pdf}}
    {}
&
\subf{\includegraphics[width=22mm]{figs/analysis/dpp_23.pdf}}
    {}
&
\subf{\includegraphics[width=22mm]{figs/analysis/dpp_24.pdf}}
    {}
&
\subf{\includegraphics[width=22mm]{figs/analysis/dpp_25.pdf}}
    {}
\\
\hline
\subf{\includegraphics[width=22mm]{figs/analysis/dpp_26.pdf}}
    {}
&
\subf{\includegraphics[width=22mm]{figs/analysis/dpp_27.pdf}}
    {}
&
\subf{\includegraphics[width=22mm]{figs/analysis/dpp_28.pdf}}
    {}
&
\subf{\includegraphics[width=22mm]{figs/analysis/dpp_29.pdf}}
    {}
&
\subf{\includegraphics[width=22mm]{figs/analysis/dpp_30.pdf}}
    {}
\\
\hline
\subf{\includegraphics[width=22mm]{figs/analysis/dpp_31.pdf}}
    {}
&
\subf{\includegraphics[width=22mm]{figs/analysis/dpp_32.pdf}}
    {}
&
\subf{\includegraphics[width=22mm]{figs/analysis/dpp_33.pdf}}
    {}
&
\subf{\includegraphics[width=22mm]{figs/analysis/dpp_34.pdf}}
    {}
&
\subf{\includegraphics[width=22mm]{figs/analysis/dpp_35.pdf}}
    {}
\\
\hline
\subf{\includegraphics[width=22mm]{figs/analysis/dpp_36.pdf}}
    {}
&
\subf{\includegraphics[width=22mm]{figs/analysis/dpp_37.pdf}}
    {}
&
\subf{\includegraphics[width=22mm]{figs/analysis/dpp_38.pdf}}
    {}
&
\subf{\includegraphics[width=22mm]{figs/analysis/dpp_39.pdf}}
    {}
&
\subf{\includegraphics[width=22mm]{figs/analysis/dpp_40.pdf}}
    {}
\\
\hline
\subf{\includegraphics[width=22mm]{figs/analysis/dpp_41.pdf}}
    {}
&
\subf{\includegraphics[width=22mm]{figs/analysis/dpp_42.pdf}}
    {}
&
\subf{\includegraphics[width=22mm]{figs/analysis/dpp_43.pdf}}
    {}
&
\subf{\includegraphics[width=22mm]{figs/analysis/dpp_44.pdf}}
    {}
&
\subf{\includegraphics[width=22mm]{figs/analysis/dpp_45.pdf}}
    {}
\\
\hline
\end{tabular}
\caption{The resolutions are fitted in bins of momentum and pseudo-rapidity. The figures displays the example of the momentum resolution, which is calculated in multiple bins in the region 0~$\leq$P$\leq$~30~GeV/c and 0~$\leq \eta \leq$~3.5. These studies are extended to the e-going direction with negative values of $\eta$.
\label{fig:fit_results}
}
\end{figure*}
\end{comment}



%----------------------- all tables go here -------------------%
% non-projective 
% projective 

Tables \ref{tab:Complexity_NonProj} and \ref{tab:Problem_NonProj} summarize the overall implementation of different pipelines for the non-projective design corresponding to both Phase-I and Phase-II optimizations. 

Tables \ref{tab:Complexity_Proj} and \ref{tab:Problem_Proj} summarize the overall implementation of different pipelines during Phase II for the projective design. 

Table \ref{tab:Parameter_Range_Proj} reports in particular the range of parameters utilized in the projective design.  

%Table \ref{tab:constraints} is a table summarizing the constraints utilized in the MOO problem. 



\cris{Merging of tables here.}

%Additionally \ref{tab:constraints} provide constraints for the optimization of Phase-II non Projective optimizations. Therefore, Phase-II non Projective Optmisation was highly constrained.


\cris{Checkpoints are created allowing to take a snapshot of the optimization while ongoing. 
%
A survey of the detector performance is created after each call. 
%
At each call an offspring of 30  new design points has been created through a genetic algorithm. A two-level parallelization is implemented as explained in Sec.~\ref{subsec:computing}.
}


\begin{comment}
%-------------------------------------------
\paragraph{Design Performance (Phase I):} 
%
Performance is shown in terms of the objective functions utilized during the optimization process. 
After the optimization, these functions are shown as a function of the phase-space (P,$\eta$). \cris{utilize P uniformly in the text}.

One particular solution from the Pareto front is taken here as an example. Fig.~\ref{fig:FrozenAnalysis_dpp} shows the momentum resolution corresponding to the baseline design of one of the pipelines from Phase-I optimization. This solution in the Pareto front shows about 20 $\%$ improvement in central and extreme forward regions. 
A similar plot in Fig.~\ref{fig:FrozenAnalysis_dth} shows the angular resolution ($d\theta$) corresponding to the baseline design, where an improvement is seen at large values of $\eta$.
The other objective is the Kalman filter inefficiency which has been minimized together with the other two objectives. 
Fig.~\ref{fig:FrozenAnalysis_KFInEff} shows the resulting KF efficiency, where it can be seen a substantial improvement with AI in the overall region $\eta$ $>$ 1.

\begin{figure}[!]
\centering
\begin{tabular}{|c|c|c|}
\hline
\subf{\includegraphics[width=44mm]{figs/FrozenConceptAnalysis/FrozenConceptAllCompare_dp_p_p_eta_0 - 1.pdf}}
    {}
    %{text}
&
\subf{\includegraphics[width=44mm]{figs/FrozenConceptAnalysis/FrozenConceptAllCompare_dp_p_p_eta_1 - 2.5.pdf}}
    {}
&
\subf{\includegraphics[width=44mm]{figs/FrozenConceptAnalysis/FrozenConceptAllCompare_dp_p_p_eta_2.5 - 3.5.pdf}}
    {}

\\
\hline
\subf{\includegraphics[width=44mm]{figs/FrozenConceptAnalysis/FrozenConceptRatio_Compare_dp_p_p_eta_0 - 1.pdf}}
    {}
&
\subf{\includegraphics[width=44mm]{figs/FrozenConceptAnalysis/FrozenConceptRatio_Compare_dp_p_p_eta_1 - 2.5.pdf}}
    {}
&
\subf{\includegraphics[width=44mm]{figs/FrozenConceptAnalysis/FrozenConceptRatio_Compare_dp_p_p_eta_2.5 - 3.5.pdf}}
    {}
\\
\hline
\end{tabular}
\caption{Momentum resolution corresponding to the Baseline design of one of the pipelines from Phase-I optimization. From Left to right in top row corresponds to momentum resolutions in various bins in eta. The objective calculated during optimization is based on 3 bins in $\eta$ and the optimization assumes a symmetric arrangement of detectors in the endcap region. Therefore, optimization was carried out only in the forward region ($\eta > 0$). The bottom row shows the ratio of the optimal solution to that of the baseline (reference) design performance. We see about 20 $\%$ improvement in central and extreme forward regions. Therefore, the optimal solution outperforms in all the bins in $\eta$.}
\label{fig:FrozenAnalysis_dpp}
\end{figure}


\begin{figure}[!]
\centering
\begin{tabular}{|c|c|c|}
\hline
\subf{\includegraphics[width=44mm]{figs/FrozenConceptAnalysis/FrozenConceptAllCompare_dth_th_p_eta_0 - 1.pdf}}
    {}
    %{text}
&
\subf{\includegraphics[width=44mm]{figs/FrozenConceptAnalysis/FrozenConceptAllCompare_dth_th_p_eta_1 - 2.5.pdf}}
    {}
&
\subf{\includegraphics[width=44mm]{figs/FrozenConceptAnalysis/FrozenConceptAllCompare_dth_th_p_eta_2.5 - 3.5.pdf}}
    {}

\\
\hline
\subf{\includegraphics[width=44mm]{figs/FrozenConceptAnalysis/FrozenConceptRatio_Compare_dth_th_p_eta_0 - 1.pdf}}
    {}
&
\subf{\includegraphics[width=44mm]{figs/FrozenConceptAnalysis/FrozenConceptRatio_Compare_dth_th_p_eta_1 - 2.5.pdf}}
    {}
&
\subf{\includegraphics[width=44mm]{figs/FrozenConceptAnalysis/FrozenConceptRatio_Compare_dth_th_p_eta_2.5 - 3.5.pdf}}
    {}
\\
\hline
\end{tabular}
\caption{Angular resolution ($d\theta$) corresponding to the Baseline design of one of the pipelines from Phase-I optimization. From Left to right in top row corresponds to momentum resolutions in various bins in eta. The objective calculated during optimization is based on 3 bins in $\eta$ and the optimization assumes a symmetric arrangement of detectors in the endcap region. Therefore, optimization was carried out only in the forward region ($\eta > 0$). The bottom row shows the ratio of the optimal solution to that of the baseline (reference) design performance. We see an improvement in $2.5 < |\eta| < 3.5$ and performs similar in other bins.}
\label{fig:FrozenAnalysis_dth}
\end{figure}


\begin{figure}[!]
\centering
\begin{tabular}{|c|c|c|}
\hline
\subf{\includegraphics[width=44mm]{figs/FrozenConceptAnalysis/FrozenConceptAllCompare_KF_InEfficiency_eta_0 - 1.pdf}}
    {}
    %{text}
&
\subf{\includegraphics[width=44mm]{figs/FrozenConceptAnalysis/FrozenConceptAllCompare_KF_InEfficiency_eta_1 - 2.5.pdf}}
    {}
&
\subf{\includegraphics[width=44mm]{figs/FrozenConceptAnalysis/FrozenConceptAllCompare_KF_InEfficiency_eta_2.5 - 3.5.pdf}}
    {}

\\
\hline
\subf{\includegraphics[width=44mm]{figs/FrozenConceptAnalysis/FrozenConceptRatio_Compare_KF_InEfficiency_eta_0 - 1.pdf}}
    {}
&
\subf{\includegraphics[width=44mm]{figs/FrozenConceptAnalysis/FrozenConceptRatio_Compare_KF_InEfficiency_eta_1 - 2.5.pdf}}
    {}
&
\subf{\includegraphics[width=44mm]{figs/FrozenConceptAnalysis/FrozenConceptRatio_Compare_KF_InEfficiency_eta_2.5 - 3.5.pdf}}
    {}
\\
\hline
\end{tabular}
\caption{Kalman Filter efficiency corresponding to the Baseline design of one of the pipelines from Phase-I optimization. From Left to right in top row corresponds to momentum resolutions in various bins in eta. The objective calculated during optimization is based on 3 bins in $\eta$ and the optimization assumes a symmetric arrangement of detectors in the endcap region. Therefore, optimization was carried out only in the forward region ($\eta > 0$). The bottom row shows the ratio of the optimal solution to that of the baseline (reference) design performance. We see an improvement in mid region $ 1.0 < \eta < 2.5 $ and $2.5 < |\eta| < 3.5$ and performs similar in other bins.
\cris{Ratios are for the inefficiency. THIS IS A PLACEHOLDER}.
}
\label{fig:FrozenAnalysis_KFInEff}
\end{figure}
\end{comment}




%%%% Start of Phase -I results %%%%%%
\begin{comment}
\paragraph{Design Performance in Phase I}

Phase-I optimization as mentioned earlier, corresponds to a set of optimizations that were done on a symmetric arrange of disks in both electron-going and hadron-going directions. 
Some of the detectors like the PID and TOF detectors were modelled using fast simulation. The optimization did not include the  cone structure and hence the active dead material interaction was not minimized in the optimization process. There were 4 combinations of technologies (pipelines) that were proposed for the inner barrel tracking system. Each combination was explored and optimized using the developed framework. Fig.~\ref{fig:Phase-I_Pipelines} shows the momentum resolution of the explored pipelines and the corresponding optimized performance. 

\begin{figure*}[!]
\centering
\begin{tabular}{c c c}
%\hline
\subf{\includegraphics[width=51mm]{figs/FrozenConceptAnalysis/AllPipelines/FrozenConceptAllComparePipeline_dp_p_p_eta_0 - 1.pdf}}
    {}
    %{text}
&
\subf{\includegraphics[width=51mm]{figs/FrozenConceptAnalysis/AllPipelines/FrozenConceptAllComparePipeline_dp_p_p_eta_1 - 2.5.pdf}}
    {}
&
\subf{\includegraphics[width=51mm]{figs/FrozenConceptAnalysis/AllPipelines/FrozenConceptAllComparePipeline_dp_p_p_eta_2.5 - 3.5.pdf}}
    {}

\\
%\hline

\end{tabular}
\caption{\cris{This is a place-holder; will be updated} Momentum resolution of different pipelines corresponding to different possible combinations of technology optimized with AI. %It is shown that any given combination of technology (pipeline) can optimized using the developed framework. 
Pipeline-IV was eventually chosen as the new reference design for the inner barrels. It should be noted that the AI-optimized configurations outperformed the original designs in all $\eta$ bins. Specifically, the optimized pipelines meet the YR PWG requirement in the region $1.0 \leq \eta < 2.5$. }\label{fig:Phase-I_Pipelines}
\end{figure*}

As a result of the Phase-I AI-assisted optimization, pipeline-IV (made by 2 vtx (ITS3-MAPS), 2 sagitta (ITS3-MAPS), 2 outer ($\mu$Rwell)) was chosen by ECCE (after discussing the results with the DWG and the PWG, see Fig.~\ref{fig:pipeline_workflow}) as the new inner tracker barrel design.
Detailed simulation of the PID and TOF detectors were made after Phase-I optimization.
At this point, the arrangement of disks in the electron-going and hadron-going directions was no more symmetric. A realistic support structure has been also implemented, along with new constraints, updated simulations of the detector system and more realistic support structures. The pipeline-IV has been selected as the new reference for the next phase (Phase-I I) in this continued optimization process.

\end{comment}



%\begin{itemize}
    %\item Out of the pipelines that were optimized, 2 pipelines were potentially chosen as they readily satisfy the PWG requirement in the central region. Also, All the pipelines improve the momentum resolution in the transition region. 
    %\item Pipeline-4 \Big [ 2 vtx (ITS3-MAPS) + 2 sagitta (ITS3-MAPS) + 2 outer ($\mu$Rwell) \Big ] was chosen by the proto-collaboration since it was chosen as the new inner tracker barrel design for ECCE.  
    
    %\item The important role of AI is to steer the decision towards choosing a pipeline. AI had assisted in choosing the appropriate technology for the inner tracking barrels (Pipeline-4). This choice of technology was not only made by simply swapping the barrel layers with different combinations but an extensive optimization was done to show that chosen pipeline can be optimized the most and also at the same time realisable by the DWG. 
    %\item Pipeline-4 is now the new reference design for the inner barrels. Detailed simulation of the PID and TOF detectors were made by end of Phase-I optimization. The arrangement of disks in the electron-going and hadron-going directions were no more symmetric. There were implementation of realistic support structure. Therefore with new constraints and updated simulations of detector system and more realistic support structures and pipeline-4 as the new updated reference design next phase (Phase-II) of optimizations continued.
   
%\end{itemize}


%--- end Karthik comment 
%%%%% End of Phase-I results %%%%%%%


%\clearpage
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
\paragraph{Design Performance --- Non-projective vs Projective:} 
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%
Results shown in this paragraph have been obtained during the optimization Phase II. 


\begin{comment}

Fig.~\ref{fig:Phase-II_Momentum_res} shows the momentum resolution for the non-projective ECCE tracker reference design and the ongoing project R\&D on the projective mechanical structure for the ECCE tracker design in bins of pseudo-rapidity.
Similarly Fig.~\ref{fig:Phase-II_dth_res} shows the angular resolution while Fig.~\ref{fig:Phase-II_KF_eff} shows the Kalman filter efficiency as defined in Eq.~\eqref{eq:objective_KF}.
\end{comment}

%\cris{Move Figures \ref{fig:Phase-II_Momentum_res}, \ref{fig:Phase-II_dth_res}, \ref{fig:Phase-II_KF_eff}, \ref{fig:Phase-II_dph_res}, \ref{fig:Phase-II_recon_eff} in Appendix.}





\begin{comment}
%\clearpage
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
\subsection{Validation}\label{subsec:validation}
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%

Validation is performed by looking at figures of merit that are not used in the optimization process. Also in Sec.~\ref{subsec:physics_analysis} we perform a physics analysis with SIDIS events to further consolidate our conclusions.
We show here as an example in Fig.~\ref{fig:Phase-II_dph_res} and Fig.~\ref{fig:Phase-II_recon_eff} the azimuthal angular resolution and the reconstruction efficiency obtained for both the non-projective and the projective ECCE tracker.
The azimuthal resolution looks consistent within the uncertainty for the two designs, while the reconstruction efficiency looks in general better for the projective design, particularly in the 1 $<$ $|\eta|$ $<$ 1.5 region where the non-projective has a larger dead area that affect the reconstruction of tracks.
\end{comment}





%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%\paragraph{validation of Phase-II projective}






%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
% Sec. 3 on Simulations 


%The ECCE tracking system strategically deploys two novel technologies: 
%
%Furthermore, as shown in Figure~\ref{fig:tracking}, the tracking system is tightly integrated with the PID detectors. 
%In particular, the AC-LGAD based Time of Flight (ToF) detectors will also provide precision space-time measurements on the track. 


%%All repositories are documented here \cite{ecce_eic_repo}.

%%The concept of Node Tree is at the center of the Fun4All software framework \cite{fun4all_doc}, in that this is how data are organized. Data object are stored in DST Tree. The user can utilize C++ based analysis modules to access them, perform analysis and save result in analysis NTuple and/or histograms for final plotting. User usually need to compile the analysis module, run it as part of fun4all reconstruction macro, and plot based on the output ROOT file. The structure of the Fun4All framework is represented in Fig.~\ref{fig:Fun4All_Workflow}.
%A more detailed description of the ECCE Software documentation can be found in the following documentation \cite{ecce_sw_doc}.



\begin{comment}
\begin{figure*}[!ht]
\centering
    \includegraphics[width=0.49\textwidth]{figs/IP6-1.5T-Starting-Setup-11142021-EEMCAL-eta3-tracking2.jpg}
    \includegraphics[width=0.49\textwidth]{figs/Oct-Concept39.png}
    \caption{tracking system of ECCE in mechanical model (left) and Geant4 simulation (right). The tracking system is tightly integrated with the PID detectors which is also shown on the right. Support and cabling for the these detectors was implemented (copper-colored cylinder-cone) to count for its material and acceptance effects.}
    \label{fig:tracking}
\end{figure*}
\end{comment}


%
%For each of the sub-detector described in this document, the dimensions of the detectors can be parametrized based on constraints. 



\begin{comment}
\begin{figure}[!]
    \centering
    %\includegraphics[scale = 0.8]{figs/ProjectionConceptAnalysis/AllinOne.pdf}
    \includegraphics[width=0.45\textwidth]{figs/TechNote_Tracking_GAUSS.pdf}
    \caption{
    \textbf{Momentum resolution for the ECCE tracker reference design and the projective design (ongoing R\&D):} The $\Delta p /p$ are extracted with single-gaussian (SG) fits (circles) to be consistent with the YR PWG and compared to double-gaussian (DG) fits (triangles). DG (see Eq.~\eqref{eq:DG}) is used in the AI-assisted pipelines as it provides more stable fits. DG results are systematically larger than the SG ones as they capture more realistic distributions (see Fig.~\ref{fig:fit_results}). 
    This effect is larger in $1<|\eta|<1.5$ for the non-projective design (blue points) since more material is traversed by the tracks; the same effect is moderately present also in $0.5<|\eta|<1$ for the same reason. 
    In the same bins, the ongoing R\&D design shows a significant reduction of the impact of the readout and services and SG (red circle) and DG (red triangles) are close to each other.  
    DG points are systematically large in $3<\eta<3.5$ and in $-3.5<\eta<3.0$, and this corresponds to edge effects at large $|\eta|$ values close to the inner radii of the disks in the endcaps.  
    In the region $-1<\eta<3.0$ $\Delta p/p$ is consistent with the YR physics requirements with SG. Note that physics in the backward region relies on the EM calorimeter also, and in the proposal it has been demonstrated that larger resolutions are acceptable.  
    \label{fig:Phase-II_Momentum_res}
    }
\end{figure}


\begin{figure}[!]
    \centering
    \includegraphics[width=0.45\textwidth]{figs/ProjectionConceptAnalysis/CompareAll_dth.pdf}
    \caption{\tetxbf{Angular resolution ($d\theta$) for ECCE projective geometry and ECCE simulation:} The resolution shows an improvement in the transition region between $1.0 < |\eta| < 1.5$. These plots have been produced using double-gaussian fits.
    \label{fig:Phase-II_dth_res}
    }
\end{figure}

\begin{figure}[!]
    \centering
    \includegraphics[width=0.45\textwidth]{figs/ProjectionConceptAnalysis/TechNote_KF_Efficiency.pdf}
    \caption{\tetxbf{KF Efficiency for ECCE projective geometry and ECCE simulation:} Reconstruction efficiency shows an improvement in the transition region between $1.0 < |\eta| < 1.5$. There is a significant drop in the transition region caused due to multiple scattering of the support structure. }
    \label{fig:Phase-II_KF_eff}
\end{figure}
\end{comment}




\begin{comment}
\begin{table}[!]
    \centering
    \resizebox{\columnwidth}{!}{%
    \begin{tabular}{M{2.5cm}|M{3.cm}|M{3.cm}|M{3.5cm}}
        \hline
        & \textbf{design pars} &  \textbf{objectives}\\
        \hline
        \hline
           %\textbf{\#} &  4(11) &  3 (4) &  4(5) %\\
        %\hline
           \textbf{ECCE tracker design (non-projective)} & \small{
           %(Phase-I symmetric design) 5 disks $z$-location (hadron endcap) and 6 barrel layers radii;
           5 disks $z$ (hadron endcap) and 4 disks $z$ (electron end cap) location,  2 $\mu$Rwell layers Radius} & \small{momentum resolution; angular resolution; Kalman filter efficiency; (pointing resolution)}
            \\
        \hline
        \hline
           \textbf{ECCE ongoing R\&D design (projective)} & \small{Angle Tracking Support ($\theta$), 2 TTL $z$-location, 1 uRwell-1 Radius, 3 FST disks, 2 EST disks (9 parameters);} & \small{momentum resolution; angular resolution; Kalman filter efficiency; angular resolution at dRICH; (pointing resolution)}
           & \small{(i) FST/EST Disks $(R_{Max}-R_{Min})\%(30.0 \ mm)=0$; (ii) FST/EST Disks $(R_{Max}-R_{Min})\%(17.8 \ mm)=0$; (iii) FST/EST $z_{n+1} - z_{n} \geq 10$; (iv) Length of vertex support structure $\leq$ 30 cm; (v) distance between any 2 $\mu$Rwell barrel layers have to be $\geq$ 5 cm } 
           %\cris{larger! It was smaller...} 
           \\
        \hline
        \hline
        
    \end{tabular}
    } 
    \caption{ \textbf{Dimensionality of the optimization pipelines:} 
    non-projective design and objective space. Following Eq.~\eqref{eq:moo}, constraints are also included. For each category, a description has been added.  Values in parentheses are the largest ones utilized in the optimization pipelines.
    The Phase-II optimization for non-projective design had less number of parameters to optimize due to the fixed support cone structure.  Notice that two additional constraints are implicitly taken into account, that is: (i) the inner radii of the disks in the endcap and the inner vertex layer in the barrel have to be compatible with the beam envelope dimensions; (ii) the barrel layers lengths and the outer radii of the disks have to be compatible with an Al-shell support structure provided by the LBNL design \cite{arrington2021eic}. Conditions (i) and (ii) are provided by internal parametrization and reflected in the Geant4 design. Potential overlaps among modules are checked before and during the optimization. }
    \label{tab:dimensionality}
\end{table}
\end{comment}




\begin{comment}
The Electron-Ion Collider (EIC) is a cutting-edge accelerator facility proposed to study the nature of the ``glue'' that binds the building blocks of the visible matter in the universe. The proposed experiment will be realized at Brookhaven National Laboratory in approximately 10 years from now, with the detector design and R\&D currently ongoing. 
%
Noticeably EIC can be one of the first facilities to leverage on Artificial Intelligence (AI) during the design and R\&D phases. Optimizing the design of its tracker is of crucial importance for the EIC Comprehensive Chromodynamics Experiment (ECCE), a consortium that is proposing a detector design based on a 1.5T solenoid. The optimization is an essential part of the design and R\&D and ECCE includes in its structure a working group dedicated to AI-based applications for the EIC detector. 
%
In this note we describe a comprehensive study in detector design of large-scale experiments using AI that has been accomplished during the detector proposal. This work required a complex parametrization of the simulated detector system. % simulated with the Fun4All framework.  
%
Our approach deals with an optimization problem in a multidimensional design space driven by multiple objectives that encode the detector performance, while satisfying several mechanical constraints. 
%
We describe our strategy and show results obtained for the ECCE tracking system. 
The AI-assisted design is agnostic to the simulation framework and can be extended after the detector proposal to other sub-detectors or system of sub-detectors to optimize the performance of the EIC detector.  
\end{comment}



\begin{comment}
\begin{table}[!]
    \centering
    %\resizebox{\columnwidth}{!}{
    \begin{adjustbox}{width=\columnwidth}
    %\begin{tabular}{| c | c | c |}
    \begin{tabular}{|M{5.cm}|M{3.cm}|M{3.5cm}|}
        \hline 
        \rowcolor{blue!15}\multicolumn{3}{|c|}{  \textbf{ECCE design (non-projective)}}\\
        \hline
        \textbf{Design Parameter} & \textbf{Reference value} & \textbf{Range} \\
        \hline
        $\mu$RWELL 1 (Inner) ($r$) Radius & 44.2 cm & [17.0, 51.0 cm] \\
        \hline
        $\mu$RWELL 2 (Inner) ($r$) Radius & 47.4 cm & [18.0, 51.0 cm] \\
        \hline
        EST 4 $z$ position &  -107.1 cm & [-110.0, -50.0 cm] \\
        \hline
        EST 3 $z$ position &  -80.0 cm & [-110.0, -40.0 cm] \\
        \hline
        EST 2 $z$ position &  -57.5 cm & [-80.0, -30.0 cm] \\
        \hline
        EST 1 $z$ position &  -35.0 cm & [-50.0, -20.0 cm] \\
        \hline
        FST 1 $z$ position & 35.0 cm & [20.0, 50.0 cm] \\
        \hline 
        FST 2 $z$ position & 57.5 cm & [30.0, 80.0 cm] \\
        \hline
        FST 3 $z$ position & 80.0 cm & [40.0, 110.0 cm] \\
        \hline
        FST 4 $z$ position & 115.0 cm & [50.0, 125.0 cm] \\
        \hline
        FST 5 $z$ position & 125.0 cm & [60.0, 125.0 cm] \\
        \hline
        \rowcolor{blue!15}\multicolumn{3}{|c|}{  \textbf{ECCE ongoing R\&D (projective)}}\\
        \hline
        \textbf{Design Parameter} & \textbf{Reference value} & \textbf{Range} \\
        \hline
        Angle (Support Cone) & 25.5 $\degree$ & [25.0$\degree$, 30.0$\degree$] \\
        \hline
        $\mu$RWELL 1 (Inner) Radius & 33.12 cm & [25.0, 45.0 cm] \\
        \hline
        ETTL $z$ position & -169.0 cm & [-171.0, -161.0 cm] \\
        \hline
        EST 2 $z$ position &  -80.05 cm & [45, 100 cm] \\
        \hline
        EST 1 $z$ position & -33.2 cm & [35, 50 cm] \\
        \hline
        FST 1 $z$ position & 33.2 cm & [35, 50 cm] \\
        \hline 
        FST 2 $z$ position & 79.85 cm & [45, 100 cm] \\
        \hline
        FST 5 $z$ position & 144 cm & [100, 150 cm] \\
        \hline
        FTTL $z$ postion & 182 & [156, 183 cm] \\
        \hline
        
    \end{tabular}
    \end{adjustbox}
    \caption{\textbf{Ranges of the design parameters:}  the table summarises the design points that are optimized for the non-projective and the projective case. The optimization range is also given for each parameter. The parameters corresponding to the non-projective case were optimized sequentially over at least three iterations, with each iteration having a set of parameters fixed. For instance, the EST/FST disks were optimized during the first iteration assuming symmetric design, and for the subsequent iterations the EST disks were optimized further in the electron endcap region.  
    %The other geometric parameter for each of the detector systems are calculated based on the parametrization discussed above. 
    Along with the design parameters the design comes with geometrical constraints too. 
    These are implemented as strong and soft constraints in the Table \ref{tab:constraints}. 
    \label{tab:ranges}
    }
\end{table}
\end{comment}


\begin{comment}
A thorough comparison between the non-projective ECCE simulation and the ongoing R\&D was carried out to optimize the support structure through a projective design.  
%
Fig.~\ref{fig:Phase-II_Momentum_res} shows a study of the obtained  momentum resolution 
%for the non-projective ECCE tracker reference design and the ongoing project R\&D on the projective mechanical structure for the ECCE tracker design 
in bins of pseudorapidity.
Similarly Fig.~\ref{fig:Phase-II_dth_res} shows the angular resolution while Fig.~\ref{fig:Phase-II_KF_eff} shows the Kalman filter efficiency as defined in Eq.~\eqref{eq:objective_KF}.
\end{comment}



\begin{comment}
Such improvement in resolution is the result of a continued multi-objective optimization process as described in Sec. \ref{sec:analysis} and summarized in Fig. \ref{fig:continued_optimization}, where the momentum resolution 
obtained during phase-I optimization using a preliminary detector concept is compared to both the non-projective and the projective R\&D designs which are instead derived from fully developed simulations in phase-II optimization.
\end{comment}


\begin{comment}
\begin{figure*}[!]
    \centering
    \includegraphics[width=0.23\textwidth]{figs/OptimizationResultsMomentumCompare_dp_p_p_eta_0 - 1.pdf}
    \includegraphics[width=0.23\textwidth]{figs/OptimizationResultsMomentumCompare_dp_p_p_eta_1 - 1.5.pdf}
    \includegraphics[width=0.23\textwidth]{figs/OptimizationResultsMomentumCompare_dp_p_p_eta_1.5 - 2.5.pdf}
    \includegraphics[width=0.23\textwidth]{figs/OptimizationResultsMomentumCompare_dp_p_p_eta_2.5 - 3.5.pdf}
    \caption{\textbf{Evolution of momentum resolution driven by the continued MOO:} Momentum resolutions in four bins of $\eta$. From left to right, respectively: $|\eta|<$ 1.0 corresponding to the barrel, 1.0 $|\leq \eta<|$ 1.5 corresponding to the transition region, and 1.5 $\leq |\eta| <$ 2.5 and 2.5 $\leq \eta <$ 3.5 corresponding to the two end-caps. Black points represent the first simulation campaign, and a preliminary detector concept in phase-I optimization which did not have a developed support structure; blue points represent the fully developed simulations for the final ECCE detector proposal concept; red points the ongoing R\&D for the optimization of the support structure. Compared to black, there is an improvement in performance in all $\eta$ bins with the exception of the transition region, an artifact that depends on the fact that black points do not include a realistic simulation of the material budget in the transition region. In the transition region, it can be also appreciate the improvement provided by the projective design. %\cris{polish text; reference in the document; move figures and reduce blank spaces}
    }
    \label{fig:continued_optimization}
\end{figure*}
\end{comment}

==> Submit_ArXiv/sections/summary.tex <==
\section{Summary}\label{sec:summary}

%EIC has been successfully using AI to assist the design optimization of the detector \cite{cisbani2020ai}. 

Large scale experiments in high energy nuclear physics entail unprecedented computational challenges and the optimization of their complex detector systems can benefit from AI-based strategies \cite{fanelli2022design}.

In this paper we described the successful implementation of a multi-objective optimization approach to steer the multidimensional design of the ECCE tracking system, taking into account the constraints from the global detector design. 
%
This work was accomplished during the EIC detector proposal, and was characterized by a continued optimization process where multiple optimization pipelines integrating different configurations of sub-detectors were compared using full \geant simulations. 
%
%
The insights provided by AI in such a multi-dimensional objective space characterizing the detector performance (\textit{e.g.}, tracking efficiency, momentum and angular resolutions), combined to other aspects like risk mitigation and costs reduction, helped selecting the candidate technology of the ECCE tracker. 
This approach is being used in an ongoing R\&D project where the design parametrization has been extended to include the support structure of the tracking system. 

The design optimization can be also extended to tune the parameters of a larger system of sub-detectors. Physics analyses are at the moment done after the optimization for a given detector design solution candidate, but they can be encoded during the optimization process as physics-driven objectives in addition to objectives representing the detector performance. %A thorough comparison of results obtained with different AI-based strategies (e.g., multi-objective optimization based on genetic algorithms and bayesian multi-objective optimization) can be also studied. 

Detector optimization with AI is anticipated to continue after the detector proposal, and activities are planned to further optimize the tracking system, including PID sub-detectors, particularly the dual-RICH \cite{cisbani2020ai}. 





%MOO has been used to ste


%These AI-based strategies can help to further optimize the proposed detector concept based on the experience of ECCE during the detector proposal.

==> fig/special_cases.tex <==
\begin{table*}
\caption{Special Cases}\label{tbl:special_cases}
\begin{tabular}{cccccc}
\toprule
event& activity& $\eta_{i,0}$& $ \mathcal{H}_{c_{t,i}}$& $\mathcal{I}^{\eta}_{c_{t,i}}$& $\mathcal{I}^{\psi}_{c_{t,i}}$\\
\midrule
\emph{extincts}& all of members in $c_{t,i}$ leave the project and migrate to $Null_{t+1}$& 1 &0 &${H}^*_{t\rightarrow t+1} + \sigma$ & 0\\
\emph{disintegration}& all of members in $c_{t,i}$ spread into different communities evenly& 0 & $-\ln{\frac{1}{m}}$& 0& $-\ln{\frac{1}{m}}$\\
\emph{maintain}& all members of $c_{t,i}$ migrate totally to a community in the next step& 0& 0& 0& 0\\
\bottomrule
\end{tabular}
\end{table*}


\begin{table*}
\begin{tabular}{cccccc}
\toprule
event& activity& $\eta_{i,0}$& $ \mathcal{H}_{c_{t,i}}$& $\mathcal{I}^{\mu}_{c_{t+1,j}}$& $\mathcal{I}^{\phi}_{c_{t+1,j}}$\\
\midrule
\emph{emerges}& all of members in $c_{t+1,j}$ are from $Null_{t+1}$& 1 & 0 &${H}^*_{t+1\leftarrow t} + \sigma$ & 0\\
\emph{recombination}& all of members in $c_{t+1,j}$ are from the prior communities evenly& 0 & $-\ln{\frac{1}{n}}$& 0& $-\ln{\frac{1}{n}}$ \\
\emph{maintain}& all members of $c_{t+1,j}$ are totally from a community in the prior step& 0& 0& 0& 0\\
\bottomrule
\end{tabular}
\end{table*}
